You See it, You Got it: Learning 3D Creation on Pose-Free Videos at Scale

Recent 3D generation models typically rely on limited-scale 3D `gold-labels' or 2D diffusion priors for 3D content creation. However, their performance is upper-bounded by constrained 3D priors due to the lack of scalable learning paradigms. In this work, we present See3D, a visual-conditional multi-view diffusion model trained on large-scale Internet videos for open-world 3D creation. The model aims to Get 3D knowledge by solely Seeing the visual contents from the vast and rapidly growing video data -- You See it, You Got it. To achieve this, we first scale up the training data using a proposed data curation pipeline that automatically filters out multi-view inconsistencies and insufficient observations from source videos. This results in a high-quality, richly diverse, large-scale dataset of multi-view images, termed WebVi3D, containing 320M frames from 16M video clips. Nevertheless, learning generic 3D priors from videos without explicit 3D geometry or camera pose annotations is nontrivial, and annotating poses for web-scale videos is prohibitively expensive. To eliminate the need for pose conditions, we introduce an innovative visual-condition - a purely 2D-inductive visual signal generated by adding time-dependent noise to the masked video data. Finally, we introduce a novel visual-conditional 3D generation framework by integrating See3D into a warping-based pipeline for high-fidelity 3D generation. Our numerical and visual comparisons on single and sparse reconstruction benchmarks show that See3D, trained on cost-effective and scalable video data, achieves notable zero-shot and open-world generation capabilities, markedly outperforming models trained on costly and constrained 3D datasets. Please refer to our project page at: https://vision.baai.ac.cn/see3d

==> arxiv/3_method_v0.tex <==
\section{Method}
The primary objective of this work is to build a robust 3D generative model from the perspective of dataset scaling-up.
Previous works \cite{deitke2023objaverse, tung2024megascenes,reizenstein2021common} laboriously collect 3D data from designed artists, stereo matching, or Structure from Motion (SfM), which can be costly and sometimes infeasible.   In contrast, multi-view images offer a highly scalable alternative, as they can be automatically extracted from the vast and rapidly growing Internet videos. By using multi-view prediction as a pretext task, we demonstrate that learned 3D priors enable various 3D creation applications, including single view generation, sparse views reconstruction, and 3D editing in open-world scenarios. 


\vspace{4pt}
The following sections outline our approach (Fig.\ref{fig:trainpipe}). \cref{sec:data} details the data curation pipeline, which selects static scenes with sufficient multi-view observations from raw video footage. \cref{sec:model} introduces our visual-conditional multi-view diffusion model, which effectively learns general 3D priors from pose-free videos. Finally, \cref{sec:3DGen} demonstrates a new visual-conditional 3D generation framework utilizing  a warping-based pipeline.


\subsection{Video Data Curation} \label{sec:data}
High-quality, large-scale video data rich in 3D knowledge is essential  for learning  accurate and reliable 3D priors. 
A well-defined 3D-aware video clip should exhibit two key properties: \textbf{1) temporally static scene content } and \textbf{ 2) significant  viewpoint variation} caused by the camera's ego-motion.
The first property ensures consistent 3D geometry across different viewpoints, while dynamic content can distort scene geometry and introduce biases that may degrade generation performance (\cref{fig:data}a-Row1). The second property guarantees  sufficient 3D observations from diverse  viewpoints. When the model is trained on videos with limited viewpoint variation (\cref{fig:data}a-Row2), it risks focusing on views adjacent to the reference view, rather than developing a comprehensive 3D understanding.


\vspace{4pt}
To obtain a massive volume of 3D data, we collect approximately  \textbf{25.48M} open-sourced raw videos, totaling \textbf{44.98 years} from the Internet, covering a wide range of categories, such as landscapes, drones, animals, plants, games, and actions. Specifically, our dataset is sourced from four websites: Pexels \cite{pexels}, Artgrid \cite{artgrid}, Airvuz \cite{airvuz}, and Skypixel \cite{skypixel}. We follow Emu3 \cite{wang2024emu3} to split the videos with PySceneDetect \cite{pyscene} to identify content changes and fade-in/out events. Additionally, we remove clips with excessive text using PaddleOCR \cite{paddle}. The detailed composition of our WebVi3D dataset is presented in \cref{tab:data_stat}.

\begin{table}[tb]
\centering
\resizebox{\linewidth}{!}{
\renewcommand{\arraystretch}{1.0}
\setlength{\tabcolsep}{2pt}
\begin{tabular}{c|c|cc|ccc}
\toprule
Website   & Domain    & \# Src. Vids     & Total Hrs.   &\#Fil. Vids   &\#Fil. Clips & Fil. Hrs. \\ \midrule
Pexels   & Open      &  6.18M                & 101.77K          & 0.61M    & 2.65M        & 9.96K             \\
Artgrid  & Open      & 3.94M               &  92.49K            &  0.54M     &  1.10M       & 8.77K      \\
Airvuz   & Drone Shot    &  5.10M                &  94.75K          &  0.54M      &  5.87M   & 8.72K                    \\
    Skypixel & Landscape & 10.27M          &   105.47K            & 0.61M      & 6.37M     & 8.82K                 \\ \midrule
  \textbf{Total}    & Open    & 25.48M         & 394.48K                & \textbf{2.30M  }    & \textbf{15.99M  }          & 36.27K  \\
\bottomrule
\end{tabular}
}
\vspace{-4pt}
\caption{\textbf{WebVi3D Dataset}. Sourced from four open websites, we curate  $\sim$2.30M videos, which are divided into 15.99M clips featuring temporally static scenes with large-range viewpoint.}
\vspace{-17pt}
\label{tab:data_stat}
\end{table}


\vspace{4pt}
However, identifying 3D-aware videos presents a nontrivial challenge.
As most videos are derived from real-world footage, such videos often contains dynamic scenes or  small camera movement. 
To address this, we propose a pipeline that automatically selects relevant, high-quality 3D-aware data (i.e., multi-view images)  by leveraging priors from instance segmentation \cite{maskrcnn}, optical flow \cite{raft}, and pixel tracking \cite{cotracker}. This pipeline comprises four core steps: 

\vspace{2pt}
\noindent \textbf{a) Temporal-Spatial Downsampling.}
To improve data filtering efficiency, we first downsample each video clip both temporally and spatially. The final resolution is set to 480p, and the temporal downsampling rate is set to 2. Note that this downsampling operation is applied  only during data curation, not during model training. 

\vspace{2pt}
\noindent \textbf{b) Semantic-Based Dynamic Recognition.} We employ the instance segmentation model, Mask R-CNN \cite{maskrcnn}, to generate motion masks for potential dynamic objects, such as humans, animals, and sports equipment. A threshold is applied to filter out videos based on the proportion of frames containing these objects, as they are more likely associated with dynamic scenes.  

\vspace{2pt}
\noindent \textbf{c) Non-Rigid Dynamic Filtering.} To precisely filter out videos with dynamic regions, we use offline optical flow estimation \cite{raft} to obtain dense matching, which enables us to identify non-rigid motion masks in video frames. These masks are then analyzed based on their locations to further determine whether the video contains dynamic content.

\vspace{2pt}
\noindent \textbf{d) Tracking-Based Small Viewpoint Filtering.} The previous three steps yield videos with static scenes.  To further ensure these videos contain multi-view images captured from a larger camera viewpoint, we track the motion trajectory of key points across frames and calculate the radius of the minimum outer tangent circle of the trajectory.
Videos with a small trajectory radius are then filtered out. More details about the data curation pipeline are provided in the Appendix \ref{supp:data}.


\begin{figure}[ht]
\centering
\includegraphics[width=\linewidth]{images/data3.pdf}
 \vspace{-17pt}
\caption{\small(a-Row1): Dynamic content modifies  scene geometry across views; (a-Row2): Limited camera movement provides insufficient multi-view observations; (b) Our \data comprises static scenes with diverse camera trajectories.} 
\vspace{-12pt}
\label{fig:data}
\end{figure}


\vspace{4pt}
Finally, we curate approximately 320M multi-view images from 15.99M video clips with static content and sufficient multi-view observations (see Fig.\ref{fig:data}b). To validate the effectiveness of our data acquisition method, we randomly select 10,000 video clips for human annotation, of which 8,859 were labeled as 3D-aware, representing 88.6\% of the total. This indicates that our pipeline effectively identifies  3D-aware videos from massive source videos. As the volume of Internet videos continues to grow, this pipeline can continuously acquire more 3D-aware data, allowing for ongoing expansion of our dataset.

 % \vspace{4pt}
\subsection{Visual Conditional Multi-View Diffusion Model} \label{sec:model}
\paragraph{Preliminary.}
Diffusion models \cite{sohl2015deep,song2020denoising,ho2020denoising} operate by perturbing the training data $X_0 \sim  q(X_0)$ through a forward diffusion process and learning to reverse it. The forward diffusion process $X_t \sim q_{t|0}(X_t | X_0)$ can be formally represented by $X_{t} = \sqrt{\bar{\alpha}_{t}} \mathbf{X}_0 + \sqrt{1 - \bar{\alpha}_{t}} \boldsymbol{\epsilon}, \quad \boldsymbol{\epsilon} \sim \mathcal{N}(0, \mathbf{I})$, where $\bar{\alpha}_{t}$ is variance schedule used in noise scheduler. In theory, $X_t$ approximates an isotropic Gaussian distribution for sufficiently large timesteps $t$. The training objective is to learn the reverse process. 

\vspace{4pt}
\noindent\textbf{Objective.} We aim for multi-view prediction: generating novel views along specified camera trajectories from a single or sparse input while ensuring consistency with the input appearance. 
The MVD model inherits the generalizability of the 2D diffusion model while capturing cross-view consistency, which naturally aligns with our goal.  Following this line, we present \ours, a pose-free, visual-conditional MVD model trained on Internet videos to enable robust 3D generation, as shown in  Fig.\ref{fig:trainpipe}.


\vspace{4pt}
\noindent\textbf{Challenge.} The main technical challenge lies in learning precise camera control from pose-free videos. 
Previous works commonly incorporate camera parameters for both input and target views into diffusion models to guide multi-view generation from specified viewpoints. However, training these models generally requires expensive 3D data with precise camera pose annotations, which limits scalability. 
To address this,  we explore an alternative approach that conditions on 2D-inductive visual hints to implicitly control camera movement during training, thereby avoiding the need for hard-to-obtain camera trajectories. 

\vspace{4pt}
\noindent\textbf{Formulation.} Formally, we propose training the MVD model conditioned on 2D-inductive visual signals, referred to as \textit{visual-condition}, without incorporating  camera parameters. This task can be formulated as designing a conditional distribution, achieved by a conditional diffusion model that minimizes:
\begin{equation}
\label{eq:loss}
\mathbb{E}_{X_0, Y_0, \epsilon, t} \left[ \left\lVert \epsilon_{\theta}(X_t, Y_0, V, t) - \epsilon \right\rVert_2^2 \right],
\end{equation}
where $X_t$ denotes the noisy latent. $X_0=\left \{ x_{0}^{i}  \right \} _{i=1}^{N}$ represents a multi-view observation of 3D content, formed by sampling one clip from  \textit{\data}  as described in Section \ref{sec:data}, with $N=S+L$ being the number of frames in each clip.  
From $X_0$, $S$ frames are randomly selected as reference views, noted as $Y_0=\left \{ y_{0}^{i}  \right \} _{i=1}^{S}$,  while the remaining $L$ frames are treated as target images, denoted $G=\left \{ g^{i}  \right \} _{i=1}^{L}$. Our approach focuses on constructing the \textit{visual-condition} $V$, which guides the diffusion model to generate plausible 3D content estimates from target viewpoints, ensuring consistency with the appearance of $Y_0$. 

\vspace{4pt}
\noindent\textbf{Principle of Visual-condition.}
A desirable \textit{visual-condition} should meet the following criteria: a) it can be constructed without the need for additional 3D annotations, b) it is independent of specific downstream tasks, and c) it offers sufficient generalization to support various task-specific visual conditions, enabling precise control of camera movements.

\vspace{4pt}
Ideally, this \textit{visual-condition} can be derived  from  pixel-space hints within the original videos, implicitly guiding the model to learn camera control.
Moreover, it should be robust enough to handle domain gaps between task-specific visual cues and pixels extracted from video data.
For example, in warping-based generation, warped images often suffer from issues like self-occlusions, artifacts, and distortions, creating a significant gap compared to real video data as shown in Fig.\ref{fig:single-3d} and Fig.\ref{fig:Vt-ablation}. Based on this, we propose constructing the \textit{visual-condition} by applying masks and noise to the input video data. Our design principles are: 

\begin{itemize}
\item \textbf{Masking}: Corrupting video data through random masking reduces reliance on direct pixel-space visual signals, helping the model partially mitigate the domain gap between task-specific visual cues and video data. 
\item \textbf{Noise Addition}: Adding noise to video data to approximate a Gaussian distribution. When applied to different downstream tasks, task-specific visual inputs are similarly noised, aligning their distribution with a Gaussian profile, and further bridging  the gap between video data and task-specific visual input.
\end{itemize}

\vspace{4pt}
\noindent\textbf{Time-dependent Visual Condition.} We initially add noise and random irregular masks to video data, creating what we call `corrupted' video data $C_t$, as defined in Eq.\ref{eq:ct}. This corrupted data is then used as the \textit{visual-condition} for MVD model training.
A key challenge of this strategy lies in determining the appropriate level of perturbation. If too much noise is added, the conditional signals become ineffective, resulting in poor visual quality and inaccurate camera control. Conversely, if insufficient noise is added, the corrupted data retains substantial details from the target images, causing the model to overly rely on visual hints from video data.

\vspace{4pt}
To overcome this, we further introduce a \textit{time-dependent noise} distribution applied to video data. The core idea is to apply higher noise levels at larger time steps, effectively disrupting video data to prevent over-reliance on it.
As the time step decreases, the noise level is reduced, providing cleaner conditional signals to facilitate content generation.
However, as the noise level decreases, the risk of information leakage increases, causing the distribution to deviate from a Gaussian distribution.
To mitigate this, we propose gradually replacing corrupted data $C_t$ with noisy latent $X_t$ as the \textit{visual-condition} 
 (see Eq.\ref{eq:mix}) , encouraging the model to primarily rely on $X_t$ for generation while minimizing dependence on pixel-space signals from video data as timestep decreases. Additionally, $X_t$ is predicted by the model, thus exhibiting task-agnostic property, as formalized by:
\begin{equation} \label{eq:ct}
C_{t} = \sqrt{\bar{\alpha}_{t'}} (1-M)\mathbf{X}_0 + \sqrt{1 - \bar{\alpha}_{t'}} \boldsymbol{\epsilon}, \quad \boldsymbol{\epsilon} \sim \mathcal{N}(0, \mathbf{I})
\end{equation}
\begin{equation} \label{eq:mix}
V_t=[W_t\ast C_t+  \left ( 1-W_t \right ) \ast X_t;M],
\end{equation}

\noindent where $M = \left\{  m^{0:S} \cup m^{S+1:N} \right \}$, with $m^{0:S}$ as the zero matrix, keeping the reference images $Y_0$ unmasked, and $m^{S+1:N}$ as random irregular masks applied to the target images $G$. $t'=f(t)$, function $f$ is strictly monotonically increasing and requires $t' < t$, which guarantees that $C_t$ contains at least as much information as $X_t$ at earlier timesteps. Here, $\bar{\alpha}_{t'}$ are variances used in DDIM \cite{song2020denoising},  and $V_t=\left \{ v_{t}^{i}  \right \} _{i=1}^{N}$ represents our final \textit{ visual-condition}, which is a mixture of $C_t$ and $X_t$, concatenated with masks $M$ along the channel dimension. 
The term $W_t$ denotes a balancing weight that decreases monotonically with timestep $t$, ranging from 1 to 0.
In practice, an additional processing step assigns $v_{t}^{0:S}$ to the reference images $Y_0$ directly, in order to inject the clean information of $Y_0$ into the model, facilitating alignment between the predicted images and the reference images.
Consequently, Eq.\ref{eq:loss} can be reformulated as $\mathbb{E}_{X_0, Y_0, \epsilon, t} \left[ \left\lVert \epsilon_{\theta}(X_t, Y_0, V_t, t) - \epsilon \right\rVert_2^2 \right]$. More detailed  definitions of $f(t)$ and $W_t$ are provided in the Appendix \ref{supp:ftwt}.


\vspace{4pt}
\noindent\textbf{Model Architecture.}
Our model architecture is based on video diffusion model \cite{svd}. However, we removed the time embedding, as we aim for the model to control the camera movement purely through visual conditions, rather than inferring movement trends based on temporal cues. To further minimize the effect of temporality, we shuffle the frames in each video clip, treating the data as unordered $X_0$. 
Specifically,  we randomly select a subset of frames from a video clip as reference images, with the remaining frames as target images. The number of reference images is randomly selected to accommodate different downstream tasks.  The multi-view diffusion model is optimized by calculating the loss only on the target images, as described in Eq.\ref{eq:loss}. Additional details on the model architecture, including the design of self-attention layers, Zero-Initialize, trainable parameters, noise schedule, and cross-attention, are provided in the Appendix \ref{supp:model}.


\subsection{Visual Conditional 3D Generation} \label{sec:3DGen}
\begin{figure*}[tb]
\centering
\includegraphics[width=0.9\linewidth]{images/infer4.pdf}
\caption{\small \textbf{\ours for Multi-View Generation}: From  iteratively generated views ({\color{brown}brown camera}), we randomly select a few anchor views (yellow stars) to guide  the generation of  target views along the {\color[RGB]{122,124,126}\textbf{gray camera trajectory}}. 
Keypoint matching is first performed to establish correspondences between the anchor views.
Next, monocular depth estimation is applied to the latest anchor view, followed by our 
 \textit{Iterative Sparse Pixel-Wise Depth Alignment} to refine the depth and recover a dense map. This dense depth is then used to warp images along the gray camera viewpoints. Subsequently, the warped images and anchor images are combined and processed according to Eq.\ref{eq:ct} and  Eq.\ref{eq:mix}, without random masking, forming the \textit{visual-condition}, which guides  MVD model to produce  3D-consistent target views. Finally, the {\color[RGB]{122,124,126}\textbf{gray camera}} turns to {\color{brown}brown}, guiding multi-view generation in the next iteration.
} 
\vspace{-15pt}
\label{fig:infer}
\end{figure*}



\noindent\textbf{Overview. }
This section demonstrates the application of \ours for domain-free 3D generation, supporting long-sequence novel view  synthesis  with complex camera trajectories. Starting with one or a few input views, we iteratively generate warped images as visual hints, guided by predefined camera poses and estimated global depth \cite{bhat2023zoedepth}. \ours is then utilized  to generate novel views along the predefined camera trajectory, conditioned on the proposed \textit{visual-condition}. This iterative pipeline is illustrated in Fig.\ref{fig:infer}, where the brown cameras represent the already generated views, and the gray cameras indicate the target views we aim to generate.


\vspace{4pt}
\noindent \textbf{Challenge.}
Recent warping-based 3D generation approaches  \cite{chung2023luciddreamer, fridman2024scenescape, lei2023rgbd2} rely on monocular depth or point clouds, and perform global point-cloud alignment to recover the actual geometry for subsequent generations. However, as the reference view often provides a limited scene observation, using offline methods tends to suffer from \textit{scale ambiguity} and \textit{geometric estimation errors}.  Moreover, previous methods often overlook correcting these geometric errors,  leading to distortions and stretching artifacts. These errors accumulate during iterative generation, severely degrading the generation quality. To address this, we propose an iterative  strategy with sparse pixel-wise depth alignment, comprising two core steps: pixel-wise depth scale alignment and global metric depth recovery.


\vspace{4pt}
\noindent \textbf{Pixel-wise Depth Scale Alignment.} We introduce  pixel-wise depth scale alignment using sparse keypoints. This approach performs high-degree-of-freedom independent optimization for all keypoints by leveraging multi-view matching priors from anchor views. Each keypoint independently identifies its multi-view correspondences, allowing for the recovery of both depth scale and surrounding geometry. The corrected scale is then propagated across the entire depth map using 2D distances between keypoints and their neighbors.

\vspace{4pt}
Specifically, denote $\{T_i\}_{i=0}^{N}$ the predefined camera trajectory. Assuming we have generated $n$ images $\{I_i\}_{i=0}^n$, we now proceed to generate the next $m$ views using the warped image from the last anchor view $I_n$,  referred to as the source view. We first utilize the pre-trained MoGe \cite{wang2024moge} to estimate the affine-invariant depth $\boldsymbol{\hat{D}}_n$ of $I_n$. Inspired by \cite{xu2023frozenrecon}, we perform sparse alignment with $1024$ pairs of matching keypoints $\{\mathbf{m}_n, \mathbf{m}_i\}_k$, obtained by the pre-trianed extractor SuperPoint \cite{detone2018superpoint} and feature matcher LightGlue \cite{lindenberger2023lightglue}. For each matched point, we optimize the corresponding scale $\alpha^k$ and shift $\beta^k$ parameters, where $k \in [0, 1024]$, Our core idea is to recover the depth scaling by minimizing the $L_2$ distance of re-projection between matching points. For each iteration, the warping operation $\Pi_{n\rightarrow i}$ transforms pixels from the source image’s coordinate frame to the target image’s coordinate frame, formulated as: $\Pi_{n \rightarrow i}(\hat{d}_n) =  \hat{d}_n K_{i} T_{i} T_{n}^{-1} K_{n}^{-1}$, where $K_i,  K_n,T_i, T_n$ represent the intrinsic and extrinsic parameters of the source and target frames, respectively. The alignment for each pair is performed using normalized coordinates, ensuring that the warping aligns with the matching prior:
\begin{equation}
    \alpha^{k*},\beta^{k*} = \mathop{argmin} \limits_{\alpha^{k},\beta^{k}} || \hat{d}_n^{k*} K_i T_i T_n^{-1} K_n^{-1} m_n^t - m_i^t||_2^2,
\end{equation}
\noindent where the recovered depth of $k$th pixel is $\hat{d}_n^{k*} = \alpha^{k} \odot \hat{d}_n^k + \beta^{k}$, the $\odot$ is the pixel-wise Hadamard Product. We minimize the matching loss via gradient descent to obtain best scale $ \alpha^{k*}$ and shift parameters $\beta^{k*}$ for each pixel. By performing individual scale recovery and geometry correction, we decouple the depth correlation among different points, achieving accurate single-view reconstruction.

\vspace{4pt}
\noindent \textbf{Global Metric Depth Recovery.} After that, we set these recovered positions as sparse guidance $\hat{d}_n^*$, and introduce Locally Weighted Linear Regression \cite{xu2023frozenrecon} (marked as LWLR in Fig.\ref{fig:infer}) to recover the whole depth map based on the locations between guided points and the other target points. Denote $(u,v)$ represent the 2D positions of the remaining target points, their depth $\boldsymbol{\hat{D}}_n$ can be fitted to the sparse guided points by minimizing the squared locally weighted distance, which is reweighed by the diagonal weight matrix as:
\begin{equation}\boldsymbol{W}_{u,v}=diag(w_1,w_2,...,w_m), w_i=\frac1{\sqrt{2\pi}}\exp(-\frac{\mathrm{dist}_i^2}{2b^2}),
\end{equation}
where $b$ is the bandwidth of Gaussian kernel, and $\mathrm{dist}$ is the Euclidean distance between the guided point and the underestimated target point. Denote $\boldsymbol{X}$ the homogeneous representation of $\boldsymbol{\hat{D}}_n$, the scale map $\boldsymbol{S}_{scale}$ and shift map $\boldsymbol{S}_{shift}$ of target points can be calculated by iterating every location on the whole image, which can be formulated as:
\begin{equation}
    \begin{gathered}
        \min_{\boldsymbol{\beta}_{u, v}} (\hat{d}_n^* -\boldsymbol{X}\boldsymbol{\beta}_{u,v})^\mathsf{T}\boldsymbol{W}_{u,v}(\hat{d}_n^* -\boldsymbol{X}\boldsymbol{\beta}_{u,v})+\lambda\boldsymbol{S}_{shift}^2, \\
    \boldsymbol{\hat{\beta}}_{u,v}=(\boldsymbol{X}^\mathsf{T}\boldsymbol{W}_{u,v}\boldsymbol{X}+\lambda)^{-1}\boldsymbol{X}^\mathsf{T}\boldsymbol{W}_{u,v}\hat{d}_n^*, \\
    \boldsymbol{\beta_{u,v}} = [\boldsymbol{S}_{scale},\boldsymbol{S}_{shift}]_{u,v} ^ \mathsf{T}, \\
    \boldsymbol{D}_n = \hat{d}_n^* \oplus  \boldsymbol{S}_{scale} \odot \boldsymbol{\hat{D}}_n + \boldsymbol{S}_{shift},
\end{gathered}
\end{equation}

\noindent where $\boldsymbol{D}_n$ is the scaled whole depth map, $\oplus$ is the concatenation operator, $\lambda$ is a $l_2$ regularization hyperparameter used for restricting the solution to be simple. Besides, the explicit constraint of the source frame with the target frames allows each novel view to maintain contextual consistency from preceding generations.

\vspace{4pt}
\noindent \textbf{Novel View Generation.}
After obtaining the aligned depth $\boldsymbol{D}_n$, we generate target visual hints through warping as $\hat{I}_j = \Pi_{n \rightarrow j}(\boldsymbol{D}_n)$. The warped images $\{\hat{I}_j\}_{j=n}^{n+m}$ contain  unfilled regions,  as indicated by the binary warping mask $\{M_j\}_{j=n}^{n+m}$, providing strong visual hints for \ours to perform novel view generation. To ensure strong multi-view consistency between the newly generated sequence and the previous content, we randomly select $k$ anchor views $\{I_k\},k \in [1,N]$ from the earlier generated frames to guide subsequent generation. The generation process is formulated as: $I_j = \ours (\hat{I}_j, M_{j}, \{I_0,I_k\})$.
We iteratively perform depth estimation, alignment, warping, and generation  until all predefined multi-view images are obtained. 

\vspace{4pt}
\noindent\textbf{3D Reconstruction.} \label{sec: 3dgs}
We reconstruct the 3D scene using 3D Gaussian Splatting (3DGS) \cite{3dgs}. 
The training objective is to minimize the sum of photometric loss and SSIM loss, consistent with the original 3DGS approach. Additionally, we introduce a perceptual loss (LPIPS \cite{lpips}) to mitigate subtle \textit{inter-frame} discrepancies in multi-view generated images during 3DGS reconstruction. LPIPS emphasizes higher-level semantic consistency between Gaussian-rendered and generated multi-view images, rather than focusing on minor high-frequency differences.
Furthermore, the potential \textit{inner-frame} diversity may lead to inconsistencies with the corresponding camera poses. Following \cite{fan2024instantsplat}, we implement joint pose-Gaussian optimization, treating camera parameters as learnable variables alongside Gaussian attributes, thereby reducing gaps between generated viewpoints and their corresponding camera poses.




==> arxiv/3_method_v1.tex <==
\section{Method}
The primary objective of this work is to build a robust 3D generative model from the perspective of dataset scaling-up.
Previous works \cite{deitke2023objaverse, tung2024megascenes,reizenstein2021common} laboriously collect 3D data from designed artists, stereo matching, or Structure from Motion (SfM), which can be costly and sometimes infeasible.   In contrast, multi-view images offer a highly scalable alternative, as they can be automatically extracted from the vast and rapidly growing Internet videos. By using multi-view prediction as a pretext task, we demonstrate that learned 3D priors enable various 3D creation applications, including single view generation, sparse views reconstruction, and 3D editing in open-world scenarios. 


\vspace{4pt}
The following sections outline our approach (Fig.\ref{fig:trainpipe}). \cref{sec:data} details the data curation pipeline, which selects static scenes with sufficient multi-view observations from raw video footage. \cref{sec:model} introduces our visual-conditional multi-view diffusion model, which effectively learns general 3D priors from pose-free videos. Finally, \cref{sec:3DGen} demonstrates a new visual-conditional 3D generation framework utilizing  a warping-based pipeline.


\subsection{Video Data Curation} \label{sec:data}
High-quality, large-scale video data rich in 3D knowledge is essential  for learning  accurate and reliable 3D priors. 
A well-defined 3D-aware video clip should exhibit two key properties: \textbf{1) temporally static scene content } and \textbf{ 2) significant  viewpoint variation} caused by the camera's ego-motion.
The first property ensures consistent 3D geometry across different viewpoints, while dynamic content can distort scene geometry and introduce biases that may degrade generation performance (\cref{fig:data}a-Row1). The second property guarantees  sufficient 3D observations from diverse  viewpoints. When the model is trained on videos with limited viewpoint variation (\cref{fig:data}a-Row2), it risks focusing on views adjacent to the reference view, rather than developing a comprehensive 3D understanding.


\vspace{4pt}
To obtain a massive volume of 3D data, we collect approximately  \textbf{25.48M} open-sourced raw videos, totaling \textbf{44.98 years} from the Internet, covering a wide range of categories, such as landscapes, drones, animals, plants, games, and actions. Specifically, our dataset is sourced from four websites: Pexels \cite{pexels}, Artgrid \cite{artgrid}, Airvuz \cite{airvuz}, and Skypixel \cite{skypixel}. We follow Emu3 \cite{wang2024emu3} to split the videos with PySceneDetect \cite{pyscene} to identify content changes and fade-in/out events. Additionally, we remove clips with excessive text using PaddleOCR \cite{paddle}. The detailed composition of our WebVi3D dataset is presented in \cref{tab:data_stat}.

\begin{table}[tb]
\centering
\resizebox{\linewidth}{!}{
\renewcommand{\arraystretch}{1.0}
\setlength{\tabcolsep}{2pt}
\begin{tabular}{c|c|cc|ccc}
\toprule
Website   & Domain    & \# Src. Vids     & Total Hrs.   &\#Fil. Vids   &\#Fil. Clips & Fil. Hrs. \\ \midrule
Pexels   & Open      &  6.18M                & 101.77K          & 0.61M    & 2.65M        & 9.96K             \\
Artgrid  & Open      & 3.94M               &  92.49K            &  0.54M     &  1.10M       & 8.77K      \\
Airvuz   & Drone Shot    &  5.10M                &  94.75K          &  0.54M      &  5.87M   & 8.72K                    \\
    Skypixel & Landscape & 10.27M          &   105.47K            & 0.61M      & 6.37M     & 8.82K                 \\ \midrule
  \textbf{Total}    & Open    & 25.48M         & 394.48K                & \textbf{2.30M  }    & \textbf{15.99M  }          & 36.27K  \\
\bottomrule
\end{tabular}
}
\vspace{-4pt}
\caption{\textbf{WebVi3D Dataset}. Sourced from four open websites, we curate  $\sim$2.30M videos, which are divided into 15.99M clips featuring temporally static scenes with large-range viewpoint.}
\vspace{-17pt}
\label{tab:data_stat}
\end{table}


\vspace{4pt}
However, identifying 3D-aware videos presents a nontrivial challenge.
As most videos are derived from real-world footage, such videos often contains dynamic scenes or  small camera movement. 
To address this, we propose a pipeline that automatically selects relevant, high-quality 3D-aware data (i.e., multi-view images)  by leveraging priors from instance segmentation \cite{maskrcnn}, optical flow \cite{raft}, and pixel tracking \cite{cotracker}. This pipeline comprises four core steps: 

\vspace{2pt}
\noindent \textbf{a) Temporal-Spatial Downsampling.}
To improve data filtering efficiency, we first downsample each video clip both temporally and spatially. The final resolution is set to 480p, and the temporal downsampling rate is set to 2. Note that this downsampling operation is applied  only during data curation, not during model training. 

\vspace{2pt}
\noindent \textbf{b) Semantic-Based Dynamic Recognition.} We employ the instance segmentation model, Mask R-CNN \cite{maskrcnn}, to generate motion masks for potential dynamic objects, such as humans, animals, and sports equipment. A threshold is applied to filter out videos based on the proportion of frames containing these objects, as they are more likely associated with dynamic scenes.  

\vspace{2pt}
\noindent \textbf{c) Non-Rigid Dynamic Filtering.} To precisely filter out videos with dynamic regions, we use offline optical flow estimation \cite{raft} to obtain dense matching, which enables us to identify non-rigid motion masks in video frames. These masks are then analyzed based on their locations to further determine whether the video contains dynamic content.

\vspace{2pt}
\noindent \textbf{d) Tracking-Based Small Viewpoint Filtering.} The previous three steps yield videos with static scenes.  To further ensure these videos contain multi-view images captured from a larger camera viewpoint, we track the motion trajectory of key points across frames and calculate the radius of the minimum outer tangent circle of the trajectory.
Videos with a small trajectory radius are then filtered out. More details about the data curation pipeline are provided in the Appendix \ref{supp:data}.


\begin{figure}[ht]
\centering
\includegraphics[width=\linewidth]{images/data3.pdf}
 \vspace{-17pt}
\caption{\small(a-Row1): Dynamic content modifies  scene geometry across views; (a-Row2): Limited camera movement provides insufficient multi-view observations; (b) Our \data comprises static scenes with diverse camera trajectories.} 
\vspace{-12pt}
\label{fig:data}
\end{figure}


\vspace{4pt}
Finally, we curate approximately 320M multi-view images from 15.99M video clips with static content and sufficient multi-view observations (see Fig.\ref{fig:data}b). To validate the effectiveness of our data acquisition method, we randomly select 10,000 video clips for human annotation, of which 8,859 were labeled as 3D-aware, representing 88.6\% of the total. This indicates that our pipeline effectively identifies  3D-aware videos from massive source videos. As the volume of Internet videos continues to grow, this pipeline can continuously acquire more 3D-aware data, allowing for ongoing expansion of our dataset.

 % \vspace{4pt}
\subsection{Visual Conditional Multi-View Diffusion Model} \label{sec:model}
\paragraph{Preliminary.}
Diffusion models \cite{sohl2015deep,song2020denoising,ho2020denoising} operate by perturbing the training data $X_0 \sim  q(X_0)$ through a forward diffusion process and learning to reverse it. The forward diffusion process $X_t \sim q_{t|0}(X_t | X_0)$ can be formally represented by $X_{t} = \sqrt{\bar{\alpha}_{t}} \mathbf{X}_0 + \sqrt{1 - \bar{\alpha}_{t}} \boldsymbol{\epsilon}, \quad \boldsymbol{\epsilon} \sim \mathcal{N}(0, \mathbf{I})$, where $\bar{\alpha}_{t}$ is variance schedule used in noise scheduler. In theory, $X_t$ approximates an isotropic Gaussian distribution for sufficiently large timesteps $t$. The training objective is to learn the reverse process. 

\vspace{4pt}
\noindent\textbf{Objective.} We aim for multi-view prediction: generating novel views along specified camera trajectories from a single or sparse input while ensuring consistency with the input appearance. 
The MVD model inherits the generalizability of the 2D diffusion model while capturing cross-view consistency, which naturally aligns with our goal.  Following this line, we present \ours, a pose-free, visual-conditional MVD model trained on Internet videos to enable robust 3D generation, as shown in  Fig.\ref{fig:trainpipe}.


\vspace{4pt}
\noindent\textbf{Challenge.} The main technical challenge lies in learning precise camera control from pose-free videos. 
Previous works commonly incorporate camera parameters for both input and target views into diffusion models to guide multi-view generation from specified viewpoints. However, training these models generally requires expensive 3D data with precise camera pose annotations, which limits scalability. 
To address this,  we explore an alternative approach that conditions on 2D-inductive visual hints to implicitly control camera movement during training, thereby avoiding the need for hard-to-obtain camera trajectories. 

\vspace{4pt}
\noindent\textbf{Formulation.} Formally, we propose training the MVD model conditioned on 2D-inductive visual signals, referred to as \textit{visual-condition}, without incorporating  camera parameters. This task can be formulated as designing a conditional distribution, achieved by a conditional diffusion model that minimizes:
\begin{equation}
\label{eq:loss}
\mathbb{E}_{X_0, Y_0, \epsilon, t} \left[ \left\lVert \epsilon_{\theta}(X_t, Y_0, V, t) - \epsilon \right\rVert_2^2 \right],
\end{equation}
where $X_t$ denotes the noisy latent. $X_0=\left \{ x_{0}^{i}  \right \} _{i=1}^{N}$ represents a multi-view observation of 3D content, formed by sampling one clip from  \textit{\data}  as described in Section \ref{sec:data}, with $N=S+L$ being the number of frames in each clip.  
From $X_0$, $S$ frames are randomly selected as reference views, noted as $Y_0=\left \{ y_{0}^{i}  \right \} _{i=1}^{S}$,  while the remaining $L$ frames are treated as target images, denoted $G=\left \{ g^{i}  \right \} _{i=1}^{L}$. Our approach focuses on constructing the \textit{visual-condition} $V$, which guides the diffusion model to generate plausible 3D content estimates from target viewpoints, ensuring consistency with the appearance of $Y_0$. 

\vspace{4pt}
\noindent\textbf{Principle of Visual-condition.}
A desirable \textit{visual-condition} should meet the following criteria: a) it can be constructed without the need for additional 3D annotations, b) it is independent of specific downstream tasks, and c) it offers sufficient generalization to support various task-specific visual conditions, enabling precise control of camera movements.

\vspace{4pt}
Ideally, this \textit{visual-condition} can be derived  from  pixel-space hints within the original videos, implicitly guiding the model to learn camera control.
Moreover, it should be robust enough to handle domain gaps between task-specific visual cues and pixels extracted from video data.
For example, in warping-based generation, warped images often suffer from issues like self-occlusions, artifacts, and distortions, creating a significant gap compared to real video data as shown in Fig.\ref{fig:single-3d} and Fig.\ref{fig:Vt-ablation}. Based on this, we propose constructing the \textit{visual-condition} by applying masks and noise to the input video data. Our design principles are: 

\begin{itemize}
\item \textbf{Masking}: Corrupting video data through random masking reduces reliance on direct pixel-space visual signals, helping the model partially mitigate the domain gap between task-specific visual cues and video data. 
\item \textbf{Noise Addition}: Adding noise to video data to approximate a Gaussian distribution. When applied to different downstream tasks, task-specific visual inputs are similarly noised, aligning their distribution with a Gaussian profile, and further bridging  the gap between video data and task-specific visual input.
\end{itemize}

\vspace{4pt}
\noindent\textbf{Time-dependent Visual Condition.} We initially add noise and random irregular masks to video data, creating what we term `corrupted' video data $C_t$, as defined in Eq.\ref{eq:ct}. This corrupted data is then served as the \textit{visual-condition} for MVD model training.
A key challenge lies in determining  the optimal perturbation level. If too much noise is added, the conditional signals become ineffective, resulting in poor visual quality and inaccurate camera control. Conversely, insufficient noise allows the corrupted data to retain significant details from target images, causing the model to over-rely on visual hints from the video data.

\vspace{4pt}
{\color{blue}Previous works \cite{muller2024multidiff,singh2022conditioning,hou2024training,zhao2024identifying} have explored various methods for modulating noise levels by adding noise to input data. Notably, Zhao et al.\cite{zhao2024identifying} introduced a time-dependent noise distribution (TimeNoise) for image-to-video diffusion models, applying noise to a reference image to mitigate information leakage and enhance  motion generation.
Inspired by this, we propose a novel time-dependent noise strategy  to enable 3D-consistent novel view generation under pose-free conditions. Unlike TimeNoise \cite{zhao2024identifying}, our approach:
1) Keeps the reference images clean, applying noise only to masked target images.  
2) Introduces a controllable mechanism, defined as \(t'=f(t),t' < t\), to regulate information leakage, preventing excessive noise from completely obscuring visual cues  and destabilizing camera control.
3) Mitigates residual information leakage at lower timesteps using a gradual replacement strategy (Eq.~\ref{eq:mix}), balancing  noise injection and information leakage  to improve generation quality and camera control.
}

\vspace{4pt}
{\color{red}Specifically, the core idea is to apply higher noise levels at larger timesteps to disrupt video data, thereby reducing the model's over-reliance on it. As  timesteps decrease, noise levels are gradually  reduced, providing cleaner conditional signals.
However, lower noise levels increase the risk of information leakage, causing  deviation from a Gaussian distribution.}
To address  this, we progressively  replace corrupted data $C_t$ with noisy latent variables $X_t$ as the \textit{visual-condition} (Eq.\ref{eq:mix}). This strategy encourages reliance primarily on the task-agnostic $X_t$, while minimizing dependence on pixel-space signals from video data as timesteps decrease, formalized by:
\begin{equation} \label{eq:ct}
C_{t} = \sqrt{\bar{\alpha}_{t'}} (1-M)\mathbf{X}_0 + \sqrt{1 - \bar{\alpha}_{t'}} \boldsymbol{\epsilon}, \quad \boldsymbol{\epsilon} \sim \mathcal{N}(0, \mathbf{I})
\end{equation}
\begin{equation} \label{eq:mix}
V_t=[W_t\ast C_t+  \left ( 1-W_t \right ) \ast X_t;M],
\end{equation}

\noindent where $M = \left\{  m^{0:S} \cup m^{S+1:N} \right \}$, with $m^{0:S}$ as the zero matrix, keeping the reference images $Y_0$ unmasked, and $m^{S+1:N}$ as random irregular masks applied to the target images $G$.  Function $f$ is strictly monotonically increasing and requires $t' < t$, which guarantees that $C_t$ contains at least as much information as $X_t$ at earlier timesteps. Here, $\bar{\alpha}_{t'}$ are variances used in DDIM \cite{song2020denoising},  and $V_t=\left \{ v_{t}^{i}  \right \} _{i=1}^{N}$ represents our final \textit{ visual-condition}, which is a mixture of $C_t$ and $X_t$, concatenated with masks $M$ along the channel dimension. 
The term $W_t$ denotes a balancing weight that decreases monotonically with timestep $t$, ranging from 1 to 0.
In practice, an additional processing step assigns $v_{t}^{0:S}$ to the reference images $Y_0$ directly, in order to inject the clean information of $Y_0$ into the model, facilitating alignment between the predicted images and the reference images.
Consequently, Eq.\ref{eq:loss} can be reformulated as $\mathbb{E}_{X_0, Y_0, \epsilon, t} \left[ \left\lVert \epsilon_{\theta}(X_t, Y_0, V_t, t) - \epsilon \right\rVert_2^2 \right]$. More detailed  definitions of $f(t)$ and $W_t$ are provided in the Appendix \ref{supp:ftwt}.


\vspace{4pt}
\noindent\textbf{Model Architecture.}
Our model architecture is based on video diffusion model \cite{svd}. However, we removed the time embedding, as we aim for the model to control the camera movement purely through visual conditions, rather than inferring movement trends based on temporal cues. To further minimize the effect of temporality, we shuffle the frames in each video clip, treating the data as unordered $X_0$. 
Specifically,  we randomly select a subset of frames from a video clip as reference images, with the remaining frames as target images. The number of reference images is randomly selected to accommodate different downstream tasks.  The multi-view diffusion model is optimized by calculating the loss only on the target images, as described in Eq.\ref{eq:loss}. Additional details on the model architecture, including the design of self-attention layers, Zero-Initialize, trainable parameters, noise schedule, and cross-attention, are provided in the Appendix \ref{supp:model}.


\subsection{Visual Conditional 3D Generation} \label{sec:3DGen}
\begin{figure*}[tb]
\centering
\includegraphics[width=0.9\linewidth]{images/infer4.pdf}
\caption{\small \textbf{\ours for Multi-View Generation}: From  iteratively generated views ({\color{brown}brown camera}), we randomly select a few anchor views (yellow stars) to guide  the generation of  target views along the {\color[RGB]{122,124,126}\textbf{gray camera trajectory}}. 
Keypoint matching is first performed to establish correspondences between the anchor views.
Next, monocular depth estimation is applied to the latest anchor view, followed by our 
 \textit{Iterative Sparse Pixel-Wise Depth Alignment} to refine the depth and recover a dense map. This dense depth is then used to warp images along the gray camera viewpoints. Subsequently, the warped images and anchor images are combined and processed according to Eq.\ref{eq:ct} and  Eq.\ref{eq:mix}, without random masking, forming the \textit{visual-condition}, which guides  MVD model to produce  3D-consistent target views. Finally, the {\color[RGB]{122,124,126}\textbf{gray camera}} turns to {\color{brown}brown}, guiding multi-view generation in the next iteration.
} 
\vspace{-15pt}
\label{fig:infer}
\end{figure*}



\noindent\textbf{Overview. }
This section demonstrates the application of \ours for domain-free 3D generation, supporting long-sequence novel view  synthesis  with complex camera trajectories. Starting with one or a few input views, we iteratively generate warped images as visual hints, guided by predefined camera poses and estimated global depth \cite{bhat2023zoedepth}. \ours is then utilized  to generate novel views along the predefined camera trajectory, conditioned on the proposed \textit{visual-condition}. This iterative pipeline is illustrated in Fig.\ref{fig:infer}, where the brown cameras represent the already generated views, and the gray cameras indicate the target views we aim to generate.


\vspace{4pt}
\noindent \textbf{Challenge.}
Recent warping-based 3D generation approaches  \cite{chung2023luciddreamer, fridman2024scenescape, lei2023rgbd2} rely on monocular depth or point clouds, and perform global point-cloud alignment to recover the actual geometry for subsequent generations. However, as the reference view often provides a limited scene observation, using offline methods tends to suffer from \textit{scale ambiguity} and \textit{geometric estimation errors}.  Moreover, previous methods often overlook correcting these geometric errors,  leading to distortions and stretching artifacts. These errors accumulate during iterative generation, severely degrading the generation quality. To address this, we propose an iterative  strategy with sparse pixel-wise depth alignment, comprising two core steps: pixel-wise depth scale alignment and global metric depth recovery.


\vspace{4pt}
\noindent \textbf{Pixel-wise Depth Scale Alignment.} We introduce  pixel-wise depth scale alignment using sparse keypoints. This approach performs high-degree-of-freedom independent optimization for all keypoints by leveraging multi-view matching priors from anchor views. Each keypoint independently identifies its multi-view correspondences, allowing for the recovery of both depth scale and surrounding geometry. The corrected scale is then propagated across the entire depth map using 2D distances between keypoints and their neighbors.

\vspace{4pt}
Specifically, denote $\{T_i\}_{i=0}^{N}$ the predefined camera trajectory. Assuming we have generated $n$ images $\{I_i\}_{i=0}^n$, we now proceed to generate the next $m$ views using the warped image from the last anchor view $I_n$,  referred to as the source view. We first utilize the pre-trained MoGe \cite{wang2024moge} to estimate the affine-invariant depth $\boldsymbol{\hat{D}}_n$ of $I_n$. Inspired by \cite{xu2023frozenrecon}, we perform sparse alignment with $1024$ pairs of matching keypoints $\{\mathbf{m}_n, \mathbf{m}_i\}_k$, obtained by the pre-trianed extractor SuperPoint \cite{detone2018superpoint} and feature matcher LightGlue \cite{lindenberger2023lightglue}. For each matched point, we optimize the corresponding scale $\alpha^k$ and shift $\beta^k$ parameters, where $k \in [0, 1024]$, Our core idea is to recover the depth scaling by minimizing the $L_2$ distance of re-projection between matching points. For each iteration, the warping operation $\Pi_{n\rightarrow i}$ transforms pixels from the source image’s coordinate frame to the target image’s coordinate frame, formulated as: $\Pi_{n \rightarrow i}(\hat{d}_n) =  \hat{d}_n K_{i} T_{i} T_{n}^{-1} K_{n}^{-1}$, where $K_i,  K_n,T_i, T_n$ represent the intrinsic and extrinsic parameters of the source and target frames, respectively. The alignment for each pair is performed using normalized coordinates, ensuring that the warping aligns with the matching prior:
\begin{equation}
    \alpha^{k*},\beta^{k*} = \mathop{argmin} \limits_{\alpha^{k},\beta^{k}} || \hat{d}_n^{k*} K_i T_i T_n^{-1} K_n^{-1} m_n^t - m_i^t||_2^2,
\end{equation}
\noindent where the recovered depth of $k$th pixel is $\hat{d}_n^{k*} = \alpha^{k} \odot \hat{d}_n^k + \beta^{k}$, the $\odot$ is the pixel-wise Hadamard Product. We minimize the matching loss via gradient descent to obtain best scale $ \alpha^{k*}$ and shift parameters $\beta^{k*}$ for each pixel. By performing individual scale recovery and geometry correction, we decouple the depth correlation among different points, achieving accurate single-view reconstruction.

\vspace{4pt}
\noindent \textbf{Global Metric Depth Recovery.} After that, we set these recovered positions as sparse guidance $\hat{d}_n^*$, and introduce Locally Weighted Linear Regression \cite{xu2023frozenrecon} (marked as LWLR in Fig.\ref{fig:infer}) to recover the whole depth map based on the locations between guided points and the other target points. Denote $(u,v)$ represent the 2D positions of the remaining target points, their depth $\boldsymbol{\hat{D}}_n$ can be fitted to the sparse guided points by minimizing the squared locally weighted distance, which is reweighed by the diagonal weight matrix as:
\begin{equation}\boldsymbol{W}_{u,v}=diag(w_1,w_2,...,w_m), w_i=\frac1{\sqrt{2\pi}}\exp(-\frac{\mathrm{dist}_i^2}{2b^2}),
\end{equation}
where $b$ is the bandwidth of Gaussian kernel, and $\mathrm{dist}$ is the Euclidean distance between the guided point and the underestimated target point. Denote $\boldsymbol{X}$ the homogeneous representation of $\boldsymbol{\hat{D}}_n$, the scale map $\boldsymbol{S}_{scale}$ and shift map $\boldsymbol{S}_{shift}$ of target points can be calculated by iterating every location on the whole image, which can be formulated as:
\begin{equation}
    \begin{gathered}
        \min_{\boldsymbol{\beta}_{u, v}} (\hat{d}_n^* -\boldsymbol{X}\boldsymbol{\beta}_{u,v})^\mathsf{T}\boldsymbol{W}_{u,v}(\hat{d}_n^* -\boldsymbol{X}\boldsymbol{\beta}_{u,v})+\lambda\boldsymbol{S}_{shift}^2, \\
    \boldsymbol{\hat{\beta}}_{u,v}=(\boldsymbol{X}^\mathsf{T}\boldsymbol{W}_{u,v}\boldsymbol{X}+\lambda)^{-1}\boldsymbol{X}^\mathsf{T}\boldsymbol{W}_{u,v}\hat{d}_n^*, \\
    \boldsymbol{\beta_{u,v}} = [\boldsymbol{S}_{scale},\boldsymbol{S}_{shift}]_{u,v} ^ \mathsf{T}, \\
    \boldsymbol{D}_n = \hat{d}_n^* \oplus  \boldsymbol{S}_{scale} \odot \boldsymbol{\hat{D}}_n + \boldsymbol{S}_{shift},
\end{gathered}
\end{equation}

\noindent where $\boldsymbol{D}_n$ is the scaled whole depth map, $\oplus$ is the concatenation operator, $\lambda$ is a $l_2$ regularization hyperparameter used for restricting the solution to be simple. Besides, the explicit constraint of the source frame with the target frames allows each novel view to maintain contextual consistency from preceding generations.

\vspace{4pt}
\noindent \textbf{Novel View Generation.}
After obtaining the aligned depth $\boldsymbol{D}_n$, we generate target visual hints through warping as $\hat{I}_j = \Pi_{n \rightarrow j}(\boldsymbol{D}_n)$. The warped images $\{\hat{I}_j\}_{j=n}^{n+m}$ contain  unfilled regions,  as indicated by the binary warping mask $\{M_j\}_{j=n}^{n+m}$, providing strong visual hints for \ours to perform novel view generation. To ensure strong multi-view consistency between the newly generated sequence and the previous content, we randomly select $k$ anchor views $\{I_k\},k \in [1,N]$ from the earlier generated frames to guide subsequent generation. The generation process is formulated as: $I_j = \ours (\hat{I}_j, M_{j}, \{I_0,I_k\})$.
We iteratively perform depth estimation, alignment, warping, and generation  until all predefined multi-view images are obtained. 

\vspace{4pt}
\noindent\textbf{3D Reconstruction.} \label{sec: 3dgs}
We reconstruct the 3D scene using 3D Gaussian Splatting (3DGS) \cite{3dgs}. 
The training objective is to minimize the sum of photometric loss and SSIM loss, consistent with the original 3DGS approach. Additionally, we introduce a perceptual loss (LPIPS \cite{lpips}) to mitigate subtle \textit{inter-frame} discrepancies in multi-view generated images during 3DGS reconstruction. LPIPS emphasizes higher-level semantic consistency between Gaussian-rendered and generated multi-view images, rather than focusing on minor high-frequency differences.
Furthermore, the potential \textit{inner-frame} diversity may lead to inconsistencies with the corresponding camera poses. Following \cite{fan2024instantsplat}, we implement joint pose-Gaussian optimization, treating camera parameters as learnable variables alongside Gaussian attributes, thereby reducing gaps between generated viewpoints and their corresponding camera poses.




==> arxiv/demo.tex <==
\makeatletter
\let\@oldmaketitle\@maketitle
\renewcommand{\@maketitle}{\@oldmaketitle
\vspace{-0.6cm}
\includegraphics[width=\linewidth]{images/top.pdf}
\centering
\captionsetup{hypcap=false}
\captionsetup{skip=2pt}
\captionof{figure}{ 
Benefiting from the proposed web-scale dataset \data, \ours enables both object- and scene-level 3D creation, including sparse-view-to-3D, (text-) image-to-3D,  and 3D editing. It can also be used for Gaussian Splatting to extract meshes or render images.
\vspace{10pt}
}\label{fig:demo}
}
\makeatother



==> preamble.tex <==
% \usepackage{lineno}
%%
% --- inline annotations
%
% \newcommand{\red}[1]{{\color{red}#1}}
% \newcommand{\todo}[1]{{\color{red}#1}}
% \newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% \newcommand{\uncer}[1]{{\color{blue}#1}}
% \newcommand{\cfer}[1]{{\color{lightpink}#1}}

% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/0_abstract.tex <==
\begin{abstract}
Recent 3D generation models typically rely on limited-scale 3D `gold-labels' or  2D diffusion priors for 3D content creation.  However, their performance is upper-bounded by constrained 3D priors due to the lack of scalable learning paradigms.   
In this work, we present \textbf{\ours}, a visual-conditional multi-view diffusion model trained on large-scale Internet videos for open-world 3D creation.
The model aims to \textbf{Get} \textbf{3D} knowledge by solely \textbf{See}ing the visual contents from the vast and rapidly growing video data --- You See it, You Got it.
To achieve this, we first scale up the training data using a proposed data curation pipeline that automatically filters out multi-view inconsistencies and insufficient observations from source videos. This results in a high-quality, richly diverse, large-scale dataset of multi-view images, termed WebVi3D, containing 320M frames from 16M video clips.
Nevertheless, learning generic 3D priors from videos without explicit 3D geometry or camera pose annotations is nontrivial, and annotating poses for web-scale videos is prohibitively expensive.
To eliminate the need for pose conditions, we introduce  an innovative  \textit{visual-condition} - a purely 2D-inductive visual signal generated  by adding time-dependent noise to the masked video data.
Finally, we introduce a novel visual-conditional 3D generation framework by integrating \ours into a warping-based pipeline for high-fidelity 3D generation. 
Our numerical and visual comparisons on single and sparse reconstruction benchmarks show that \ours, trained on cost-effective and scalable video data, achieves notable zero-shot and open-world generation capabilities, markedly outperforming models trained on costly and constrained 3D datasets. Additionally, our model naturally supports other image-conditioned 3D creation tasks, such as 3D editing, without further fine-tuning.

%Eventually, we unleash the power of  \textit{\ours}  and propose a  novel visual-conditional 3D generation approach by integrating it into a warping-based pipeline for high-fidelity 3D  generation. 


% \textbf{\color{blue}{See}}ing an ever-growing volume of video data, the model aims to gain insights into the underlying  structure of the \textbf{\color{blue}{3D}} world. 
% Training only on videos, the model aims to gain insights into the underlying  structure of the \textbf{\color{blue}{3D}} world. In other words, `see videos, got 3D'. 

%It employs multi-view prediction as a proxy task to learn generic 3D priors, establishing a scalable leaning paradigm for robust 3D creation.
\end{abstract}



% \todo{------Version 1 by baorui-------} 
% In this paper, we present an approach to Novel View Synthesis that improves the generalization of synthesized views involving unseen object types and new scenes. Without pursuing novel technical modules, our goal is to build a powerful base model for creating anything in 3D from single or sparse views. We achieve this by learning 3D priors from easily accessible web-scale video data, predicting consistency multi-views with warping condition. Instead of attempting to scale expensive 3D data, we demonstrate how to leverage pose-free video data from public sources, to enable generalized 3D knowledge.
% We investigate two key issues that make data scaling-up promising. First, video data frequently contains dynamic objects and limited camera movement, leading to inconsistent and incomplete observation of the scene. This issue will introduce dynamic biases and over-reliance on reference images in the model. To overcome this, we carefully designed key strategies to automatically filter suitable data for learning 3D priors from noisy sources. Second, learning precise control of camera movement from video data without pose annotations is challenging. Our approach casts multi-view generation as a multi-view 2D warping-inpainting task, which relies solely on unmasked clues instead of explicit pose conditions to infer camera movement. However, accurately simulating the warping operation on video data without 3D geometric and camera information is difficult. To address this, we propose a time-dependent noise distribution for the warping image during training, applying higher noise levels at larger time steps to disrupt it, followed by a self-supervised backward diffusion process at smaller time steps to reduce the model's dependency on explicit warping for bridging the training-inference gap. Our method shows the potential of using web-scale video data for a scalable and generalized 3D solution.


% \todo {--------Version 2 by lu----------}
% State-of-the-art 3D generation models typically rely on either limited-scale 3D `gold-labels' or  2D diffusion priors for 3D content creation. 
% However, learning from limited 3D data restricts their model generalizability, while leveraging 2D diffusion priors often leads to  3D-inconsistency. 没有一个scalable的范式去学习3D priors.

% In this work, we provide a promising alternative that implicitly learns univerisal 3D priors from large-scale Internet videos. 

% 1） 收集multi-view images 2）

% Empirically, we first validate the effectiveness of Internet videos for scalable 3D generation, and present a systematic solution, including \uncer{a comprehensive 3D-aware video data curation workflow, a novel visual-conditional multi-view diffusion model, and an effective  warping-based novel view synthesis task}. 
% Given limited observations (e.g.,single or sparse views), our model, \textit{\ours}, is capable of generating multiple high-quality, 3D-consistent novel views involving unseen object types and new scenes. These views can subsequently be used for 3D reconstruction, enabling rendering from any viewpoint.
% Evaluation  on the XX and YY datasets showing that \textit{\ours}, trained on easily accessible and  virtually  unlimited video data, exhibits remarkable zero-shot and open-world generation capabilities, significantly outperforming models trained on costly and constrained 3D datasets.
% \end{abstract}

% \todo{------Version 3 ------} 
% We present \textit{\ours}, a scalable multi-view diffusion (MVD) model for 3D generation. 
% Existing 3D generation models typically rely on either limited-scale 3D `gold-labels' or 2D diffusion priors for 3D content creation. Nevertheless, limited 3D data restricts their model generalizability, and using off-the-shelf 2D priors often leads to 3D-inconsistency. 
% Here, we provide a promising alternative that learns 3D priors from scalable and cost-effective Internet videos. Yet, learning generic 3D priors from videos without explicit 3D geometry or camera pose annotations (i.e., pose-free videos) is nontrivial, and pose annotation for web-scale videos is prohibitively expensive.
% To address this, we present \textit{\ours}, a scalable multi-view diffusion (MVD) model trained on Internet videos for 3D generation. Specifically, we first curate \textit{WebVi3D}, a 3D-aware, pose-free video dataset with a total duration of 4.41 GPU years, specifically tailored for training MVD models. 
% % To enable pose-aware conditioning from pose-free videos, we introduce a novel \textit{visual-condition} - a purely 2D-inductive signal created by adding time-dependent noise to the masked input image.
% To eliminate the need for pose condition, we then   introduce a novel \textit{visual-condition} - a purely 2D-inductive signal created by adding time-dependent noise to the masked video data.
% Eventually, we unleash the power of the proposed DreamScaler by integrating it into a warping-based pipeline for high-quality 3D content generation. 
% % We then train the visual-conditional MVD model on \textit{WebVi3D}, and apply it to the warping-based 3D generation task. 
% % We eventually apply the Dreamscaler to the warping-based 3D generation task. 
% % Given limited observations (e.g.,single or sparse views), our model is capable of generating multiple high-quality, 3D-consistent target views involving unseen object types and new scenes, which can be further used for 3D reconstruction, supporting rendering from arbitrary viewpoints.
% Our evaluation of the XX and YY datasets shows that \textit{\ours}, trained on cost-effective and scalable video data, achieves notable zero-shot and open-world generation capabilities, markedly outperforming models trained on costly and constrained 3D datasets. Additionally, \textit{\ours} naturally supports other image-conditioned generation tasks, such as 3D editing, without requiring further fine-tuning.

==> sec/1_intro.tex <==
\vspace{-8pt}

\section{Introduction}
\label{sec:intro}
\vspace{-5pt}
Recent advances in 3D generation are essential for fields like virtual reality, entertainment, and simulation, offering the potential not only to recreate intricate real-world structures but also to expand human imagination.
Nevertheless, developing these models is constrained by the scarcity and high costs of accessible 3D datasets. Despite recent industry efforts \cite{tochilkin2024triposr, zhang2024clay, yang2024hunyuan3d}  create extensive proprietary 3D assets, these initiatives come with substantial financial and operational burdens. Currently, building  such a large-scale 3D dataset for academia remains prohibitively expensive. This motivates us to pursue a scalable, accessible, and affordable data source that can compete with advanced closed-source solutions, thereby enabling the broader research community to train high-performance 3D generation models.


% \vspace{2pt}
Human perception of the 3D world does not rely on specific 3D representation (e.g., point clouds\cite{point}, voxel grids \cite{voxel}, meshes \cite{mesh}, or neural fields \cite{mildenhall2021nerf})  or precise camera conditions. Instead, our 3D awareness is shaped by multi-view observations accumulated throughout our lives. This raises the question:  \textit{Can models similarly learn universal 3D priors from large collections of multi-view images?}  Fortunately, Internet videos offer a rich source of multi-view images, captured from various locations with diverse sensors and complex camera trajectories, providing a scalable, accessible, and cost-effective data source. Thus, \textit{how can we effectively learn 3D knowledge from Internet videos?}


% \vspace{2pt}
% Next token prediction tasks \cite{} employ autoregressive techniques to pre-train models on vast Internet data, enabling them to acquire substantial knowledge in both visual and textual domains. Their success suggests that a similar approach, training multi-view prediction model at scale, can facilitate understanding of 3D knowledge. Meanwhile, diffusion models \cite{} have recently revolutionized image and video generation by using web-scale datasets. \uncer{ Motivated by these advancements, our objective is to develop  a scalable multi-view diffusion (MVD) model for open-world 3D generation using Internet videos.}

% \vspace{2pt}
The core challenges in achieving this goal are twofold: 1) filtering relevant, 3D-aware video data from raw sources, specifically static scenes with varied camera viewpoints that provide sufficient multi-view observations; and 2) learning generic 3D priors from videos lacking explicit 3D geometry and camera pose annotations (i.e. pose-free videos). This work carefully addresses these challenges and  introduces a pose-free, visual-conditional multi-view diffusion (MVD) model, \textit{\ours}, for open-world 3D creation.


% selects 3D-aware videos by leveraging priors from instance segmentation \cite{maskrcnn}, optical flow \cite{raft}, and pixel tracking \cite{cotracker} . This pipeline 
% \vspace{2pt}
Specifically, we establish a novel video data curation pipeline that automatically filters out  data with dynamic content or restricted camera viewpoints from source videos.
The resulting dataset, termed WebVi3D, comprises 15.99M video clips from 25.48M source videos, totaling 4.41 years in duration—orders of magnitude larger than previous 3D datasets, such as DLV3D (0.01M) \cite{ling2024dl3dv}, RealEstate10K (0.08M) \cite{real10k}, MVImgNet (0.22M) \cite{yu2023mvimgnet} and Objaverse (0.8M) \cite{deitke2023objaverse}.

% \vspace{2pt}
% MVD models inherit the generative capabilities of 2D diffusion models while modeling multi-view correlations. With advantages in both generalizability and 3D-consistency, they have been widely studied for 3D generation \cite{shi2023mvdream,liu2023syncdreamer}. 
% Typically, these models rely on precise camera poses as conditional inputs \cite{shi2023mvdream,gao2024cat3d,hong2023lrm,liu2023zero, muller2024multidiff}  to guide 3D-consistent view generation. Alternatively, some approaches employ warped images rendered from ground-truth 3D assets to indicate camera movements\cite{yu2024viewcrafter,tung2024megascenes}. 
MVD models have recently gained  widespread attention due to their advantages of integrating the generative capabilities of 2D diffusion models while maintaining consistency across multiple views \cite{shi2023mvdream,liu2023syncdreamer}.
Typically, these models rely on precise camera poses \cite{shi2023mvdream,gao2024cat3d,hong2023lrm,liu2023zero, muller2024multidiff} or warped images rendered according to camera position \cite{yu2024viewcrafter,tung2024megascenes} as conditional inputs to guide 3D-consistent view generation. We refer to these conditions, derived from pose or 3D annotations, as 3D-inductive conditions.  
However, annotating web-scale videos is prohibitively costly, or even intractable in some  cases, posing significant challenges for scaling. 
To address this, we propose a novel, pose-free \textit{visual-condition} derived from pixel-space hints within videos.  It is a purely 2D-inductive visual signal, created by introducing \textit{time-dependent noise} to masked input videos, free from any 3D-inductive bias. This enables training  MVD model at scale, without requiring pose annotations.

% \vspace{2pt}
% \todo{Ultimately, we integrate the proposed model into a warping-based pipeline, and introduce a novel visual-conditional 3D generation framework.}

% \todo{Finally, we propose a novel multi-view generation pipeline that builds comprehensive scene observation by iteratively refining the geometry of novel views and constructing visual conditions for multi-view generation by \ours. These generated images are fed into a robust 3D Gaussian Splatting reconstruction to produce corresponding 3D Gaussians that can render arbitrary viewpoints.}

% As anticipated, \textit{\ours}  exhibits the potential to adapt to tasks that use \textit{pixel-space} hints differing from those in videos, without requiring additional training. For instance, in warping-based 3D generation tasks \cite{chung2023luciddreamer,shriram2024realmdreamer}, pixels from a reference image are rearranged through warp operations, serving as a \textit{specific} visual-condition to indicate camera movement. However, warped images often suffer from artifacts or distortions, leading to a significant domain gap compared to real video frames. Whereas, our \textit{visual-condition} functions as a \textit{generic} visual-condition, capable of accommodating such unnatural images. Similarly, it can naturally generalize to 3D editing tasks \cite{} where the masked image acts as another form of \textit{specific} visual-condition.  In this paper, \todo{we primarily focus on warping-based 3D generation as a representative application, with a basic verification for 3D editing task included in the Appendix. }

%我们的visual-condition sever as a general condition, 可以naturally支持那些与video 图片不一样的其他任务， 比如warp-based 3D generation 以及3D editing。 Take warp-based 3D generation for example, 巴拉巴拉----> warped image is a \textit{specific} visual-condition----> 我们的visual-condition 可以包容 warped image这类unnatural的图片。  
% 为了进一步unleash the power of DreamScaler , we introduce a novel warping-based multi-view generation framework.  where we first construct \textit{visual-condition} by \textit{\ours}, then we build comprehensive scene observation by iteratively refining the geometry of predicted views.  These generated images are finally fed into a robust 3D Gaussian Splatting reconstruction to produce corresponding 3D Gaussians that can render from arbitrary viewpoints.


Intuitively, the proposed \textit{ visual-condition} can generalize effectively  to tasks that rely on pixel-space hints distinct from those in videos, such as warping-based 3D generation \cite{chung2023luciddreamer,shriram2024realmdreamer} and mask-based 3D editing \cite{chen2024gaussianeditor}, without requiring additional training, see \cref{fig:demo}.  For instance, in warping-based 3D generation, pixels from a reference image are rearranged through warping operations, creating a \textit{specific} visual-condition to indicate camera movement. However, these warped images often exhibit artifacts or distortions, causing a significant domain gap compared to video frames. Whereas, our \textit{visual-condition} functions as a \textit{generic} one, capable of accommodating such unnatural images. 



% \todo{Finally, we propose a novel multi-view generation pipeline that builds comprehensive scene observation by iteratively refining the geometry of novel views and constructing visual conditions for multi-view generation by \ours. These generated images are fed into a robust 3D Gaussian Splatting reconstruction to produce corresponding 3D Gaussians that can render arbitrary viewpoints.}


% \vspace{4pt}
To further harness the potential  of \ours, we introduce an innovative visual-conditional 3D generation framework utilizing  a warping-based pipeline. This framework first constructs the \textit{visual-condition} using  \ours, then iteratively refines the geometry of novel views to build comprehensive scene observations. Finally, the generated images are used for Gaussian Splatting reconstruction \cite{3dgs,huang20242d}, which can be rendered from arbitrary viewpoints or converted into meshes through post-processing \cite{lorensen1998marching}.
In summary, our key contributions are as follows.

\begin{itemize}

\item We present \ours, a scalable visual-conditional MVD model for open-world 3D creation, which can be trained on web-scale video collections without pose annotations.

\item We curate WebVi3D, a multi-view images dataset containing static scenes with sufficient multi-view observations, and establish an automated pipeline for video data curation to train the MVD model. 

\item We introduce a novel warping-based 3D generation framework with \ours, which supports long-sequence generation with complex camera trajectories. 
% supporting both object- and scene-level 3D reconstruction 
% 轨迹更复杂，long sequence view generation. 
\item  We achieve state-of-the-art results in single and sparse views reconstruction, demonstrating remarkable zero-shot and open-world generation capability, offering a novel perspective on scalable 3D generation.
\end{itemize}


\begin{figure*}[tb]
\centering
\includegraphics[width=0.8\linewidth]{images/training4.pdf}
\vspace{-10pt}
\caption{\small \textbf{Overview of \ours.}
(a) We propose a four-step data curation pipeline to select multi-view images from Internet videos, forming the WebVi3D dataset, which includes $\sim$16M video clips across  diverse categories and concepts. 
(b) Given multiple views, we corrupt the original data into corrupted images $c_{t}^{i}$
at timestep $t$ by applying random masks and time-dependent noise. We then reweight the guidance of  $c_{t}^{i}$ and the noisy latent $x_{t}^{i}$ for the diffusion model to form  \textit{ visual-condition} $v_{t}^{i}$ through a time-dependent mixture. 
(c) MVD model is capable of training at scale to generate multi-view images conditioned on $v_{t}^{i}$, without requiring pose annotations. Since $v_{t}^{i}$ is a task-agnostic visual signal formed through time-dependent noise  and mixture,  it enables the trained model to robustly adapt to various  downstream tasks.}
\vspace{-17pt}
\label{fig:trainpipe}
\end{figure*}
% (a) We We propose four strategies to 从互联网video中筛选多视角图片，集合成数据集WebVi3D，resulting in 16M clips that encompass diverse categories and concepts. (b) 给定一个多视图序列，我们通过随机mask和time-dependent noise addition操作将原始数据破坏为noisy images C_t, 根据timestep t。Via time-dependent mixture, We reweight the level of guidance of noisy latent X_t and noisy images C_t for the diffusion model based on timestep t, denoted as visual-condition. (c) 我们训练MVD model to generate multi-views conditioned on visual-condition. Visual-condition不需要pose标注，通过time-dependent noise and mixture形成任务无关的视觉信号，从而可以让训练好的MVD model鲁棒性的适应各种下游任务。




















% \textbf{Specifically}, to filter useful 3D-aware video data and make data scaling promising, \todo{We propose a sophisticated data selection pipeline that utilizes pre-trained instance semantic segmentation \cite{}, optical flow \cite{} and pixel-tracking \cite{} prior to filter out interfering data in the presence of dynamic content and camera viewing angles that are too small in a coarse-to-fine manner.} As a result, we curate approximately 23M video clips with a total duration of 4.41 GPU years for training MVD model, an order of magnitude larger than previous 3D datasets, \todo{like RealEstate10K (XX M)\cite{}, Tanks and Temples (XX M)\cite{}, DLV3D (XX M)\cite{}.}  We refer to our curated dataset as WebVi3D (Videos for Novel View Synthesis).
% It achieves both good consistency and generalizability, providing a robust multi-view  prior for 3D generation tasks. 
%Empirically, we first validate the effectiveness of Internet videos for 3D generation, and present a systematic exploration that includes \uncer{ a detailed 3D-aware video data curation pipeline, a novel visual-conditioned  MVD model, and an effective warping-based 3D generation task}, as illustrated in Fig.1. Conditioned on limited observations (e.g., single or sparse views), our method is capable of generating multiple high-quality, 3D-consistent novel views of objects or scenes. These generated views facilitate robust 3D reconstruction,  allowing rendering from any viewpoint.

==> sec/1_intro_v0.tex <==
\section{Introduction}
\label{sec:intro}


\todo{Red: todo-------------------;} \uncer{Blue: uncertain------------------;}

\noindent \todo{Definitions:  \{1. Model name; 2. pseudo-3D-video data ?; 3.Unstructured internet videos; 4. Pose-free video; 5.Time-dependent noise distribution; 6. The first to do mixed dataset training\}}


The generation of 3D content has gained increasing significance across a range of applications, such as gaming, virtual reality, and film production.......


\textbf{State-of-the-art} 3D generation approaches generally fall into two categories:
1) Learning generative models from 3D datasets, where expensive 3D annotations, such as 3D representations (e.g. point clouds, volumes, meshes or neural fields) \cite{} or precise camera conditions are provided \cite{}. With explicit 3D priors, these models can better understand and preserve geometric features. However, the dependence on costly and limited-scale 3D datasets hinders their ability to generalize effectively in open-world or highly imaginative scenarios. 
2) Lifting 2D generation into 3D \cite{}, where methods optimize 3D representations using 2D diffusion priors through intricate optimization techniques like score distillations \cite{}.  Yet 2D priors do not readily translate into coherent 3D representations, methods based on 2D generation often struggle to preserve high geometric fidelity, leading to issues such as multi-view inconsistency and poor global geometry.

\textbf{In this work}, we aim to develop a scalable 3D generation model. 
However, constructing a web-scale 3D dataset is prohibitively expensive and currently impractical.
Inspired by large vision foundation models (e.g., CLIP\cite{}, EVA-CLIP\cite{}), which have demonstrated the power of web-scale text supervision in enhancing visual representations, we pose a compelling question: \uncer{can 3D generation models benefit from large, diverse, and readily  accessible internet data sources?}
To explore this, we introduce \textit{DreamScaler}, a novel view synthesis approach that trains a multi-view diffusion (MvD) model on  internet videos, effectively mitigating the issue of 3D data scarcity while ensuring both generalizability  and multi-view consistency. % in the generated content.

\textbf{The core challenges}  in  achieving this goal are two-fold:   
1) \textit{filtering useful pseudo-3D-video data} (i.e., videos with static scenes and varied camera viewpoints that provide  sufficient multi-view information)  from raw source videos;
and 2) \textit{learning 3D priors on pose-free videos} (i.e., videos without explicit 3D geometric or camera pose information).  
This work comprehensively addresses these challenges by introducing \uncer{a detailed pseudo-3D-video data curation workflow and a scalable MvD training framework}, aiming to offer a robust and generalized alternative for 3D solution.

% \todo{[Data curation----Warping Simulation---Blending]}  
\textbf{Specifically}, to filter useful pseudo-3D data and make data scaling promising, \todo{we [describe the difficulties and solutions?].} As a result, we curate approximately 2M high-quality training data, an order of magnitude larger than previous 3D datasets, \todo{like XX (?M), YY(?M).}

To learn 3D knowledge from  pose-free videos, we cast multi-view generation as a multi-view 2D warping-inpainting  task that depends solely on visible visual cues, without explicit camera pose conditions.
A key technical challenge in this task arises from training the MvD model on normal view images while  inferring only conditioned on warped images, leading to an out-of-distibution (ODD) problem.
To address this, we introduce a \textit{time-dependent noise distribution} for the warping process during training, applying higher noise at larger time steps and lower noise at smaller ones. This strategy  effectively reduces the model's reliance on explicit warping, bridging the training-inference gap.

Empirically, we first validate the effectiveness of internet videos for 3D content generation, and present a systematic solution that includes \uncer{ a comprehensive pseudo-3D-video data curation process, a novel video-based MvD training framework, and an effective multi-view 2D warping-inpainting learning task}, as illustrated in Fig.1. Conditioned on limited observations (e.g., single or sparse views), our model is capable of generating multiple high-quality, 3D-consistent novel views. These generated views can subsequently be utilized for 3D reconstruction, enabling rendering from any viewpoint.
In summary, our \textbf{key contributions} are as follows:

\begin{itemize}
% \item We build the first billion-scale 3D foundation generative model, \textit{DreamScaler}, which can be trained on extensive  and diverse video collections. 

\item We present a novel view synthesis approach, \textit{DreamScaler}, trained on internet videos, which improves the generalization of synthesized views for unseen object types and novel scenes.

\item We curate 20M pseudo-3D data from internet videos, establishing a detailed and scalable video data curation workflow for training 3D generation models. 
\item \uncer{We train multi-view diffusion at scale by casting 3D generation as a multi-view 2D warping-inpainting task. }
\item  We achieve state-of-the-art results on XX and YY, demonstrating remarkable zero-shot and open-world generation capability. %, offering a new perspective on learning scalable 3D generation models using internet videos.

\end{itemize}




% In response to these challenges, our approach innovatively leverages web-scale pose-free video data to train MvD models. We prepare a large-scale dataset, an order of magnitude larger than previous 3D datasets, and design a multi-view 2D warping-inpainting task to ensure view consistency. Additionally, we introduce a time-dependent noise distribution in our training framework to improve the model's ability to learn cross-view dependencies. By combining video and 3D data, we significantly reduce reliance on curated 3D datasets and create a scalable training framework.
% As a result, our method demonstrates state-of-the-art performance in synthesizing novel 3D views. It showcases superior scalability and generalization capabilities, effectively addressing the limitations of previous approaches. Our model not only mitigates the issue of 3D data scarcity but also opens new avenues for utilizing internet videos to enhance 3D content generation, providing valuable insights for future research

==> sec/2_related_work.tex <==
\vspace{-5pt}
\section{Related work}
\vspace{-5pt}
\label{sec:related_work}

% \noindent \textbf{Lifting 2D Generation into 3D.} Recent advances in 3D generation have been largely driven by the success of 2D diffusion models \cite{sohl2015deep,song2020denoising,ho2020denoising,rombach2022high}, which have revolutionized image and video generation. These works typically optimize 3D representations by maximizing the likelihood evaluated by 2D diffusion priors \cite{poole2022dreamfusion,latentnerf,tang2023dreamgaussian,wang2024prolificdreamer,kim2023collaborative,lin2023magic3d, yi2023gaussiandreamer, sun2023dreamcraft3d,12345}. 
% An alternative approach uses  a warping-inpainting pipeline, integrating an offline depth estimator with a 2D diffusion-based inpainting model to iteratively generate 3D content \cite{chung2023luciddreamer, engstler2024invisible, yu2024wonderworld,yu2024viewcrafter,muller2024multidiff,hollein2023text2room,wang2024vistadream}.
% However, 2D priors do not readily translate into coherent 3D representations. As a result, 2D lifting-based approaches often struggle to preserve high geometric fidelity, leading to issues like multi-view inconsistency and poor global geometry \cite{yu2024wonderjourney}. 

% \noindent \textbf{Directly Learning 3D Priors.}
% To better preserve geometric features, some works focus on directly learning 3D priors. For instance, feed-forward approaches \cite{hong2023lrm,gupta20233dgen, pflrm,mvlrm,wei2024meshlrm,longlrm,tochilkin2024triposr,tang2025lgm,xu2024instantmesh,xu2024grm,shen2024gamba,lu2024large,triplanegaussian,splatter,liu2025mvsgaussian,chen2025mvsplat,charatan2024pixelsplat,instant3d} take single/few views as input and directly output 3D representations using an encoder-decoder architecture, eliminating the need for additional optimization process per instance. Another line of research involves training diffusion models to predict 3D representations, such as point clouds \cite{lcm,pointe}, mesh \cite{lyu2023controllable,alliegro2023polydiff,shapee}, and implicit neural representation \cite{ma2024shapesplat, ssdnerf,wu2024direct3d,zhang2024clay}. 
% However, these methods generally focus on object-level generation \cite{deitke2023objaverse,wu2023omniobject3d,tang2025lgm,triplanegaussian,zhang2024clay}, limiting their applicability to scene-level generation. Although recent research has made strides in building scene-level 3D datasets  \cite{knapitsch2017tanks,ling2024dl3dv,barron2022mipnerf360,dai2017scannet}, their scale remains relatively limited. The reliance on costly, limited-scale 3D datasets restricts  generalization to open-world or highly imaginative scenarios. 
% In contrast, our approach  curates a large-scale, richly diverse dataset of multi-view images from Internet videos. By training the model at scale, it effectively supports both object-level and scene-level 3D creation. 

% \noindent \textbf{Learning Multi-view Priors for 3D Generation. }
% MVD  model inherits  the generative capabilities of 2D diffusion models while capturing multi-view correlations, achieving both generalizability and 3D consistency.  These merits have made it a focal point in recent 3D generation research \cite{shi2023mvdream,shi2023zero123++,12345++,yu2024viewcrafter, wang2023imagedream,long2024wonder3d,liu2023syncdreamer,han2025vfusion3d,qiu2024richdreamer,sargent2023zeronvs,gao2024cat3d}. 
% However, as 2D diffusion models are typically  trained on 2D datasets, they lack precise control over image pose.
% To address this, MVD-based approaches often  train their models on images paired with camera poses \cite{watson2022novel,liu2023zero,sargent2023zeronvs, wu2024reconfusion,gu2023nerfdiff}, where poses serve as  essential conditional inputs, represented by camera extrinsics \cite{sargent2023zeronvs,shi2023mvdream}, relative poses \cite{liu2023zero,shi2023zero123++,liu2023syncdreamer}, or Plücker rays \cite{gao2024cat3d,xu2024camco}. Yet, pose-conditional models  rely heavily on costly pose-annotated data, restricting training to smaller 3D datasets, thereby constraining their adaptability to out-of-distribution scenarios.
% In contrast, we introduce a  novel visual-conditional approach   that supports scalable, pose-free MVD model training for open-world 3D generation. 


Some works focus on directly learning 3D priors. For instance, feed-forward approaches \cite{hong2023lrm,gupta20233dgen, pflrm,mvlrm,wei2024meshlrm,longlrm,tochilkin2024triposr,tang2025lgm,xu2024instantmesh,xu2024grm,shen2024gamba,lu2024large,triplanegaussian,splatter,liu2025mvsgaussian,chen2025mvsplat,charatan2024pixelsplat,instant3d} take single/few views as input and directly output 3D representations using an encoder-decoder architecture, eliminating the need for additional optimization process per instance. Another line of research involves training diffusion models to predict 3D representations, such as point clouds \cite{lcm,pointe}, mesh \cite{lyu2023controllable,alliegro2023polydiff,shapee}, and implicit neural representation \cite{ma2024shapesplat, ssdnerf,wu2024direct3d,zhang2024clay}. 
However, these methods generally focus on object-level generation \cite{deitke2023objaverse,wu2023omniobject3d,tang2025lgm,triplanegaussian,zhang2024clay}, limiting their applicability to scene-level generation. Although recent research has made strides in building scene-level 3D datasets  \cite{knapitsch2017tanks,ling2024dl3dv,barron2022mipnerf360,dai2017scannet}, their scales remain relatively limited. The reliance on costly, limited-scale 3D datasets restricts  generalization to open-world or highly imaginative scenarios. 
In contrast, our approach  curates a large-scale, richly diverse dataset of multi-view images from Internet videos. By training the model at scale, it effectively supports both object-level and scene-level 3D creation. 
\textbf{Another parallel research direction, MVD}  model inherits  the generative capabilities of 2D diffusion models while capturing multi-view correlations, achieving both generalizability and 3D consistency.  These merits have made it a focal point in recent 3D generation research \cite{shi2023mvdream,shi2023zero123++,12345++,yu2024viewcrafter, wang2023imagedream,long2024wonder3d,liu2023syncdreamer,han2025vfusion3d,qiu2024richdreamer,sargent2023zeronvs,gao2024cat3d}. 
However, as 2D diffusion models are typically  trained on 2D datasets, they lack precise control over image pose.
To address this, MVD-based approaches often  train their models on images paired with camera poses \cite{watson2022novel,liu2023zero,sargent2023zeronvs, wu2024reconfusion,gu2023nerfdiff}, where poses serve as  essential conditional inputs, represented by camera extrinsics \cite{sargent2023zeronvs,shi2023mvdream}, relative poses \cite{liu2023zero,shi2023zero123++,liu2023syncdreamer}, or Plücker rays \cite{gao2024cat3d,xu2024camco}. Yet, pose-conditional models  rely heavily on costly pose-annotated data, restricting training to smaller 3D datasets, thereby constraining their adaptability to out-of-distribution scenarios.
In contrast, we introduce a  novel visual-conditional approach   that supports scalable, pose-free MVD model training for open-world 3D generation. 





%, effectively supporting 3D content creation with both generalizability and multi-view consistency.





==> sec/3_method.tex <==
\vspace{-10pt}
\section{Method}
\vspace{-5pt}
The primary objective of this work is to build a robust 3D generative model from the perspective of dataset scaling-up.
Previous works \cite{deitke2023objaverse, tung2024megascenes,reizenstein2021common} laboriously collect 3D data from designed artists, stereo matching, or Structure from Motion (SfM), which are often costly and in some cases, infeasible.   In contrast, multi-view images offer a highly scalable alternative, as they can be automatically extracted from the vast and rapidly growing Internet videos. Using multi-view prediction as a pretext task, we show that learned 3D priors enable a range of 3D creation applications, such as single view generation, sparse views reconstruction, and 3D editing in open-world scenarios. The following sections outline our approach (Fig.\ref{fig:trainpipe}). Sec.\ref{sec:data} details the data curation pipeline, Sec.\ref{sec:model} introduces visual-conditional multi-view diffusion model, and Sec.\ref{sec:3DGen} demonstrates a new visual-conditional 3D generation framework.

% In the following sections, we outline our approach (\cref{fig:trainpipe}). \cref{sec:data} details the data curation pipeline, which selects static scenes with sufficient multi-view observations from raw video footage. \cref{sec:model} introduces our visual-conditional multi-view diffusion model, which effectively learns general 3D priors from pose-free videos. Finally, \cref{sec:3DGen} demonstrates a new visual-conditional 3D generation framework utilizing  a warping-based pipeline.


\vspace{-7pt}
\subsection{Video Data Curation} \label{sec:data}
\vspace{-6pt}
High-quality, large-scale video data rich in 3D knowledge is essential  for learning  accurate and reliable 3D priors. 
A well-defined 3D-aware video clip should exhibit two key properties: \textbf{a) temporally static scene content } and \textbf{ b) large viewpoint variation caused by the camera's ego-motion.} 
The first property ensures consistent 3D geometry across different viewpoints, while the dynamic content alters the scene’s geometry, introduces biases that may degrade generation performance (see \cref{fig:data}a-Row1). The second property ensures sufficient 3D observations from multiple viewpoints. If the model is trained on videos with limited viewpoint variation (see \cref{fig:data}a-Row2), it may focus primarily on views adjacent to the reference view, rather than developing a comprehensive 3D understanding.


To obtain a massive volume of 3D data, we collect approximately  \textbf{25.48M} open-sourced raw videos, totaling \textbf{44.98 years} from the Internet, covering a wide range of categories, such as landscapes, drones, animals, plants, games, and actions. Specifically, our dataset is sourced from four websites: Pexels \cite{pexels}, Artgrid \cite{artgrid}, Airvuz \cite{airvuz}, and Skypixel \cite{skypixel}. We follow Emu3 \cite{wang2024emu3} to split the videos with PySceneDetect \cite{pyscene} to identify content changes and fade-in/out events. Additionally, we remove clips with excessive text using PaddleOCR \cite{paddle}. The detailed composition of our WebVi3D dataset is presented in \cref{tab:data_stat}.


\begin{table}[ht]
\vspace{-10pt}
\centering
\resizebox{0.44\textwidth}{!}{
\begin{tabular}{c|c|cc|ccc}
\toprule
Website   & Domain    & \# Src. Vids     & Total Hrs.   &\#Fil. Vids   &\#Fil. Clips & Fil. Hrs. \\ \midrule
Pexels   & Open      &  6.18M                & 101.77K          & 0.61M    & 2.65M        & 9.96K             \\
Artgrid  & Open      & 3.94M               &  92.49K            &  0.54M     &  1.10M       & 8.77K      \\
Airvuz   & Drone Shot    &  5.10M                &  94.75K          &  0.54M      &  5.87M   & 8.72K                    \\
    Skypixel & Landscape & 10.27M          &   105.47K            & 0.61M      & 6.37M     & 8.82K                 \\ \midrule
  \textbf{Total}    & Open    & 25.48M         & 394.48K                & \textbf{2.30M  }    & \textbf{15.99M  }          & 36.27K  \\
\bottomrule
\end{tabular}
}
\vspace{-6pt}
\caption{\textbf{WebVi3D Dataset}. Sourced from four open websites, we curate  $\sim$2.30M videos, which are divided into 15.99M clips featuring temporally static scenes with large-range viewpoint.}
\vspace{-10pt}
\label{tab:data_stat}
\end{table}

% \vspace{2pt}
However, identifying 3D-aware videos presents a nontrivial challenge.
Since most videos are derived from real-world footage, such videos often contains dynamic scenes or  small camera movement. 
To address this, we propose a sophisticated pipeline to automatically select relevant, high-quality 3D data  by leveraging priors from instance segmentation \cite{maskrcnn}, optical flow \cite{raft}, and pixel tracking \cite{cotracker}. This pipeline consists of four core steps: 1) Temporal-Spatial Downsampling, 2) Semantic-Based Dynamic Recognition, 3) Non-Rigid Dynamic Filtering, and 4) Tracking-Based Small Viewpoint Filtering. The detailed curation pipeline can be found at Appendix.

Finally, we curate approximately 320M multi-view images from 15.99M video clips with static content and sufficient multi-view observations (see Fig.\ref{fig:data}b). To better validate the effectiveness of our data acquisition method, we randomly select 10,000 video clips for human annotation, of which 8,859 were labeled as 3D-aware, representing 88.6\% of the total. This indicates that our pipeline effectively filtered 3D videos from massive video data. As the volume of Internet videos continues to grow, we can continually use this pipeline to acquire more 3D data, thereby expanding our data support over time.


\begin{figure}[tb]
\centering
\includegraphics[width=0.44\textwidth]{images/data3.pdf}
\vspace{-14pt}
\caption{\small(a-Row1): Dynamic content alters scene geometry across views; (a-Row2): Limited camera movement provides insufficient multi-view observations; (b) Our \data comprises with static scenes and diverse camera trajectories.} 
\vspace{-19pt}
\label{fig:data}
\end{figure}
 
\vspace{-5pt}
\subsection{Visual-conditional Multi-View Diffusion Model} \label{sec:model}
\vspace{-5pt}
\paragraph{Preliminary.}
Diffusion models \cite{sohl2015deep,song2020denoising,ho2020denoising} operate by perturbing the training data $X_0 \sim  q(X_0)$ through a forward diffusion process and learning to reverse it. The forward diffusion process $X_t \sim q_{t|0}(X_t | X_0)$ can be formally represented by $X_{t} = \sqrt{\bar{\alpha}_{t}} \mathbf{X}_0 + \sqrt{1 - \bar{\alpha}_{t}} \boldsymbol{\epsilon}, \quad \boldsymbol{\epsilon} \sim \mathcal{N}(0, \mathbf{I})$, where $\bar{\alpha}_{t}$ is variance schedule used in noise scheduler. In theory, $X_t$ approximates an isotropic Gaussian distribution for sufficiently large timesteps $t$. The training objective is to learn the reverse process. 

\noindent\textbf{Objective.} We aim for multi-view prediction: generating novel views along specified camera trajectories from a single or sparse input, while ensuring consistency with the input appearance. 
MVD model inherits the generalizability of 2D diffusion model while capturing cross-view consistency, which naturally aligns with our goal.  Following this line, we present \textit{\ours}, a pose-free, visual-conditional MVD model trained on Internet videos to enable robust 3D generation, as shown in  Fig.\ref{fig:trainpipe}.

% \paragraph{Challenge.}
\noindent\textbf{Challenge.} The main technical challenge lies in learning precise camera control from pose-free videos. 
Previous works commonly incorporate camera parameters for both input and target views into diffusion models to guide multi-view generation from specified viewpoints. However, training these models generally requires expensive 3D data with precise camera pose annotations, which limits scalability. 
To address this,  we explore an alternative approach that conditions on 2D-inductive visual hints to implicitly control camera movement during training, thereby avoiding the need for hard-to-obtain camera trajectories. 
% \paragraph{Formulation.}

\noindent\textbf{Formulation.} Formally, we propose training the MVD model conditioned on 2D-inductive visual signals, referred to as \textit{visual-condition}, without incorporating  camera parameters. This task can be formulated as designing a conditional distribution, achieved by a conditional diffusion model that minimizes:
\vspace{-5pt}
\begin{equation}
\label{eq:loss}
\mathbb{E}_{X_0, Y_0, \epsilon, t} \left[ \left\lVert \epsilon_{\theta}(X_t, Y_0, V, t) - \epsilon \right\rVert_2^2 \right],
\vspace{-5pt}
\end{equation}
where $X_t$ denotes the noisy latent as mentioned in \cref{sec:model}. Here  $X_0=\left \{ x_{0}^{i}  \right \} _{i=1}^{N}$ represents a multi-view observation of 3D content, formed by sampling one clip from  \textit{\data}  as described in Section \ref{sec:data}, with $N=S+L$ being the number of frames in each clip.  
From $X_0$, $S$ frames are randomly selected as reference view(s), denoted  $Y_0=\left \{ y_{0}^{i}  \right \} _{i=1}^{S}$,  while the remaining $L$ frames are treated as target images, denoted  $G=\left \{ g^{i}  \right \} _{i=1}^{L}$. Our approach focuses on constructing the \textit{visual-condition} $V$, which guides the diffusion model to generate plausible 3D content estimates from target viewpoints consistent with the appearance of $Y_0$. 

% \subsubsection{ Time-dependent Visual Condition} 
% \paragraph{\todo{Principle of Visual-condition.}}
\noindent\textbf{Principle of \textit{Visual-condition}.}
A desirable \textit{visual-condition} should satisfy  the following criteria: a) it can be constructed without the need for additional 3D annotations, b) it is independent of specific downstream tasks, and c) it offers sufficient generalization to support various task-specific visual conditions, enabling precise control of camera movements.

% \vspace{2pt}
Ideally, this \textit{visual-condition} can be derived  from  pixel-space hints within the original videos, implicitly guiding the model to learn camera control.
Moreover, it should be robust enough to handle domain gaps between task-specific visual cues and pixels extracted from video data.
For example, in warping-based generation, warped images often suffer from issues like self-occlusions, artifacts, and distortions, creating a significant gap compared to real video data as shown in Fig.\ref{fig:single-3d} and Fig.\ref{fig:Vt-ablation}. Based on this, we propose constructing the \textit{visual-condition} by applying masks and noise to the input video data. Our design principles are: 
\begin{itemize}
\item \textbf{Masking}: Corrupting video data through random masking reduces reliance on direct pixel-space visual signals, helping the model partially mitigate the domain gap between task-specific visual cues and video data. 
\item \textbf{Noise Addition}: Adding noise to video data to approximate a Gaussian distribution. When applied to different downstream tasks, task-specific visual inputs are similarly noised, aligning their distribution with a Gaussian profile, and further bridging  the gap between video data and task-specific input.
\end{itemize}

\noindent\textbf{Time-dependent Visual Condition.} We initially add noise and random irregular masks to video data, creating what we call `corrupted' video data $C_t$, as defined in Eq.\ref{eq:ct}. This corrupted data is then used as the \textit{visual-condition} for MVD model training.
A key challenge of this strategy lies in determining the appropriate level of perturbation. If too much noise is added, the conditional signals become ineffective, resulting in poor visual quality and inaccurate camera control. Conversely, if insufficient noise is added, the corrupted data retains substantial details from the target images, causing the model to overly rely on visual hints from video data.

To overcome this, we further introduce a \textit{time-dependent noise} distribution applied to video data. The core idea is to apply higher noise levels at larger time steps, effectively disrupting video data to prevent over-reliance on it.
As the time step decreases, the noise level is reduced, providing cleaner conditional signals to facilitate content generation.
However, as the noise level decreases, the risk of information leakage increases, causing the distribution to deviate from a Gaussian distribution.
To mitigate this, we propose gradually replacing corrupted data $C_t$ with noisy latent $X_t$ as the \textit{visual-condition} 
 (see Eq.\ref{eq:mix}) , encouraging the model to primarily rely on $X_t$ for generation while minimizing dependence on pixel-space signals from video data as timestep decreases. Additionally, $X_t$ is predicted by model and thus exhibits task-agnosticity, as formalized by:
\begin{equation} \label{eq:ct}
C_{t} = \sqrt{\bar{\alpha}_{t'}} (1-M)\mathbf{X}_0 + \sqrt{1 - \bar{\alpha}_{t'}} \boldsymbol{\epsilon}, \quad \boldsymbol{\epsilon} \sim \mathcal{N}(0, \mathbf{I})
\end{equation}
\begin{equation} \label{eq:mix}
V_t=[W_t\ast C_t+  \left ( 1-W_t \right ) \ast X_t;M],
\end{equation}

\noindent where $M = \left\{  m^{0:S} \cup m^{S+1:N} \right \}$, with $m^{0:S}$ as the zero matrix, keeping the reference images $Y_0$ unmasked, and $m^{S+1:N}$ as random irregular masks applied to the target images $G$. $t'=f(t)$, function $f$ is strictly monotonically increasing and requires $t' < t$, which guarantees that $C_t$ contains at least as much information as $X_t$ at earlier timesteps. Here, $\bar{\alpha}_{t'}$ are variances used in DDIM \cite{song2020denoising},  and $V_t=\left \{ v_{t}^{i}  \right \} _{i=1}^{N}$ represents our final \textit{ visual-condition}, which is a mixture of $C_t$ and $X_t$, concatenated with masks $M$ along the channel dimension.  Consequently, Eq.\ref{eq:loss} can be reformulated as $\mathbb{E}_{X_0, Y_0, \epsilon, t} \left[ \left\lVert \epsilon_{\theta}(X_t, Y_0, V_t, t) - \epsilon \right\rVert_2^2 \right]$. 
In practice, an additional processing step assigns $v_{t}^{0:S}$ to the reference images $Y_0$ directly, in order to inject the clean information of $Y_0$ into the model, facilitating alignment between the predicted images and the reference images.
The term $W_t$ represents a balancing weight that decreases monotonically with timestep $t$, ranging from 1 to 0. 

\noindent\textbf{Model Architecture.}
Our model architecture is based on video diffusion model \cite{svd}. However, we removed the time embedding, as we aim for the model to control the camera movement purely through visual conditions, rather than inferring movement trends based on temporal cues. To further minimize the effect of temporality, we shuffle the frames in each video clip, treating the data as unordered $X_0$. 
Specifically,  we randomly select a subset of frames from a video clip as reference images, with the remaining frames as target images. The number of reference images is randomly selected to accommodate different downstream tasks.  The multi-view diffusion model is optimized by calculating the loss only on the target images, as described in Eq.\ref{eq:loss}. For details on the model architecture, such as design of self-attention layers, Zero-Initialize, trainable parameters, noise schedule and cross-attention, please refer to the Appendix.


\vspace{-5pt}
\subsection{Visual Conditional 3D Generation} \label{sec:3DGen}
\vspace{-5pt}
\begin{figure*}[tb]
\vspace{-17pt}
\centering
\includegraphics[width=0.8\linewidth]{images/infer4.pdf}
\vspace{-10pt}
\caption{\small \textbf{\ours for Multi-View Generation}: From  iteratively generated views ({\color{brown}brown camera}), we randomly select a few anchor views (yellow stars) to guide  the generation of  target views along the {\color[RGB]{122,124,126}\textbf{gray camera trajectory}}. 
Keypoint matching is first performed to establish correspondences between the anchor views.
Next, monocular depth estimation is applied to the latest anchor view, followed by our 
\textit{Iterative Sparse Pixel-Wise Depth Alignment} to refine the depth and recover a dense map. This dense depth is then used to warp images along the gray camera viewpoints. Subsequently, the warped images and anchor images are combined and processed according to Eq.\ref{eq:ct} and  Eq.\ref{eq:mix}, without random masking, forming the \textit{visual-condition}, which guides  MVD model to produce  3D-consistent target views. Finally, the {\color[RGB]{122,124,126}\textbf{gray camera}} turns to {\color{brown}brown}, guiding multi-view generation in the next iteration.
} 
\vspace{-17pt}
\label{fig:infer}
\end{figure*}

In this section, we apply the proposed \textit{\ours} for domain-free 3D generation, enabling long-sequence novel view  generation with complex camera trajectories. Given a single or a few input views, we iteratively generate warped images with predefined camera poses and estimated global depth \cite{bhat2023zoedepth} as visual hints, \ours is then applied to generate frames corresponding to the target poses. This iterative pipeline is shown in Fig.\ref{fig:infer}, where the brown cameras represent the already generated views, and our objective is to generate the target views, marked as gray cameras.

Recent efforts \cite{chung2023luciddreamer, fridman2024scenescape, lei2023rgbd2} rely on monocular depth or point clouds, and perform global point-cloud alignment to recover the actual geometry for subsequent generations. However, since the reference view often provides a limited scene observation, using offline methods tends to suffer from \textit{scale ambiguity} and \textit{geometric estimation errors}, while previous methods overlook the correction of geometric estimation errors, resulting in distortions and stretching artifacts. These errors accumulate during iterative generation, severely degrading the generation quality.

\noindent \textbf{Pixel-wise Depth Scale Alignment.} To further correct local geometry errors, we propose pixel-wise depth scale alignment using sparse keypoints. we perform high-degree-of-freedom independent optimization for all keypoints by leveraging multi-view matching priors from anchor views. 
Each keypoint independently identifies its multi-view matches,  enabling the recovery of both depth scale and surrounding geometry.
Finally, we propagate the corrected  scale to the entire depth map using the 2D distances between keypoints and their neighbors.

Specifically, let $\{T_i\}_{i=0}^{N}$ denote  the predefined camera trajectory. Suppose we have generated $n$ images $\{I_i\}_{i=0}^n$, we now proceed to generate the next $m$ views using warped image from the last anchor views $I_n$,  which referred to as source view. We first utilize the pre-trained MoGe \cite{wang2024moge} to estimate affine-invariant depth $\boldsymbol{\hat{D}}_n$ of $I_n$. Inspired by \cite{xu2023frozenrecon}, we perform sparse alignment with $1024$ pairs of matching keypoints $\{\mathbf{m}_n, \mathbf{m}_i\}_k$, obtained by the pre-trianed extractor SuperPoint \cite{detone2018superpoint} and feature matcher LightGlue \cite{lindenberger2023lightglue}. For each matched point, we optimize the corresponding scale $\alpha^k$ and shift $\beta^k$ parameters, where $k \in [0, 1024]$, Our core idea is to recover the depth scaling by minimizing the $L_2$ distance of re-projection between matching points. For each iteration, the warping operation $\Pi_{n\rightarrow i}$ transforms pixels from the source image’s coordinate frame to the target image’s coordinate frame, formulated as: $\Pi_{n \rightarrow i}(\hat{d}_n) =  \hat{d}_n K_{i} T_{i} T_{n}^{-1} K_{n}^{-1}$, where $K_i,  K_n,T_i, T_n$ represent the intrinsic and extrinsic parameters of the source and target frames, respectively. The alignment for each pair is performed using normalized coordinates, ensuring that the warping aligns with the matching prior:
\vspace{-0.2cm}
\begin{equation}
    \alpha^{k*},\beta^{k*} = \mathop{argmin} \limits_{\alpha^{k},\beta^{k}} || \hat{d}_n^{k*} K_i T_i T_n^{-1} K_n^{-1} m_n^t - m_i^t||_2^2,
\vspace{-0.25cm}
\end{equation}
\noindent where the recovered depth of $k$th pixel is $\hat{d}_n^{k*} = \alpha^{k} \odot \hat{d}_n^k + \beta^{k}$, the $\odot$ is the pixel-wise Hadamard Product. We minimize the matching loss via gradient descent to obtain best scale $ \alpha^{k*}$ and shift parameters $\beta^{k*}$ for each pixel. By performing individual scale recovery and geometry correction, we decouple the depth correlation among different points, achieving accurate single-view reconstruction.

\noindent \textbf{Global Metric Depth Recovery.} After that, we set these recovered positions as sparse guidance $\hat{d}_n^*$, and introduce Locally Weighted Linear Regression \cite{xu2023frozenrecon} (marked as LWLR in Fig.\ref{fig:infer}) to recover the whole depth map based on the locations between guided points and the other target points. Let the global scale and shift parameters be $\boldsymbol{\beta_{u,v}} = [\boldsymbol{S}_{scale},\boldsymbol{S}_{shift}]_{u,v} ^ \mathsf{T}$, the metric depth recovery can be formulated as: 
\vspace{-0.1cm}
\begin{equation}
\min_{\boldsymbol{\beta}_{u, v}} (\hat{d}_n^* -\boldsymbol{X}\boldsymbol{\beta}_{u,v})^\mathsf{T}\boldsymbol{W}_{u,v}(\hat{d}_n^* -\boldsymbol{X}\boldsymbol{\beta}_{u,v})+\lambda\boldsymbol{S}_{shift}^2.
\vspace{-5pt}
\end{equation}

After obtaining the aligned depth $\boldsymbol{D}_n$, we generate the target visual hint through warping $\hat{I}_j = \Pi_{n \rightarrow j}(\boldsymbol{D}_n)$. The warped image $\{\hat{I}_j\}_{j=n}^{n+m}$ carries unfilled regions as the binary warping mask $\{M_j\}_{j=n}^{n+m}$, which serves as a strong visual hint for \ours to perform generation. To ensure multi-view consistency between the newly generated sequence and the previous content, we randomly select $k$ anchor views $\{I_k\},k \in [1,N]$ from the earlier  generated frames to guide subsequent generation. The generation process  can be formulated as: $I_j = \ours (\hat{I}_j, M_{j}, \{I_0,I_k\})$. We iteratively perform depth estimation, alignment, warping, and generation until all target images are acquired. 

\noindent\textbf{3D Reconstruction.} \label{sec: 3dgs}
We reconstruct the 3D scene using 3D Gaussian Splatting (3DGS) \cite{3dgs}. Following \cite{fan2024instantsplat}, we additionally introduce joint pose-Gaussian optimization to reduce the gaps between generated viewpoints and their corresponding camera poses. Please kindly refer to the Appendix for more details about global metric depth recovery and 3D reconstruction.

% appendix
% Our training minimizes the sum of photometric loss and SSIM loss as the original 3DGS. We additionally introduce a perceptual loss (LPIPS \cite{lpips}) to mitigate the impact of subtle \textbf{inter-frame} discrepancies in multi-view generated images on 3D geometric structure (3DGS) reconstruction. LPIPS emphasizes higher-level semantic consistency between the Gaussian-rendered and generated multi-view images, rather than focusing on minor high-frequency differences.
% Besides, the potential \textbf{inner-frame} diversity may cause inconsistency with the corresponding camera poses. Following \cite{fan2024instantsplat}, we introduce joint pose-Gaussian optimization, where camera parameters are treated as learnable variables alongside Gaussian attributes, thus reducing gaps between generated viewpoints and their corresponding camera poses.





% The intrinsic and extrinsic of the reference frame and the warped target visual hints $\{\hat{I}_j\}_{j=n}^{n+m}$ are denoted as $K_n, \{K_j\}_{j=n}^{n+m}$ and $T_n, \{T_j\}_{j=n}^{n+m}$. The warping operation between reference and on of the target view $\Pi_{n \rightarrow j}$ can be defined as: $\Pi_{n \rightarrow j}(\cdot) =  d_n K_{j} T_{j} T_{n}^{-1} K_{n}^{-1}$, where 


% Previous works \cite{chung2023luciddreamer,yu2024viewcrafter} usually maintain a global point cloud for next-frame rendering, however, the depth estimation and MVD are tightly coupled, using global point cloud to produce visual guidance may easily introduce error accumulation. Therefore, we cut the correlation with the early-stage estimation, and use only the latest generated view for next-frame visual guidance. However, to maintain geometric consistency within the 3D scene, It is required to restore the actual depth scale so that the next frame will be aligned to the expected camera trajectory. 


% This exploits multi-view consistency for point-by-point geometric restoration and global scale recovery for multi-view generation, providing higher quality visual guidance for multi-view generation.


% Additionally, we explicitly constrain the alignment of the point cloud in the current frame with the previous frame, allowing each new view to incorporate contextual information from preceding frames.


% Inspired by \cite{frozenrecon}, we present a learning-based monocular geometric alignment, which leverages the robust matching prior to \cite{lightglue} to obtain precise metric depth. Instead of directly recovering the actual scale at once, we conduct geometric alignment from a few reliable matching points. For each matched point, we predict a scale and offset, which not only restores the depth scale locally but also corrects potential geometric estimation errors. We then diffuse these local metric to obtain global metric depth. Specifically, for the $i^{th}$ step, denote the reference image $I_i$, and the corresponding mono-depth map $d_i$, the corresponding intrinsic and extrinsic are $K_i, T_i$, we detect feature correspondences between the target image and each reference image $I_j, j \in (0, i-1)$ by applying the LightGlue \cite{lightglue}, obtaining $k$ groups of matching pairs $\{\mathbf{m}_i, \mathbf{m}_j\}$, where $k=1024$ in our experiment.

% Next, we scale the matched monocular depths $d_i$ of the target image with learnable scale $\alpha$ map and shift  $\beta$ map, to yield the sparse metric depth $\hat{d}_i$:
% \begin{equation}
%     \hat{d}_i =  \alpha \cdot (\alpha \cdot d_i + \beta)  + \beta,
% \label{eq: scale shift}
% \end{equation}
% where we set $\alpha = 4.0 $ and $\beta = 0.25$ for faster convergence. For each iteration, the optimized metric depth is then used in the warping operation $\Pi_{i\rightarrow j}$ to transform pixels from the reference image’s coordinate frame to the target image’s coordinate frame, yielding warped coordinates $\mathbf{C}_{\text{sample}}^j = \Pi_{i\rightarrow j}(m_i)$. The matching loss is computed for each image pair using normalized coordinates, ensuring the warping aligns with detected match points:
% \begin{equation}
%     \mathcal{L}_{\text{match}} = \frac{1}{|\mathbf{m}_j|} \sum{\mathbf{m}_j} \| \mathbf{C}_{\text{sample}}^j - \mathbf{m}_j \|_2^2,
% \end{equation}
% where we minimize $\mathcal{L}_{\text{match}}$ via gradient descent over the scale and shift parameters. Finally, we utilize the Locally Weighted Liner Regression \cite{frozenrecon} to diffuse the sparse points to global scale-consistent depth. We conducted depth estimation, learning-based alignment, warping, and generation repeatedly until we had acquired all predefined multi-view images.

% \noindent\textbf{3D Reconstruction.}  After acquiring the multi-view images through the above process, we reconstruct the 3D scene using 3D Gaussian Splatting (3DGS) \cite{3dgs}. 3DGS represents scenes with a set of explicit anisotropic 3D Gaussians. Each Gaussian distribution is defined by a 3D covariance matrix $\bm{\Sigma}$ and a center position at point (mean) $\mathcal{X}$. A 3D Gaussian distribution $G(\mathcal{X})$ is formulated as follows:
% \begin{equation}
%     G(\mathcal{X}) = e ^{- \frac{1}{2} \mathcal{X}^{T} \bm{\Sigma}^{-1} \mathcal{X}},
% \end{equation}
% the rendering color $\boldsymbol{C}$ of each pixel is accumulated by blending the overlapping Gaussians as $\boldsymbol{C} = \bm{\Sigma}_{i \in N} \alpha_i c_i \Pi_{j=1}^{i-1} (1 - \alpha_j)$, where $\alpha_i$ is $\sigma_i$ multiplied by $\bm{\Sigma}'$. The tile-based rasterizer is utilized for efficient forward and backward passes. We concatenate the monocular depth estimates for each viewpoint from the previous stage into an initial point cloud, and optimize Gaussians with generated multi-view images. 

% However, the multi-view images are obtained from generation, the potential diversity may cause problems of inconsistency in the the generated views with their corresponding camera poses. Following \cite{instantsplat}, we further introduce a joint pose-Gaussian optimization to remove gaps between generated viewpoints and camera poses. Specifically, we turn camera parameters $\boldsymbol{T}$ into learnable variables with Gaussians attributes $G$. The detailed optimization is as follows:
% \begin{equation}
%     \boldsymbol{G}^*,\boldsymbol{T}^*=\arg\min_{\boldsymbol{G},\boldsymbol{T}}\sum_{v\in N}\sum_{i=1}^{HW}\left\|\tilde{\boldsymbol{C}}_v^i(\boldsymbol{G},\boldsymbol{T})-\boldsymbol{C}_v^i(\boldsymbol{G},\boldsymbol{T})\right\|,
% \end{equation}
% where $N$ is the number of generated views. This joint-optimization reduces the effects of inconsistencies between the generated observation and the camera poses, and promotes more robust 3D reconstruction.

% For more effectively optimized by gradient decent, the 3D covariance matrix  $\Sigma$  can be decomposed into a rotation matrix $\textbf{R}$ and a scaling matrix $\textbf{S}$ via $\bm{\Sigma} = \textbf{R}\textbf{S}\textbf{S}^{T}\textbf{R}^{T}$, where $\textbf{J}$ is the Jacobian of the affine approximation of the projection transformation. Finally, the color $C$ of each pixel is accumulated by blending the overlapping Gaussians as $C = \bm{\Sigma}_{i \in N} \alpha_i c_i \Pi_{j=1}^{i-1} (1 - \alpha_j)$, where $\alpha_i$ is $\sigma_i$ multiplied by $\bm{\Sigma}'$. The tile-based rasterizer is utilized for efficient forward and backward pass.





% For each iteration, the optimized metric depth is then used in a point cloud warping operation to transform pixels from the reference image’s coordinate frame to the target image’s coordinate frame based on the relative pose \mathbf{P}{\text{rel}}^i, yielding warped coordinates \mathbf{C}{\text{sample}}^i and a validity index set \mathbf{V}_{\text{idx}}.

==> sec/3_method_v0.tex <==
\section{Method}

Below we describe our XXX in Section xx, our XXX in Section xx.

\subsection{Preliminary:  Diffusion Models}
% \subsection{Background}
% \paragraph{Warping operation.}
%\paragraph{Diffusion model.}

Diffusion models operate by perturbing the training data $X_0 \sim  q(X_0)$ through a forward diffusion process and learning to reverse it. The forward diffusion process $X_t \sim q_{t|0}(X_t | X_0)$ can be formally represented by, 
\begin{equation}
X_{t} = \sqrt{\bar{\alpha}_{t}} \mathbf{X}_0 + \sqrt{1 - \bar{\alpha}_{t}} \boldsymbol{\epsilon}, \quad \boldsymbol{\epsilon} \sim \mathcal{N}(0, \mathbf{I}),
\end{equation}
where $\bar{\alpha}_{t}$ is variance schedule used in noise scheduler. In theory, $X_t$ approximates an isotropic Gaussian distribution for sufficiently large timesteps $t$ . The objective of training is to learn the reverse process. Thus, a trained diffusion model can generate a sample from the target distribution $q(X_0)$ by converting back sampling noise from Gaussian distribution via reverse process.

\begin{figure*}[tb]
\centering
\includegraphics[width=0.85\linewidth]{images/WonderWorld.pdf}
\caption{\small \todo{Training-pipeline.} Illustration of \textit{\ours}. Given single or sparse views, it provides ....  }
\label{fig:trainpipe}
\end{figure*}



\subsection{Latent Multi-View Diffusion Model}
Given a single or multiple sparse views  of a 3D scene, the goal of the model is to generate multiple views from the given their camera poses, ensuring alignment with the appearance of the input view(s). Previous works have typically incorporated the camera parameters  for  input views and  target views into a diffusion model to guide the generation of target images under target perspective. However, training these models often relies heavily on expensive 3D data, which includes precise annotations of camera movements.

Distinguished from prior works that laboriously collect 3D data meeting these requirements from designed artists, stereo matching, or Structure from Motion (SfM), which is costly, time-consuming, or even infeasible in certain situations. The main point of our work is to build a powerful foundation model from the perspective of dataset scaling-up. Compared to 3D data, `pseudo-3D-video' is highly scalable because it can be automatically extracted from the vast amount of video data available on the internet, which accumulates rapidly over time. Therefore, considering that `pseudo-3D-video' lacks camera annotations, we explore a solution that relies solely on visual signal from video data to control the camera's movement and generate multi-view images for target  perspectives during training phase , thereby avoiding the need for hard-to-obtain camera trajectories. In other words, we propose to train a multi-view diffusion model conditioned on visual hints without injecting camera parameters into the model. In summary, this task can be formulated as designing a conditional distribution , which is achieved by a conditional diffusion model minimizing,
\begin{equation}
\label{eq:loss}
\mathbb{E}_{X_0, Y_0, \epsilon, t} \left[ \left\lVert \epsilon_{\theta}(X_t, Y_0, V_0, t) - \epsilon \right\rVert_2^2 \right]
\end{equation}
where $X_t \sim q_{t|0}(X_t | X_0)$, and $X_0=\left \{ x_{0}^{i}  \right \} _{i=1}^{N}$ is a multi-view observation of a 3D  content, which is formed by sampling clip in the filtered video data, and $N$ is the number of frames in the sampled clip.  We randomly selected $S$ frames from $X_0$ as the given reference view(s) $Y_0=\left \{ y_{0}^{i}  \right \} _{i=1}^{S}$ of a 3D content, the other $L$ frames server as target images $T=\left \{ t^{i}  \right \} _{i=1}^{L}$. We focus on designing a novelty visual-condition expressed as $V_0$, which should guide the diffusion model to generate target images $T$ that present plausible estimation of the 3D scene under the target viewpoints that aligns with the appearance of $Y_0$. More importantly, our goal is to design a robust visual condition that can be constructed without relying on additional 3D annotations and is independent of downstream tasks. This visual condition should exhibit sufficient generalization capability to accommodate different task-specific visual conditions for precise camera movement control. Based on the aforementioned analysis, we believe that selecting some pixels in images as the source of the visual condition allows the model to learn the capability of controlling camera positions using pixel-level visual cues. Furthermore, we aim for the proposed visual condition to exhibit strong robustness, particularly when there is a domain gap between the task-specific visual cues and the pixels extracted from video data. For instance, in warp-based generation, warp images often present challenges such as self-occlusions, artifacts and distortions, which create a significant gap compared to the visual signals in real videos, as illustrated in the Fig.?. Therefore, our design principles are: 1) Reducing the information of video data through random masking, thereby reducing the dependency on visual signals from pixels. This enables the model to partially ignore the gap between task-specific visual cues and video data. 2) Introducing noise into the video data to make its distribution closer to a Gaussian distribution. When applied to different downstream tasks, the input task-specific visual cues are also subjected to noise, bringing their distribution closer to a Gaussian distribution, thereby reducing the distribution distance between the downstream task and video data to some extent.


% \uncer{Warping the given view(s) onto the camera plane defined by the target camera parameters provides an effective visual hint, as warp images inherently capture camera movement information through the rearrangement of pixels from the input images, replacing the camera parameters. However, it is indeed not trivial to construct warp images as conditioning in the use of such large-scale video data, especially in cases where the camera trajectories and 3D geometric structures of a large volume of video data are unknown. To address this dilemma, we first analyze the properties of warp images and then propose a solution.As shown in Fig. 4, warp images generally exhibit four distinct characteristics compared to regular images: 1) missing regions, 2) occlusions, 3) artifacts, and 4) geometric distortions. The first two characteristics arise the movement of the camera, which causes some points in the point cloud to be unable to project onto the target camera plane, or self-occlusion occurring within the camera plane. The latter two characteristics are caused by the imperfections in the estimated point cloud due to insufficient observation. Based on the above analysis, the specific content of warp images is formed by various complex factors, including point cloud quality, camera poses, and self-occlusion relationships in the 3D scene, making it challenging to simulate such warp images using video data. Therefore, we propose a novel solution. We abandon the highly impractical approach of simulating warp images from video data as visual hints. Instead, we attempt to explore whether it is feasible to use video data as visual hints during the training phase, while using warp images as visual hints during the inference phase. Our insight is to minimize the model's dependence on visual cues from video data as much as possible, thereby enabling the model to disregard the differences between visual cues from video data during training and warped images during inference.}

% In our preliminary attempts, a natural approach is to perturb and randomly mask video data, then use this corrupted video data as visual hints to condition the diffusion model.

Our initial attempt involved introducing noise and random irregular masks on video data, referred to as corrupted video data. The corrupted video data is used as visual hints conditioned on the model.
% aiming to balance the model's difficulty in predicting target views from $X_t$ or visual hints, thereby reducing reliance on visual hints.
A critical challenge of this strategy lies in determining the appropriate level of perturbation to add to the video data. If significant noise is added, it makes it challenging to effectively employ conditional signals, resulting in poor visual quality and inaccurate camera control. Conversely, if minimal noise is added, the corrupted video data will retain substantial details of the target images, leading the model to become overly reliant on visual hints from video data. 
% To explain further, compared to using warped images as visual hints during inference, minimally corrupted video data retains significant information about the target views during training. This information leakage during training exacerbates the training-inference discrepancy, leading to a significant drop in test performance. 

To overcome this, we designed a time-dependent noise distribution on video data. The key principle is to add high noise levels at large time steps to sufficiently disrupt the video data, preventing over-reliance, while transitioning to lower noise levels as the time step decreases, serving as cleaner conditional signals to aid content generation. As the noise level gradually decreases, the risk of information leakage increases and the distribution begins to diverge from a Gaussian distribution. We suggest gradually replacing the disrupted video data with $X_t$ as visual hints, thereby forcing the model to rely primarily on $X_t$ for generation and neglect the pixel signals from video data, as formulated by,

\begin{equation}
V_t=[W_t\ast C_t+  \left ( 1-W_t \right ) \ast X_t;M]
\end{equation}

\begin{equation}
C_{t} = \sqrt{\bar{\alpha}_{t'}} (1-M)\mathbf{X}_0 + \sqrt{1 - \bar{\alpha}_{t'}} \boldsymbol{\epsilon}, \quad \boldsymbol{\epsilon} \sim \mathcal{N}(0, \mathbf{I}),
\end{equation}

\begin{equation}
t'=f(t)
\end{equation}

where $M=\left \{ m^{i}  \right \} _{i=1}^{N}$ denote random irregular mask operations, in which $m^{0:S}$ are the zero matrix to ensure the given reference images are clean without masking, and $\bar{\alpha}_{t'}$ are variances used in DDIM, and $V_t=\left \{ v_{t}^{i}  \right \} _{i=1}^{N}$ indicate be the visual hints mentioned in Eq.\ref{eq:loss}, which is a mixture of $C_t$ and $X_t$ concatenated with masks $M$ along the channel dimension. In practice, there is an additional processing step where we set $v_{t}^{0:S}$ to given images $Y_0$ to benefit that the information from $Y_0$ is retained as it inject into model, facilitating the alignment of the output multi-view and the given images. $W_t$ is the balance weight, which is designed to decrease monotonically with timestep $t$, ranging from 1 to 0. Function $f$ is designed to be strictly monotonically increasing and requires that $t' < t$, thus ensuring that $C_t$ does not contain less information than $X_t$ at the early timestep. Otherwise, when timestep $t$ is large enough, $C_t$ will overclose to Gaussian noise, resulting in no ability to control the camera movement at all.

\noindent\textbf{Model architecture.} Our model architecture is similar to video diffusion model[?]. However, we removed the time embedding, as we want the model to control the camera solely through visual conditions rather than inferring the movement trend based on temporality. Furthermore, to minimize the effect of temporality, we shuffle frames in each video clip as unordered data $X_0$. The main backbone of our model is consistent with the 2D diffusion model but includes 3D self-attention connecting the latents of multiple images, as in prior work[?]. Specifically, we reuse the existing 2D self-attention layers of the original 2D diffusion model as 3D self-attention by inflating different views in the self-attention layers. To inject visual conditions, we add the necessary convolutional kernels and biases via he Zero-Initialize[?]. We initialize the model from 2D diffusion[?] and fine-tune all the parameters, using FlashAttention for acceleration. Similar to prior work[?], we found it crucial to switch from a scaled-linear noise schedule to a linear schedule to achieve better global consistency between multiple views. We perform cross-attention between the latents of multiple views and per-token CLIP embeddings of reference images via linear guidance mechanism[?]. Finally, we randomly select a subset of frames from a video clip as reference images, while the number of this reference images is randomly selected in order to adapt to different downstream tasks, and the remaining frames serve as target images. The multi-view diffusion model is optimized by just calculating loss on the target images, as described in Eq.\ref{eq:loss}.

% $V_t=\left \{ v_{t}^{i}  \right \} _{i=1}^{N}$ are the visual hints, which are used as condition injected into the diffusion model to guide the generation of multiple views in Eq.\ref{eq:loss}. $\bar{\alpha}_{t'}$ are variances used in DDIM. $W_t$ is the balance weight, which is designed to decrease monotonically with timestep $t$, ranging from 1 to 0. $X_t=\left \{ x_{t}^{i}  \right \} _{i=1}^{N}$ is the noise latent at timestep $t$, which introduces noise to $X_0$ by employing diffusion model’s inversion process. During the training phase, $R_0$ denotes corrupted video data formed by irregular masks. In the testing phase, $R_0$ denotes the warp images corresponding to a predefined camera trajectory. Function $f$ is designed to be strictly monotonically increasing and requires that $t' < t$, thus ensuring that $C_t$ does not contain less information than $X_t$. Otherwise, when timestep $t$ is large enough, $C_t$ will converge to Gaussian noise, resulting in no ability to control the camera movement at all. Here, $N = S + M$, where $S$ is the number of given images, and $M$ is the number of target images. 


\subsection{Data Curation}
\label{sec:data}
Pretraining on high-quality large-scale video data with 3D features is essential for our model to produce accurate and reliable 3D priors. A well-defined 3D video has two properties: a) the contents in the scene remain static temporally, and b) the camera's ego-motion produces long-range multi-view baselines. The first one ensures consistent scene geometry across different viewpoints in the video, which facilitate our model to learn accurate 3D priors. While the dynamic areas create biases in the model's comprehension of 3D, thus degrading the generation accuracy. The second provides sufficient 3D observations from multiple viewpoints, thereby providing our model with a more comprehensive understanding of the 3D world. Conversely, when pre-training with multi-view videos with small baselines, the model \todo{will be prone to fall into a local minima, where it tends to generate images that are close to the reference viewpoint that achieves lower training loss}, without actually learning the 3D priors imposed by the camera movement.
% 其中第一个xxx，第二个会xxxx。
% 为了获取到大量的3D数据，我们收集了各种各样的视频数据用于我们的模型训练。但是挑出来是不trivial的。

Current open-source 3D dataset that meets our definition, such as RealEstate10K \cite{}, Tanks and Temples \cite{}, etc., contains a limited number of multi-view images, which is far from meeting our model pre-training requirements. To obtain a massive volume of 3D data, we collect about \textbf{25M} open-sourced video clips of \textbf{44.98 GPU years} from the internet, covering a wide range of categories, such as landscapes, animals, plants, games, and actions as preparation. Specifically, our dataset consists of four sources of Pexels\footnote{https://www.pexels.com/search/videos/videos/}, Artgrid\footnote{https://artlist.io/stock-footage}, Airvuz\footnote{https://www.airvuz.com/collections}, and Skypixel\footnote{https://www.skypixel.com/}. We follow previous effort \cite{svd} to split the videos with PySceneDetect\footnote{https://github.com/Breakthrough/PySceneDetect} to identify content changes and fade-in/out events, respectively. We also remove clips with excessive text using PaddleOCR\footnote{https://github.com/PaddlePaddle/PaddleOCR}. Our detailed dataset formulation is shown in \cref{tab:data_stat}.

% \todo{whether add previous 3D dataset info or not?}
% \begin{table}[!ht]
% \centering
% \resizebox{0.48\textwidth}{!}{
% \begin{tabular}{ccccccc}
% \toprule
% Source   & Domain    & \#Videos         & \#Clips                   & Total Duration                                                &\# Filtered Clips           & Filtered Duration \\ \midrule
% Pexels   & Open      & 729,489 +545160      & 729,489 +5451602          &   10,905.46h,554.4d,1.24y+90860.03h,3785.84d,10.36y            & 86,995 + 519571         & 1300.52h, ratio 0.12+8661.18h              \\
% Artgrid  & Open      & 485,270 +545160        &  485,270 +5451602        &  1,627.52h,67.81h,0.19y+90860.03h,3785.84d,10.36             &  21,756  +519571      & 106.75h,4.45d.0.01y, ratio0.065+8661.18h      \\
% Airvuz   & Landscape & 88,150  +545160         &  1,649,761 +5451602     &  3,889.17h,162d,0.44y+90860.03h,3785.84d,10.36y              &  19,323  +519571        & 60.55h,ratio 0.012+8661.18h                     \\
% Skypixel & Landscape & 723,454 +545160        &  7,813,660 +5451602     &   14,608.23h,608d,1.67y+90860.03h,3785.84d,10.36y            & 85,983  +519571           & 160.75h,ratio 0.011+8661.18h                 \\ \midrule
% Total    & -         & xx                   & xx                         & xx              & xx                  &                \\
% \bottomrule
% \end{tabular}
% }
% \caption{Initial Dataset Statistic.}
% \label{tab:data_stat}
% \end{table}
\begin{table}[!ht]
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{ccccccc}
\toprule
Source   & Domain    & \#Videos         & \#Clips           & Total Time (hrs)         &\#Filtered Clips  & Filtered Time (hrs) \\ \midrule
Pexels   & Open      & 1,274,649      & 6,181,091          &   101,765.49          & 606,566         & 9,961.70              \\
Artgrid  & Open      & 1,030,430        &  3,936,872        &  92,487.55            &  541,327        & 8,767.93      \\
Airvuz   & Drone & 633,310         &  5,101,363     &  94,749.20                &  538,894        & 8,721.73                     \\
Skypixel & Landscape & 1,268,614       &  10,265,262     &   105,468.26            & 605,554           & 8,821.93                 \\ \midrule
Total    & Open         & 4,207,003       & 25,484,588     & 394,470.5              & 2,292,341            & 36,273.29               \\
\bottomrule
\end{tabular}
}
\caption{Detailed Component of Our VideoNVS Dataset.}
\label{tab:data_stat}
\end{table}

However, we found that identifying these 3D videos is not trivial. Since most of the videos are derived from real shots, the data is filled with dynamic scenes, as well as videos with minimal camera movement. Therefore, we propose a novel and sophisticated pipeline to filter out high-quality 3D data, which is composed of four core steps: 1) Temporal-Spatial Downsampling, 2) Semantic-Based Dynamic Filtering, 3) Non-Rigidity Dynamic Recognition, and 4) Tracking-Based Small Baseline Filtering.

\subsubsection{Step 1: Temporal-Spatial Downsampling}
We downsample each video in time and space thereby increasing the efficiency. Temporally, we downsample by a factor of two, retaining an image every two frames for subsequent identification. Spatially, for each segmented image, it is different in aspect ratio between images in different videos. To ensure that the original content is as reliable as possible after downsampling, we downsample a different multiplier according to the size of the original resolution to achieve comparable resolution. In this paper, we use the final resolution of 480p. It is worth noting that our downsampling here is only for more efficient data filtering, and we use additional data processing during pretraining.


\subsubsection{Step 2: Semantic-Based Dynamic Filter}
We process the content recognition on each image frame. We follow \cite{rodynrf} to utilize the off-the-shelf instant segmentation model Mask R-CNN \cite{} to generate coarse motion masks $\mathcal{M}_m$ of humans, animals, sports, etc. If the number of frames with motion mask is more than half of the total number of frames in the current video, we consider that there is a higher probability of dynamic regions in this video, and we remove this in the subsequent processing.

% The semantic-based dynamic filter $\mathcal{F}_m$ can be formulated as:

% \begin{equation}
% \mathcal{F}_m = \left\{\begin{array}{l}
%      A \\
%      B
% \end{array}\right.
% \end{equation}

% where $\operatorname{sum}(M_m) = \Sigma_{u,v=0}^{W,H}(u,v)$. xxxx

% \begin{equation}
%         \mathcal{F}(\mathcal{C})=\left\{\begin{array}{l}
% \frac{\operatorname{sum}\left(\mathcal{M}_{\mathcal{C}}\right)}{W \times H}, \frac{\operatorname{sum}\left(\mathcal{M}_{\mathcal{C}}\right)}{W \times H}<\Theta \\
% 1-\frac{\operatorname{sum}\left(\mathcal{M}_{\mathcal{C}}\right)}{W \times H}, \frac{\operatorname{sum}\left(\mathcal{M}_{\mathcal{C}}\right)}{W \times H}>\Theta
% \end{array}\right.
% \end{equation}

\subsubsection{Step 3: Non-Rigid Dynamic Recognition}
After coarse filtering out videos with common dynamic objects, we apply a more precise strategy to filter out videos with non-rigidity dynamic regions, such as drifting water or swaying trees \cite{rodynrf}. Following \cite{rodynrf}, we first apply pretrained RAFT \cite{raft} to generate optical flow between every two extracted frames, we then calculate and threshold the Sampson distance to obtain a non-rigid motion mask $\mathcal{M}_s$, where the Sampson distance is the distance of each pixel to the estimated epipolar line \cite{}. A higher number of these mask pixels represents a higher probability of motion occurring in the current frame. However, it is unreliable to rely solely on this condition to determine whether there is a motion, because most of our data are collected from real shots, where people usually place the dynamic object of interest in the center of the imaging plane, and these moving regions may not very large. Therefore, based on this assumption, we additionally consider the location of the dynamic mask appears. Therefore, we propose a dynamic score $\mathcal{S}$ to evaluate the dynamic probability of the current frame. Denote $H, W$ is the height and weight of an image, $W'=0.25\times W, H'=0.25\times H$ is the central start of an image, the proportion $\Theta_i$ of the entire image occupied by the mask, and the central proportion $\Theta_c$ of the central area can be calculated as:
\begin{equation}
\Theta_i = \frac{\Sigma_{u,v=0}^{W,H}\mathcal{M}_s(u,v)}{H\times W}, \\
\Theta_c = \frac{\Sigma_{u,v=W', H'}^{W-W',H-H'}\mathcal{M}_s(u,v)}{H/2\times W/2}.
\end{equation}
The dynamic score can be formulated as:
\begin{equation}
\mathcal{S}_i =\begin{cases}
     2, & \Theta_i \geq 0.12 \And \Theta_c \geq 0.35 \\
      1.5, &\Theta_i \geq 0.12 \And 0.2 \leq \Theta_c < 0.35 \\
      1, &\Theta_i < 0.12 \And 0.2 \leq \Theta_c < 0.35 \\
      0.5, &\Theta_i < 0.12 \And \Theta_c < 0.2 
\end{cases}.
\end{equation}
% After that, we determine whether a dynamic region appears in the current frame based on the number of pixels and the overall position of the mask. We notice that most of the dynamic regions in casually captured videos are distributed in the central area of the image. 
% \sigma_s(\mathcal{M}_s)=\Sigma_{u,v=0}^{W,H}\mathcal{M}_s(u,v), \\
% \sigma_c(\mathcal{M}_s)=\Sigma_{u,v=W', H'}^{W-W',H-H'}\mathcal{M}_s(u,v)
This strategy enhances the focus of the dynamic region in the center of the image, which increases the accuracy of filtering. We then calculate the final dynamic score $\mathcal{S}$ of the whole sequence as:
\begin{equation}
    \mathcal{S} = \Sigma_{i=0}^N \mathcal{S}_i,
\end{equation}
where $N$ represents the number of extracted frames. When $\mathcal{S} >= 0.25 \times N$, we filter out this sequence as dynamic video.

\subsubsection{Step 4: Tracking-Based Small Baseline Filter}
We obtained videos where the scene contents remained static in previous steps. As we mentioned above, we still need to obtain videos consisting of multi-view images with a large camera baseline. Our core idea is to track the motion trajectory of key points in an image by tracking them in different frames and determining the radius of the minimum outer tangent circle of the trajectory. If a large number of circle radii are smaller than the threshold, it indicates that the camera trajectory of this video is small, and it is not possible to extract a multi-view image with a larger baseline. The procedure combines keypoint extraction, trajectory tracking, and circle fitting using RANSAC (Random Sample Consensus).

We further downsample the previously extracted video frames by taking every fourth frame to reduce computational complexity. Then, we leverage SuperPoint \cite{superpoint} to extract keypoints $\mathbf{K} \in \mathbb{R}^{N \times 2}$ on the first frame, where $N=100$ is the number of detected keypoints, are used to initialize tracking. Keypoints are tracked through all frames using pretrained CoTracker \cite{cotracker}. It generates trajectories and the keypoints' visibility over time as:
\begin{equation}
\mathbf{T}_{\text{pred}}, \mathbf{V}_{\text{pred}} = \text{CoTracker}(\mathbf{I}, \text{queries}=\mathbf{K}),
\end{equation}
where $\mathbf{I}$ is the input frames, $\mathbf{T}_{\text{pred}} \in \mathbb{R}^{1 \times T \times N \times 2}$ represents the tracked positions of each keypoint across time steps, and $\mathbf{V}_{\text{pred}} \in \mathbb{R}^{1 \times T \times N \times 1}$ indicates the visibility of each point. For each tracked keypoint, a circle fitting method is applied to its trajectory. We select only those frames where the keypoint is visible $(\mathbf{V}_{\text{pred}} = 1)$. Let $\mathbf{T}_{\text{visible}} \in \mathbb{R}^{M \times 2}$ be the filtered points, where $M$ is the number of visible points, we apply the RANSAC-based circle fitting algorithm to $\mathbf{T}_{\text{visible}}$ to find the circle’s center $\mathbf{c} = (c_x, c_y)$ and radius  $r$:
\begin{equation}
\mathbf{c}, r = \text{RANSAC}(\mathbf{T}_{\text{visible}}),
\end{equation}
the RANSAC algorithm selects random subsets of three points to define candidate circles, computes inliers, and optimizes for the circle with the highest inlier count and smallest radius. Finally, we count the number of circles with a radius smaller than a threshold  $r \leq 20$:
\begin{equation}
\text{count} = \sum_{i=1}^{N} \mathbb{I}(r_i \leq 20),
\end{equation}
where $\mathbb{I}$ is the indicator function. The mean radius is also computed to provide an overall measurement of the circular motion. If the number of small radius circle is more than 40 and the average circular motion is less than 5, we filter this video with small camera trajectory.

\subsubsection{User Study}
To verify the effectiveness of our data filtering pipeline, we randomly selected 10,000 video clips as user study before filtering, of which the number of videos that satisfy our definition of 3D video is 1,163, and the percentage of 3D data is 11.6\%. We also randomly selected 10,000 video clips for people to annotate after data screening, and found that the number of 3D video annotations was 9,304 videos with a ratio of 93\%, which is 81.4\% higher compared to the previous one, indicating that our proposed method effectively preserves 3D data.

\subsection{Visual Condition-based Image-to-3D Generation}
In this section, we leverage the 3D priors of \ours for domain-free 3D generation. We utilize monocular depth estimation \cite{geowizard} to provide preliminary 3D structure, and generate visual guidance with depth-based warping iteratively for multi-view generation. Recent efforts \cite{chung2023luciddreamer, fridman2024scenescape, lei2023rgbd2} typically aligned the affine-invariant depth with the preceding estimated 3D structure, which conducts one-step global scale and shift recovery. However, monocular depth estimation leads to geometry errors due to limited observation, which cannot be corrected simply by aligning the global scales from the preceding frames. Therefore, visual hints generated through previous methods are prone to distortions and stretching errors that affect subsequent generation.\todo{viewcrafter?}

To address this limitation, we propose a learning-based alignment to impose mono-depth align with 3D structure and further refine monocular geometry. We start by learning sparse pixel-level depth restoration via matching prior on multi-view generation, 


and then diffuse the local metric to the global depth map. 



% Previous works \cite{chung2023luciddreamer,yu2024viewcrafter} usually maintain a global 


% point cloud for next-frame rendering, however, the depth estimation and MVD are tightly coupled, using global point cloud to produce visual guidance may easily introduce error accumulation. Therefore, we cut the correlation with the early-stage estimation, and use only the latest generated view for next-frame visual guidance. 

% pre-define a camera trajectory for synthesizing novel viewpoints, 



% Following \cite{luciddreamer, wonderworld}, we utilize a monocular depth estimation \cite{geowizard} to provide preliminary geometry, pre-define a camera trajectory for synthesizing novel viewpoints, and generate partial visual hints as novel view guidance with homography warping. We further introduce a 3D Gaussian Splatting \cite{3dgs} with camera refinement for 3D representation.
% Benefiting from the robust visual conditioning strategy, our MVD model demonstrates resilience to artifacts and distortions from the monocular depth estimation for warping. However, significant viewpoint shifts and depth estimation errors still remain challenging in certain regions. To address these issues, we propose learning-based monocular geometric alignment, which leverage the robust matching prior \cite{lightglue} to recover the actual scale of depths and corrects erroneous where needed.
Specifically, suppose we have generated $n$ images $\{I_i\}_{i=0}^N$, we now perform next $m$ frames generation, using the visual hints warped from the last frame $I_n$, which termed as reference view. We utilize pretrianed GeoWizard \cite{geowizard} to estimate affine-invariant depth $\hat{d}_n$. Inspired by \cite{frozenrecon}, we conduct geometric alignment from a set of sparse  reliable matching points, where we detect feature correspondences between the target image and each reference image $I_j, j \in (0, i-1)$ by applying the pretrianed LightGlue \cite{lightglue}, obtaining $k$ groups of matching pairs $\{\mathbf{m}_i, \mathbf{m}_j\}$, where $k=1024$ in our experiment.



which not only restores the depth scale locally but also corrects potential geometric estimation errors.

 and then diffuse the local metric to the global depth map. Instead of directly recovering the actual scale at once, 



The intrinsic and extrinsic of the reference frame and the warped target visual hints $\{\hat{I}_j\}_{j=n}^{n+m}$ are denoted as $K_n, \{K_j\}_{j=n}^{n+m}$ and $T_n, \{T_j\}_{j=n}^{n+m}$. The warping operation between reference and on of the target view $\Pi_{n \rightarrow j}$ can be defined as: $\Pi_{n \rightarrow j}(\cdot) =  d_n K_{j} T_{j} T_{n}^{-1} K_{n}^{-1}$, where we can obtain target visual hint as $\hat{I}_j = \Pi_{n \rightarrow j}(I_n)$. The warped image $\{\hat{I}_j\}_{j=n}^{n+m}$ carries unfilled regions as the binary warping mask $\{M_j\}_{j=n}^{n+m}$, which is also a strong visual hint for \ours to perform novel view generation. To ensure strong multi-view consistency between the newly generated sequence and the previous content, we randomly select several anchor views ${I_k},k \in [1,N]$ from the already generated images to guide subsequent generation. The generated multi-view images can be formulated as:
\begin{equation*}
    I_j = \ours (\hat{I}_j, M_{j}, \{I_0,I_k\}).
\end{equation*}

% Previous works \cite{chung2023luciddreamer,yu2024viewcrafter} usually maintain a global point cloud for next-frame rendering, however, the depth estimation and MVD are tightly coupled, using global point cloud to produce visual guidance may easily introduce error accumulation. Therefore, we cut the correlation with the early-stage estimation, and use only the latest generated view for next-frame visual guidance. However, to maintain geometric consistency within the 3D scene, It is required to restore the actual depth scale so that the next frame will be aligned to the expected camera trajectory. 


This local-to-global depth optimization strategy exploits multi-view consistency for point-by-point geometric restoration and global scale recovery for multi-view generation, providing higher quality visual guidance for multi-view generation.


Additionally, we explicitly constrain the alignment of the point cloud in the current frame with the previous frame, allowing each new view to incorporate contextual information from preceding frames.


Inspired by \cite{frozenrecon}, we present a learning-based monocular geometric alignment, which leverages the robust matching prior to \cite{lightglue} to obtain precise metric depth. Instead of directly recovering the actual scale at once, we conduct geometric alignment from a few reliable matching points. For each matched point, we predict a scale and offset, which not only restores the depth scale locally but also corrects potential geometric estimation errors. We then diffuse these local metric to obtain global metric depth. Specifically, for the $i^{th}$ step, denote the reference image $I_i$, and the corresponding mono-depth map $d_i$, the corresponding intrinsic and extrinsic are $K_i, T_i$, we detect feature correspondences between the target image and each reference image $I_j, j \in (0, i-1)$ by applying the LightGlue \cite{lightglue}, obtaining $k$ groups of matching pairs $\{\mathbf{m}_i, \mathbf{m}_j\}$, where $k=1024$ in our experiment.

Next, we scale the matched monocular depths $d_i$ of the target image with learnable scale $\mathbf{s}_{scale}$ map and shift  $\mathbf{s}_{shift}$ map, to yield the sparse metric depth $\hat{d}_i$:
\begin{equation}
    \hat{d}_i =  \mathbf{s}_{scale} \cdot (\alpha \cdot d_i + \beta)  + \mathbf{s}_{shift},
\label{eq: scale shift}
\end{equation}
where we set $\alpha = 4.0 $ and $\beta = 0.25$ for faster convergence. For each iteration, the optimized metric depth is then used in the warping operation $\Pi_{i\rightarrow j}$ to transform pixels from the reference image’s coordinate frame to the target image’s coordinate frame, yielding warped coordinates $\mathbf{C}_{\text{sample}}^j = \Pi_{i\rightarrow j}(m_i)$. The matching loss is computed for each image pair using normalized coordinates, ensuring the warping aligns with detected match points:
\begin{equation}
    \mathcal{L}_{\text{match}} = \frac{1}{|\mathbf{m}_j|} \sum{\mathbf{m}_j} \| \mathbf{C}_{\text{sample}}^j - \mathbf{m}_j \|_2^2,
\end{equation}
where we minimize $\mathcal{L}_{\text{match}}$ via gradient descent over the scale and shift parameters. This iterative learning effectively aligns the geometric representation across views, resulting in more accurate 3D scene reconstruction and depth alignment. Finally, we utilize the Locally Weighted Liner Regression \cite{frozenrecon} to diffuse the sparse points to global scale-consistent depth. We conducted depth estimation, learning-based alignment, warping, and generation repeatedly until we had acquired all predefined multi-view images.

\noindent\textbf{3D Reconstruction.}  After acquiring the multi-view images through the above process, we reconstruct the 3D scene using 3D Gaussian Splatting (3DGS) \cite{3dgs}. 3DGS represents scenes with a set of explicit anisotropic 3D Gaussians. Each Gaussian distribution is defined by a 3D covariance matrix $\bm{\Sigma}$ and a center position at point (mean) $\mathcal{X}$. A 3D Gaussian distribution $G(\mathcal{X})$ is formulated as follows:
\begin{equation}
    G(\mathcal{X}) = e ^{- \frac{1}{2} \mathcal{X}^{T} \bm{\Sigma}^{-1} \mathcal{X}},
\end{equation}
the rendering color $\boldsymbol{C}$ of each pixel is accumulated by blending the overlapping Gaussians as $\boldsymbol{C} = \bm{\Sigma}_{i \in N} \alpha_i c_i \Pi_{j=1}^{i-1} (1 - \alpha_j)$, where $\alpha_i$ is $\sigma_i$ multiplied by $\bm{\Sigma}'$. The tile-based rasterizer is utilized for efficient forward and backward passes. We concatenate the monocular depth estimates for each viewpoint from the previous stage into an initial point cloud, and optimize Gaussians with generated multi-view images. 

However, the multi-view images are obtained from generation, the potential diversity may cause problems of inconsistency in the the generated views with their corresponding camera poses. Following \cite{instantsplat}, we further introduce a joint pose-Gaussian optimization to remove gaps between generated viewpoints and camera poses. Specifically, we turn camera parameters $\boldsymbol{T}$ into learnable variables with Gaussians attributes $G$. The detailed optimization is as follows:
\begin{equation}
    \boldsymbol{G}^*,\boldsymbol{T}^*=\arg\min_{\boldsymbol{G},\boldsymbol{T}}\sum_{v\in N}\sum_{i=1}^{HW}\left\|\tilde{\boldsymbol{C}}_v^i(\boldsymbol{G},\boldsymbol{T})-\boldsymbol{C}_v^i(\boldsymbol{G},\boldsymbol{T})\right\|,
\end{equation}
where $N$ is the number of generated views. This joint-optimization reduces the effects of inconsistencies between the generated observation and the camera poses, and promotes more robust 3D reconstruction.

% For more effectively optimized by gradient decent, the 3D covariance matrix  $\Sigma$  can be decomposed into a rotation matrix $\textbf{R}$ and a scaling matrix $\textbf{S}$ via $\bm{\Sigma} = \textbf{R}\textbf{S}\textbf{S}^{T}\textbf{R}^{T}$, where $\textbf{J}$ is the Jacobian of the affine approximation of the projection transformation. Finally, the color $C$ of each pixel is accumulated by blending the overlapping Gaussians as $C = \bm{\Sigma}_{i \in N} \alpha_i c_i \Pi_{j=1}^{i-1} (1 - \alpha_j)$, where $\alpha_i$ is $\sigma_i$ multiplied by $\bm{\Sigma}'$. The tile-based rasterizer is utilized for efficient forward and backward pass.





% For each iteration, the optimized metric depth is then used in a point cloud warping operation to transform pixels from the reference image’s coordinate frame to the target image’s coordinate frame based on the relative pose \mathbf{P}{\text{rel}}^i, yielding warped coordinates \mathbf{C}{\text{sample}}^i and a validity index set \mathbf{V}_{\text{idx}}.

==> sec/4_exp.tex <==
\vspace{-10pt}
\section{Experiments}
\vspace{-5pt}
% In this section, we first introduce the implementation details of \ours in \cref{exp:imple} and the dataset used for evaluation in \cref{exp:data}. Next, we present the 3D reconstruction results using our model with single-view and sparse-view inputs in \cref{exp: single} and \cref{exp: sparse}, respectively. Subsequently, we demonstrate the performance of zero-shot generation using our proposed novel 3D generation pipeline in \cref{exp: generation}. Finally, we conduct ablation experiments in \cref{exp: ablation} to validate the effectiveness of the proposed modules.

In \cref{exp: single}, we present the single view and sparse views reconstruction with \ours as prior.  Next, we conduct ablation experiments in \cref{exp: ablation} to validate the effectiveness of the proposed modules. Additionally, implementation details, more results on open-world 3D creation, and further ablation experiments are provided in the Appendix. We also present more generation results including long-sequence novel view generation in the Appendix.

% \subsection{Implementation Details.} M'o
% \label{exp:imple}
% xxxxxxx

% Metrics
%为什么用这些指标 为什么不仅能反映生成视角的质量 还能说明控制视角的准确不准确

% \subsection{Evaluation Dataset} 
% \label{exp:data}
% We follow previous work on single/sparse-view generation and conduct evaluations on several datasets including scene-level: Tanks and Temples, RealEstate10K \cite{real10k}, LLFF \cite{llff}, MipNeRF-360 \cite{barron2022mipnerf360}; and object-level: CO3D \cite{co3d},  DTU \cite{dtu}. Tanks and Temples containing videos of large-scale scenes, RealEstate10K comprises video clips of indoor scenes, MipNeRF-360 contains a complex central object or area and a detailed background. LLFF and DTU are dataset of forward-facing scenes, Co3D is a video dataset containing object recordings. In the following sections, we will provide detailed experimental settings of each dataset.


\vspace{-5pt}
\subsection{Single and Sparse Views to 3D}
\label{exp: single}
\vspace{-5pt}
\noindent\textbf{Experimental Setting.} \ours supports multi-view generation from a single input view. Following prior work \cite{yu2024viewcrafter}, our evaluation is conducted on the test split of three real-world datasets with various camera trajectories, including Tanks-and-Temples \cite{knapitsch2017tanks}, RealEstate10K \cite{real10k}, CO3D \cite{reizenstein2021common}. 
% Tanks-and-Temples contains videos of large-scale scenes, we use 9 scenes for evaluation. RealEstate10K comprises video clips of indoor scenes, we adopt 10 scenes from its original test set. CO3D is an object-level dataset containing different object recordings, we evaluated on all 10 scenes. 
%We follow ViewCrafter’s approach \cite{yu2024viewcrafter} of constructing easy/hard evaluation sets based on different sampling rates to process the original videos. 
We follow the approach in ViewCrafter \cite{yu2024viewcrafter} for constructing easy/hard evaluation sets based on different sampling rates applied to the original videos. 
We re-implement ViewCrafter using the  official code released by \cite{yu2024viewcrafter} to validate our easy/hard set splitting, with results shown as ViewCrafter* in \cref{tab:single-sparse}. We conduct comparisons with warping-based baselines, including LucidDreamer \cite{chung2023luciddreamer}, camera-conditional video generation model MotionCtrl \cite{wang2024motionctrl},  warp-image conditional ViewCrafter \cite{yu2024viewcrafter}, and multi-view diffusion model ZeroNVS \cite{sargent2023zeronvs}. We use the same point cloud rasterization as proposed in ViewCrafter \cite{yu2024viewcrafter} instead of depth-based warping to generate visual conditions for fair comparisons. Following \cite{yu2024viewcrafter}, we evaluate only the visual quality of images generated by multi-view diffusion without rendering novel views through 3D reconstruction. We report PSNR, SSIM, and LPIPS \cite{lpips} as evaluation metrics. Among these, PSNR is a traditional pixel-level metric that measures image similarity, which is significantly affected by viewpoint shifts. As such, PSNR reflects the accuracy of viewpoint control provided by our proposed \textit{visual-condition} in multi-view generation.

\noindent\textbf{Results.} The quantitative comparison results are presented  in the top rows of \cref{tab:single-sparse}. Only average metrics for the easy and hard sets are reported here, detailed values are available in the Appendix. The results for ViewCrafter* are comparable to those reported in its original paper, confirming successful alignment between our method and the baselines. Numerically, our approach  outperforms all baseline methods across all metrics. Specifically, compared to the re-implemented ViewCrafter, our approach achieves a 4.63 dB improvement, demonstrating its capability to generate high-quality novel views. PSNR further demonstrates significant gains, indicating our proposed \textit{visual-condition} enables  precise camera control. Qualitative results are shown in the top rows of \cref{fig:single-3d}. \ours generates high-quality, realistic content within minutes. Dispite limited visual cues provided by the warped images, our method produces more reliable and  realistic results with fewer artifacts. 

\noindent\textbf{Sparse Views to 3D.} We follow CAT3D \cite{gao2024cat3d} to generate dense multi-view images from 3, 6 and 9 sparse views input, and then conduct 3DGS reconstruction for novel view rendering. Qualitative and quantitative results are shown in \cref{tab:single-sparse} and \cref{fig:single-3d}, respectively. The experimental setting, comparison baselines, analysis and more results are provided in the Appendix.


% \begin{table*}[t]
% \caption{\textbf{Quantitative comparison of zero-shot novel view synthesis on Tanks-and-Temples\cite{Knapitsch2017tnt}, RealEstate10K\cite{zhou2018real10k} and CO3D\cite{reizenstein21co3d} dataset.}
% }
% \label{tab:comp_zero}
% \centering
% \resizebox{0.9\textwidth}{!}{%
% \huge
% \begin{tabular}{lcccccc}
% \cmidrule[\heavyrulewidth]{1-7}
%  \textbf{Dataset}
%  & \multicolumn{3}{c}{\textbf{Easy set}} & \multicolumn{3}{c}{\textbf{Hard set}} \\
%  \cmidrule(lr){2-4} \cmidrule(lr){5-7}
%  Method & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ \\ \cmidrule{1-7}

% \textbf{Tanks-and-Temples}\\
%  LucidDreamer~\cite{chung2023luciddreamer}   & 0.413 & 14.53 & 0.362  & 0.558 & 11.69 & 0.267 \\
%   ZeroNVS~\cite{sargent2023zeronvs}  & 0.482 & 14.71 & 0.380  & 0.569 & 12.05 & 0.309 \\
%  MotionCtrl~\cite{wang2024motionctrl}  &  0.400 &  15.34 &  0.427  &  0.473 &  13.29 &  0.384   \\
%   ViewCrafter & 0.194 & 21.26 & 0.655  & 0.283 & 18.07 & 0.563  \\ \cmidrule{1-7}    
%   ViewCrafter* & 0.221 & 20.39
%  & 0.648 & 0.289 & 17.86 & 0.584  \\
%   Ours & 0.167 & 25.01 & 0.756  & 0.214 & 22.52 & 0.714  \\
%   \cmidrule{1-7}    
% \textbf{RealEstate10K} \\
%  LucidDreamer~\cite{chung2023luciddreamer}     & 0.315 & 16.35 & 0.579  & 0.400 & 14.13 & 0.511   \\
%  ZeroNVS~\cite{sargent2023zeronvs}    & 0.364 & 16.50 & 0.577  & 0.431 & 14.24 & 0.535  \\ 
%  MotionCtrl~\cite{wang2024motionctrl}  & 0.341 & 16.31 & 0.604  & 0.386 & 16.29 & 0.587  \\
%   ViewCrafter (ours) & 0.145 & 21.81 & 0.796  & 0.178 & 22.04 & 0.798 
%   \\ \cmidrule{1-7}  
%   ViewCrafter* & 0.164 & 20.59
%  & 0.825 & 0.201 & 20.40 & 0.778  \\
%   Ours & 0.125 & 26.54 & 0.872  & 0.167 & 24.18 & 0.837  \\
%   \cmidrule{1-7}    
% \textbf{CO3D} \\
%  LucidDreamer~\cite{chung2023luciddreamer}     & 0.429 & 15.11 & 0.451  & 0.517 & 12.69 & 0.374   \\ 
%  ZeroNVS~\cite{sargent2023zeronvs}    & 0.467 & 15.15 & 0.463  & 0.524 &  13.31 &  0.426 \\
%  MotionCtrl~\cite{wang2024motionctrl}  & 0.393 & 16.87 & 0.529  & 0.443 & 15.46 & 0.502   \\
%  ViewCrafter (ours) & 0.243 & 21.38 & 0.687 & 0.324 & 18.96 & 0.641 \\
%  \cmidrule[\heavyrulewidth]{1-7}
%  ViewCrafter* & 0.331 & 20.12
%  & 0.703 & 0.348 & 18.02 & 0.653  \\
%   Ours & 0.225 & 25.23 & 0.781  & 0.276 & 23.33 & 0.748  \\
%   \cmidrule{1-7}    
% \end{tabular}
% }
% \end{table*}


% \begin{table*}[t]
% \centering
% \resizebox{0.9\textwidth}{!}{%
% \huge
% \begin{tabular}{lccccccccc}
% \cmidrule[\heavyrulewidth]{1-10}
%   \textbf{Dataset}
%  & \multicolumn{3}{c}{\textbf{3-view}} & \multicolumn{3}{c}{\textbf{6-view}} & \multicolumn{3}{c}{\textbf{9-view}} \\
%   Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ \cmidrule{1-10}

% % \textbf{RealEstate10K}\\
% %   Zip-NeRF$^*$~\cite{barron2023zip}     & 20.77 &  0.774 &  0.332 & 27.34 & 0.906 & 0.180  & 31.56 & 0.947 & 0.118 \\
% %    ZeroNVS$^*$~\cite{sargent2023zeronvs}    & 19.11 & 0.675 & 0.422 & 22.54 & 0.744 & 0.374  & 23.73 & 0.766 & 0.358 \\
% %   ReconFusion~\cite{wu2023reconfusion}         &  25.84 &  0.910 &  0.144 &  29.99 &  0.951 &  0.103 &  31.82 &  0.961 &  0.092   \\
% %    CAT3D & 26.78 & 0.917 & 0.132 & 31.07 & 0.954 & 0.092 & 32.20 & 0.963 & 0.082 \\
% %    Ours & 26.78 & 0.917 & 0.132 & 31.07 & 0.954 & 0.092 & 32.20 & 0.963 & 0.082
% %   \\ \cmidrule{1-10}
% \textbf{LLFF} \\
%   Zip-NeRF$^*$~\cite{zipnerf}     & 17.23 & 0.574 & 0.373 & 20.71 & 0.764 & 0.221 & 23.63 & 0.830 & 0.166 \\ 
%   MuRF \cite{xu2024murf} & 21.34 & 0.722 & 0.245 & 23.54 & 0.796 & 0.199 & 24.66 & 0.836 & 0.164 \\
%     FSGS \cite{zhu2025fsgs} & 20.31 & 0.652 & 0.288 & 24.20 & 0.811 & 0.173 & 25.32 & 0.856 & 0.136 \\
%     BGGS & 21.44 & 0.751 & 0.168 & 24.84 & 0.845 & 0.106 & 26.17 & 0.877 & 0.090 \\
%   ZeroNVS$^*$~\cite{sargent2023zeronvs}    & 15.91 & 0.359 & 0.512 & 18.39 & 0.449 & 0.438 & 18.79 & 0.470 & 0.416 \\
%   DepthSplat \cite{xu2024depthsplat} & 17.64 & 0.521 & 0.321 & 17.40 & 0.499 & 0.340 & 17.26 & 0.486 & 0.341 \\
%   ReconFusion~\cite{wu2024reconfusion}         &  21.34 &  0.724 &  0.203 &  24.25 &  0.815 &  0.152 &  25.21 &  0.848 &  0.134\\
%   CAT3D & 21.58 & 0.731 & 0.181 & 24.71 & 0.833 & 0.121 & 25.63 & 0.860 & 0.107 \\
%   Ours & 23.23 & 0.768 & 0.135 & 25.32 & 0.820 & 0.104 & 26.19 & 0.844 & 0.098
%       \\ \cmidrule{1-10}                
% \textbf{DTU} \\
%     Zip-NeRF$^*$~\cite{zipnerf}     &  9.18 & 0.601 & 0.383 &  8.84 & 0.589 & 0.370 &  9.23 & 0.592 & 0.364  \\
%     MuRF \cite{xu2024murf} & 21.31 & 0.885 & 0.127 & 23.74 & 0.921 & 0.095 & 25.28 & 0.936 & 0.084 \\
%     FSGS \cite{zhu2025fsgs} & 17.34 & 0.818 & 0.169 & 21.55 & 0.880 & 0.127 & 24.33 & 0.911 & 0.106 \\
%     BGGS & 20.71 & 0.862 & 0.111 & 24.31 & 0.917 & 0.073 & 26.70 & 0.947 & 0.052 \\
%  ZeroNVS$^*$~\cite{sargent2023zeronvs}    & 16.71 & 0.716 & 0.223 & 17.70 & 0.737 & 0.205 & 17.92 & 0.745 & 0.200  \\
%  DepthSplat \cite{xu2024depthsplat} & 15.59 & 0.525 & 0.373 & 15.061 & 0.523 & 0.406 & 14.87 & 0.478 & 0.451 \\
%  ReconFusion~\cite{wu2024reconfusion}         &  20.74 &  0.875 &  0.124 &  23.62 &  0.904 &  0.105 & 24.62 &  0.921 &  0.094\\
%   CAT3D & 22.02 & 0.844 & 0.121 & 24.28 & 0.899 & 0.095 & 25.92 & 0.928 & 0.073 \\
%   Ours & 28.04 & 0.884 & 0.073 & 29.09 & 0.900 & 0.066 & 29.99 & 0.911 & 0.059
% \\ \cmidrule{1-10}
%  % \textbf{CO3D} \\
%  %  Zip-NeRF$^*$~\cite{barron2023zip}     & 14.34 & 0.496 & 0.652 & 14.48 & 0.497 & 0.617 & 14.97 & 0.514 & 0.590  \\
%  %  ZeroNVS$^*$~\cite{sargent2023zeronvs}    & 17.13 & 0.581 & 0.566 & 19.72 & 0.627 & 0.515 &  20.50 &  0.640 &  0.500 \\ 
%  %  ReconFusion~\cite{wu2023reconfusion}         &  19.59 &  0.662 &  0.398 &  21.84 &  0.714 &  0.342 &  22.95 &  0.736 &  0.318 \\
%  %   CAT3D & 20.57 & 0.666 & 0.351 & 22.79 & 0.726 & 0.292 & 23.58 & 0.752 & 0.273 \\
%  %   Ours & 23.88 & 0.748 & 0.268 & 31.07 & 0.954 & 0.092 & 32.20 & 0.963 & 0.082
%  %  \\ \cmidrule{1-10}                      
% \textbf{Mip-NeRF 360} \\
%   Zip-NeRF$^*$~\cite{zipnerf}     & 12.77 & 0.271 &  0.705  & 13.61 & 0.284 & 0.663  & 14.30 & 0.312 & 0.633  \\ 
%   DepthSplat \cite{xu2024depthsplat}    & 13.85 & 0.254 & 0.621 & 13.82 & 0.260 & 0.636 & 14.48 & 0.288 & 0.602 \\
%   ZeroNVS$^*$~\cite{sargent2023zeronvs}    & 14.44 & 0.316 & 0.680 & 15.51 & 0.337 & 0.663 & 15.99 &  0.350 &  0.655 \\
%   ReconFusion~\cite{wu2024reconfusion}         &  15.50 &  0.358 &  0.585  &  16.93 &  0.401 &  0.544 &  18.19 &  0.432 &  0.511    \\
%   CAT3D & 16.62 & 0.377 & 0.515 & 17.72 & 0.425 & 0.482 & 18.67 & 0.460 & 0.460 \\
%   Ours & 17.35 & 0.442 & 0.422 & 19.03 & 0.517 & 0.365 & 19.89 & 0.542 & 0.335 \\
%  \cmidrule[\heavyrulewidth]{1-10}
% \end{tabular}
% }
% \caption{\textbf{Quantitative comparison of few-view 3D reconstruction}. }

% \label{tab:main_table}
% \end{table*}


\begin{table*}[t]
\vspace{-14pt}\
% \scriptsize
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{cccccccccc}
\toprule
        \textbf{Methods} & \multicolumn{3}{c}{\textbf{Tanks-and-Temples \cite{knapitsch2017tanks}}} & \multicolumn{3}{c}{\textbf{RealEstate10K \cite{real10k}}} & \multicolumn{3}{c}{\textbf{CO3D \cite{reizenstein2021common}}} \\
 % \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
 \midrule
                   \textbf{Single View}                         & PSNR $\uparrow$  & SSIM $\uparrow$  & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
\midrule
                   LucidDreamer \cite{chung2023luciddreamer}            & 13.11 & 0.314 & 0.485 & 15.24 & 0.545 & 0.357 & 13.90 & 0.412 & 0.473 \\
                   ZeroNVS \cite{sargent2023zeronvs}                 & 13.38 & 0.344 & 0.525 & 15.37 & 0.556 & 0.397 & 14.23 & 0.444 & 0.495 \\
                   MotionCtrl \cite{wang2024motionctrl}               & 14.31 & 0.405 & 0.436 & 16.30 & 0.596 & 0.363 & 16.16 & 0.515 & 0.418 \\
                   ViewCrafter \cite{yu2024viewcrafter}             & \cellcolor{orange!20}19.66 & \cellcolor{yellow!20}0.609 & \cellcolor{orange!20}0.238 & \cellcolor{orange!20}21.93 & \cellcolor{yellow!20}0.797 & \cellcolor{orange!20}0.161 & \cellcolor{orange!20}20.17 & \cellcolor{yellow!20}0.664 & \cellcolor{orange!20}0.283 \\
                   ViewCrafter* \cite{yu2024viewcrafter}             & \cellcolor{yellow!20}19.13 & \cellcolor{orange!20}0.616 & \cellcolor{yellow!20}0.255 & \cellcolor{yellow!20}20.49 & \cellcolor{orange!20}0.802 & \cellcolor{yellow!20}0.183 & \cellcolor{yellow!20}19.07 & \cellcolor{orange!20}0.678 & \cellcolor{yellow!20}0.339 \\
                   Ours                     & \cellcolor{red!20}23.76 & \cellcolor{red!20}0.735 &\cellcolor{red!20}0.191 & \cellcolor{red!20}25.36 & \cellcolor{red!20}0.854 & \cellcolor{red!20}0.146 & \cellcolor{red!20}24.28 & \cellcolor{red!20}0.765 &\cellcolor{red!20} 0.251 \\
\midrule
                   \textbf{Sparse Views (3 Views)}    & \multicolumn{3}{c}{\textbf{LLFF \cite{mildenhall2019local}}} & \multicolumn{3}{c}{\textbf{DTU \cite{dtu}}} & \multicolumn{3}{c}{\textbf{MipNeRF-360 \cite{barron2022mipnerf360}}} \\
 % \cmidrule(lr){2-11}
 \midrule
                   Zip-NeRF$^{\dag}$ \cite{zipnerf}            & 17.23 & 0.574 & 0.373 & 9.18  & 0.601 & 0.383 & 12.77 & 0.271 & 0.705 \\
                   MuRF \cite{xu2024murf}                    & 21.34 & 0.722 & 0.245 & \cellcolor{yellow!20}21.31 & \cellcolor{red!20}0.885 & 0.127 & -     & -     & -     \\
                   FSGS  \cite{zhu2025fsgs}                   & 20.31 & 0.652 & 0.288 & 17.34 & 0.818 & 0.169 & -     & -     & -     \\
                   BGGS \cite{han2024binocular}                    & \cellcolor{yellow!20}21.44 & \cellcolor{orange!20}0.751 & \cellcolor{orange!20}0.168 & 20.71 & 0.862 & \cellcolor{orange!20}0.111 & -     & -     & -     \\
                   ZeroNVS$^{\dag}$ \cite{sargent2023zeronvs}             & 15.91 & 0.359 & 0.512 & 16.71 & 0.716 & 0.223 & 14.44 & 0.316 & 0.680 \\
                   DepthSplat \cite{xu2024depthsplat}              & 17.64 & 0.521 & 0.321 & 15.59 & 0.525 & 0.373 & 13.85 & 0.254 & 0.621 \\
                   ReconFusion \cite{wu2024reconfusion}             & 21.34 & 0.724 & 0.203 & 20.74 & \cellcolor{yellow!20}0.875 & 0.124 & \cellcolor{yellow!20}15.50 & \cellcolor{yellow!20}0.358 & \cellcolor{yellow!20}0.585 \\
                   CAT3D \cite{gao2024cat3d}                   & \cellcolor{orange!20}21.58 & \cellcolor{yellow!20}0.731 & \cellcolor{yellow!20}0.181 & \cellcolor{orange!20}22.02 & 0.844 & \cellcolor{yellow!20}0.121 & \cellcolor{orange!20}16.62 & \cellcolor{orange!20}0.377 & \cellcolor{orange!20}0.515 \\
                   Ours                     & \cellcolor{red!20}23.23 & \cellcolor{red!20}0.768 & \cellcolor{red!20}0.135 & \cellcolor{red!20}28.04 & \cellcolor{orange!20}0.884 & \cellcolor{red!20}0.073 & \cellcolor{red!20}17.35 & \cellcolor{red!20}0.442 & \cellcolor{red!20}0.422 \\
\bottomrule
\end{tabular}%
}
\vspace{-0.3cm}
 \caption{\textbf{Quantitative Comparison of Single/Sparse Views Generation.} The top rows are results given single view as input, where ViewCrafter$^{*}$ indicates our re-implemented result. The bottom rows are novel view rendering quality given 3 views as input, where Zip-NeRF$^{\dag}$ and ZeroNVS$^{\dag}$ are modified versions with sparse views input as reported in CAT3D.} \label{tab:single-sparse}
 \vspace{-0.5cm}
\end{table*}



% \begin{table*}[t]
% \caption{\textbf{Quantitative comparison of zero-shot novel view synthesis on Tanks-and-Temples\cite{Knapitsch2017tnt}, RealEstate10K\cite{zhou2018real10k} and CO3D\cite{reizenstein21co3d} dataset.}
% }
% \label{tab:comp_zero}
% \centering
% \resizebox{0.9\textwidth}{!}{%
% \huge
% \begin{tabular}{lcccccc}
% \cmidrule[\heavyrulewidth]{1-7}
%  \textbf{Dataset}
%  & \multicolumn{3}{c}{\textbf{Easy set}} & \multicolumn{3}{c}{\textbf{Hard set}} \\
%  \cmidrule(lr){2-4} \cmidrule(lr){5-7}
%  Method & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ \\ \cmidrule{1-7}

% \textbf{Tanks-and-Temples}\\
%  LucidDreamer~\cite{chung2023luciddreamer}   & 0.413 & 14.53 & 0.362  & 0.558 & 11.69 & 0.267 \\
%   ZeroNVS~\cite{sargent2023zeronvs}  & 0.482 & 14.71 & 0.380  & 0.569 & 12.05 & 0.309 \\
%  MotionCtrl~\cite{wang2024motionctrl}  &  0.400 &  15.34 &  0.427  &  0.473 &  13.29 &  0.384   \\
%   ViewCrafter & 0.194 & 21.26 & 0.655  & 0.283 & 18.07 & 0.563  \\ \cmidrule{1-7}    
%   ViewCrafter* & 0.221 & 20.39
%  & 0.648 & 0.289 & 17.86 & 0.584  \\
%   Ours & 0.167 & 25.01 & 0.756  & 0.214 & 22.52 & 0.714  \\
%   \cmidrule{1-7}    
% \textbf{RealEstate10K} \\
%  LucidDreamer~\cite{chung2023luciddreamer}     & 0.315 & 16.35 & 0.579  & 0.400 & 14.13 & 0.511   \\
%  ZeroNVS~\cite{sargent2023zeronvs}    & 0.364 & 16.50 & 0.577  & 0.431 & 14.24 & 0.535  \\ 
%  MotionCtrl~\cite{wang2024motionctrl}  & 0.341 & 16.31 & 0.604  & 0.386 & 16.29 & 0.587  \\
%   ViewCrafter (ours) & 0.145 & 21.81 & 0.796  & 0.178 & 22.04 & 0.798 
%   \\ \cmidrule{1-7}  
%   ViewCrafter* & 0.164 & 20.59
%  & 0.825 & 0.201 & 20.40 & 0.778  \\
%   Ours & 0.125 & 26.54 & 0.872  & 0.167 & 24.18 & 0.837  \\
%   \cmidrule{1-7}    
% \textbf{CO3D} \\
%  LucidDreamer~\cite{chung2023luciddreamer}     & 0.429 & 15.11 & 0.451  & 0.517 & 12.69 & 0.374   \\ 
%  ZeroNVS~\cite{sargent2023zeronvs}    & 0.467 & 15.15 & 0.463  & 0.524 &  13.31 &  0.426 \\
%  MotionCtrl~\cite{wang2024motionctrl}  & 0.393 & 16.87 & 0.529  & 0.443 & 15.46 & 0.502   \\
%  ViewCrafter (ours) & 0.243 & 21.38 & 0.687 & 0.324 & 18.96 & 0.641 \\
%  \cmidrule[\heavyrulewidth]{1-7}
%  ViewCrafter* & 0.331 & 20.12
%  & 0.703 & 0.348 & 18.02 & 0.653  \\
%   Ours & 0.225 & 25.23 & 0.781  & 0.276 & 23.33 & 0.748  \\
%   \cmidrule{1-7}    
% \end{tabular}
% }
% \end{table*}


% \begin{table*}[t]
% \centering
% \resizebox{0.9\textwidth}{!}{%
% \huge
% \begin{tabular}{lccccccccc}
% \cmidrule[\heavyrulewidth]{1-10}
%   \textbf{Dataset}
%  & \multicolumn{3}{c}{\textbf{3-view}} & \multicolumn{3}{c}{\textbf{6-view}} & \multicolumn{3}{c}{\textbf{9-view}} \\
%   Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ \cmidrule{1-10}
% \textbf{LLFF} \\
%   Zip-NeRF$^*$~\cite{zipnerf}     & 17.23 & 0.574 & 0.373 & 20.71 & 0.764 & 0.221 & 23.63 & 0.830 & 0.166 \\ 
%   MuRF \cite{xu2024murf} & 21.34 & 0.722 & 0.245 & 23.54 & 0.796 & 0.199 & 24.66 & 0.836 & 0.164 \\
%     FSGS \cite{zhu2025fsgs} & 20.31 & 0.652 & 0.288 & 24.20 & 0.811 & 0.173 & 25.32 & 0.856 & 0.136 \\
%     BGGS & 21.44 & 0.751 & 0.168 & 24.84 & 0.845 & 0.106 & 26.17 & 0.877 & 0.090 \\
%   ZeroNVS$^*$~\cite{sargent2023zeronvs}    & 15.91 & 0.359 & 0.512 & 18.39 & 0.449 & 0.438 & 18.79 & 0.470 & 0.416 \\
%   DepthSplat \cite{xu2024depthsplat} & 17.64 & 0.521 & 0.321 & 17.40 & 0.499 & 0.340 & 17.26 & 0.486 & 0.341 \\
%   ReconFusion~\cite{wu2024reconfusion}         &  21.34 &  0.724 &  0.203 &  24.25 &  0.815 &  0.152 &  25.21 &  0.848 &  0.134\\
%   CAT3D & 21.58 & 0.731 & 0.181 & 24.71 & 0.833 & 0.121 & 25.63 & 0.860 & 0.107 \\
%   Ours & 23.23 & 0.768 & 0.135 & 25.32 & 0.820 & 0.104 & 26.19 & 0.844 & 0.098
%       \\ \cmidrule{1-10}                
% \textbf{DTU} \\
%     Zip-NeRF$^*$~\cite{zipnerf}     &  9.18 & 0.601 & 0.383 &  8.84 & 0.589 & 0.370 &  9.23 & 0.592 & 0.364  \\
%     MuRF \cite{xu2024murf} & 21.31 & 0.885 & 0.127 & 23.74 & 0.921 & 0.095 & 25.28 & 0.936 & 0.084 \\
%     FSGS \cite{zhu2025fsgs} & 17.34 & 0.818 & 0.169 & 21.55 & 0.880 & 0.127 & 24.33 & 0.911 & 0.106 \\
%     BGGS & 20.71 & 0.862 & 0.111 & 24.31 & 0.917 & 0.073 & 26.70 & 0.947 & 0.052 \\
%  ZeroNVS$^*$~\cite{sargent2023zeronvs}    & 16.71 & 0.716 & 0.223 & 17.70 & 0.737 & 0.205 & 17.92 & 0.745 & 0.200  \\
%  DepthSplat \cite{xu2024depthsplat} & 15.59 & 0.525 & 0.373 & 15.061 & 0.523 & 0.406 & 14.87 & 0.478 & 0.451 \\
%  ReconFusion~\cite{wu2024reconfusion}         &  20.74 &  0.875 &  0.124 &  23.62 &  0.904 &  0.105 & 24.62 &  0.921 &  0.094\\
%   CAT3D & 22.02 & 0.844 & 0.121 & 24.28 & 0.899 & 0.095 & 25.92 & 0.928 & 0.073 \\
%   Ours & 28.04 & 0.884 & 0.073 & 29.09 & 0.900 & 0.066 & 29.99 & 0.911 & 0.059
% \\ \cmidrule{1-10}                  
% \textbf{Mip-NeRF 360} \\
%   Zip-NeRF$^*$~\cite{zipnerf}     & 12.77 & 0.271 &  0.705  & 13.61 & 0.284 & 0.663  & 14.30 & 0.312 & 0.633  \\ 
%   DepthSplat \cite{xu2024depthsplat}    & 13.85 & 0.254 & 0.621 & 13.82 & 0.260 & 0.636 & 14.48 & 0.288 & 0.602 \\
%   ZeroNVS$^*$~\cite{sargent2023zeronvs}    & 14.44 & 0.316 & 0.680 & 15.51 & 0.337 & 0.663 & 15.99 &  0.350 &  0.655 \\
%   ReconFusion~\cite{wu2024reconfusion}         &  15.50 &  0.358 &  0.585  &  16.93 &  0.401 &  0.544 &  18.19 &  0.432 &  0.511    \\
%   CAT3D & 16.62 & 0.377 & 0.515 & 17.72 & 0.425 & 0.482 & 18.67 & 0.460 & 0.460 \\
%   Ours & 17.35 & 0.442 & 0.422 & 19.03 & 0.517 & 0.365 & 19.89 & 0.542 & 0.335 \\
%  \cmidrule[\heavyrulewidth]{1-10}
% \end{tabular}
% }
% \caption{\textbf{Quantitative comparison of few-view 3D reconstruction}. }

% \label{tab:main_table}
% \end{table*}


% appendix
% \subsection{Sparse views to 3D}
% \label{exp: sparse}
% \noindent\textbf{Experimental Setting.} We further extend our model to the sparse-view reconstruction task. We conduct evaluations on the following three datasets, including LLFF \cite{mildenhall2019local}, DTU \cite{dtu}, and Mip-NeRF 360 \cite{barron2022mipnerf360}, where LLFF and DTU are dataset of forward-facing scenes, and MipNeRF-360 contains a complex central object or area and a detailed background. We compare our methods with various few-shot 3D reconstruction baselines including optimization-based MuRF \cite{xu2024murf}, FSGS \cite{zhu2025fsgs}, and BGGS \cite{han2024binocular}; diffusion-based including CAT3D \cite{gao2024cat3d}, ZeroNVS (modified from single-view input to multiview input) \cite{sargent2023zeronvs}, and ReconFusion \cite{wu2024reconfusion}; and feed-forward DepthSplat \cite{xu2024depthsplat}. We follow the same evaluation protocol with \cite{niemeyer2022regnerf,zhu2025fsgs, wu2024reconfusion} where the 3, 6, 9 views are selected as input. For few-shot reconstruction, we first follow CAT3D \cite{gao2024cat3d} to generate dense multi-view images from sparse views input, and then conduct 3DGS reconstruction with pose optimization as proposed in \cref{sec: 3dgs} to render test views for evaluation. We also report PSNR, SSIM, LPIPS \cite{lpips} to evaluate the novel view synthesis.


\begin{figure}[tb]
% \vspace{-3pt}
\centering
\includegraphics[width=0.45\textwidth]{images/exp2.pdf}
\vspace{-8pt}
\caption{\textbf{Qualitative Comparison of Single/Sparse View Generation.} Top three rows are results with a single view input. Bottom two rows are novel view renderings from 3DGS, where Ours is trained on dense multi-view generation given 3 views as input. Our method outperformed other baselines in capturing high-frequency details, such as text and stairs. {\color{blue}Best viewed in zoom}.}
\vspace{-16pt}
\label{fig:single-3d}
\end{figure}

% 

% appendix
% \noindent\textbf{Results.} The quantitative comparison results given 3 views as input are presented in the bottom rows in \cref{tab:single-sparse}, the remaining results for 6, 9 views setting are refered to the Appendix. The 3DGS model trained on dense multi-view images generated by \ours outperformed state-of-the-art reconstruction models in novel view rendering, demonstrating that \ours can provide high-quality and highly consistent multi-view support for 3D reconstruction without additional constraints. Compared to ReconFusion \cite{wu2024reconfusion} and CAT3D \cite{gao2024cat3d}, which also apply diffusion priors for sparse view reconstruction, our method achieved significant improvements, demonstrating the effectiveness of our model at scale. The qualitative visual comparisons are shown in \cref{fig:single-3d}, our NVS results exhibit fewer floating artifacts, indicating that \ours is capable of generating more consistent and high-quality multi-view images.

\vspace{-5pt}
\subsection{Ablation Study}
\vspace{-5pt}
\label{exp: ablation}
\noindent\textbf{Scaling up Data.}  We first investigate the impact of training data by ablating different ratios of our training dataset. We train the model with 10\%, 20\%, 40\%, 80\%, and 100\% of the training set, and then test the performance of single-view generation on RealEstate10K, resulting in 19.32, 21.04, 22.57, 24.08 and 25.01 in term of PSNR,  respectively. Meanwhile, we train the model with unfiltered data, and we observe that the generated content often exhibited movement or deformation, resulting in a significant degradation of the performance (PSNR:19.55). We analyzed that the cause of this phenomenon is that most of the content in the source video cannot remain stationary and geometrically invariant across frames, resulting in a weakening of multi-view consistency. In combination, we demonstrate that data quality and diversity play an essential role when training large-scale MVD model.


\noindent\textbf{\textit{Visual-condition}.} Excluding the benefits of data scaling, we investigate  the effectiveness of our \textit{visual-condition} on pose-free data. Previous work \cite{yu2024viewcrafter} has demonstrated that warped images can serve  as a pivot condition to guide the model to generate the target viewpoint. However, due to the reliance on the annotated camera to control the projection and unprojection, warp-based conditions are inherently unscalable. Therefore, we compare the model's ability to control cameras conditioned on pose-free \textit{visual-condition} and conditioned on warped images. Specifically, we extract a subset of  MVImageNet \cite{yu2023mvimgnet} for training and testing. 
\begin{wraptable}{r}{0.3\textwidth}
\scriptsize
\vspace{-0.4cm}
\resizebox{0.3\textwidth}{!}{%
\begin{tabular}{cccc}
\toprule
Model &  LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$  \\
\midrule
MV-Posed &  0.182 & 26.21 & 0.822  \\
MV-UnPose &  0.443 & 16.14 & 0.521  \\
MV-UnposeT &  0.194  & 25.56 &  0.811  \\
\bottomrule
\end{tabular}
}
\vspace{-0.2cm}
\caption{\textbf{Ablation on \textit{visual-condition}.}}
\vspace{-0.6cm}
\label{tab:abl_Vt}
\end{wraptable}
For each multi-view sequence in training set, we select the point cloud of the first frame and render it into the subsequent 5 camera planes along the camera trajectory, based on the 3D annotations in the dataset. We obtain warped images and form pairs with the ground-truth multi-views to train a MVD model, referred to as MV-Posed. With the same experimental settings (training set, network architecture, batch size and predicted sequence length), we train an additional model without any 3D annotations, except for the modification of warp condition to the time-dependent \textit{visual-condition} $V_t$ described in Sec.\ref{sec:model}, called MV-UnposeT. Meanwhile, we use randomly masked multiple views as condition to train the model as another baseline, called MV-Unpose. 

The results are reported in Tab.\ref{tab:abl_Vt} and Fig.\ref{fig:Vt-ablation}, where the performance of MV-Posed and MV-Unpose is comparable. In contrast, MV-Unpose struggles to handle the gap between the warped image and masked images, in the case of geometric distortion and self-obscuration. These results suggest that the \textit{visual-condition} provides a viable alternative to 3D-reliant warped condition. 
Despite a significant domain gap between $V_t$ and warp images as shown in Fig.\ref{fig:Vt-ablation}, our model robustly handles this discrepancy, thanks to the time-dependent nature of the condition.
   



\begin{figure}[tb]
\centering
\includegraphics[width=0.47\textwidth]{images/ablation_1.pdf}
\vspace{-0.3cm}
\caption{Top: Qualitative ablation of \textit{visual-condition}; Bottom: As timestep decreases, visualize the trend of \textit{visual-condition}.}
\label{fig:Vt-ablation}
\vspace{-0.6cm}
\end{figure}

==> sec/5_conclusion.tex <==
\vspace{-7pt}
\section{Conclusion}
\vspace{-4pt}
% 提升3D生成的上限。 通过只看video就可以get 3D
% We present, \ours , a scalable framework with the potential to enable data scaling to any arbitrary size. Specifically, the automated filtering pipline indicates the potential of training data to evolve alongside the progress of the Internet. Visual condition frees the MVD model from its reliance on camera annotations, enabling multi-view prediction at scale and realizing the concept of 'Get 3D by solely Seeing'. We show that the robust 3D priors learned by \ours enable a range of 3D creation applications, such as single-view generation, sparse view reconstruction, and 3D editing in open-world scenarios. We believe \ours  provides a new direction for pushing the upper bound of 3D generative models through dataset scaling. We hope our efforts will encourage the 3D research community to pay more attention to large-scale unposed data, bypassing the costly 3D data barrier, and enabling chase the gap with powerful closed-source 3D generative models.


%We develop a scalable 3D generation model \ours, from the perspective of dataset scaling up, and provide a systematic solution that include: 1) \textit{automated data curation pipeline}: through which, we curate a new dataset, \data. It demonstrates the potential to evolve alongside the growing volume of Internet data;  2) \textit{Visual-condition}： it eliminates the need for camera annotations, enabling MVD model training at scale, which  aligns with the concept of 'Get 3D by solely Seeing'.  3) \textit{visual conditional 3D generation}: we introduce a novel 3D generation framework using the proposed \ours, which supports long-sequence novel view generation along complex camera trajectories.


We propose a scalable 3D generation framework from the perspective of  dataset scaling, offering  a systematic solution that includes: 1) a new dataset, \data, curated via an automated pipeline, with the potential to evolve with the growing volume of Internet data. 2) a new model, \ours, capable of scalable training without pose annotations, aligning with the concept of `Get 3D by solely Seeing'. 3) a novel \ours-based 3D generation framework that supports long-sequence view generation with complex camera trajectories.
 We show that the 3D priors learned by \ours enable a range of 3D creation applications, including single-view generation, sparse view reconstruction, and 3D editing in open-world scenarios. We believe \ours  provides a new direction for pushing the upper bound of 3D generation through dataset scaling. We hope our efforts will encourage the 3D research community to pay more attention to large-scale unposed data, bypassing the costly 3D data barrier and chasing the gap with powerful closed-source 3D solutions.







\clearpage

==> sec/demo.tex <==
\makeatletter
\let\@oldmaketitle\@maketitle
\renewcommand{\@maketitle}{\@oldmaketitle
\vspace{-0.6cm}
\includegraphics[width=\linewidth]{images/top.pdf}
\centering
\captionsetup{hypcap=false}
\captionsetup{skip=2pt}
\captionof{figure}{ 
Benefiting from the proposed web-scale dataset \data, \ours enables both object- and scene-level 3D creation, including (text-) image-to-3D, sparse-view-to-3D, and 3D editing. It can also be used for Gaussian Splatting to extract meshes or render images.
\vspace{10pt}
}\label{fig:demo}
}
\makeatother

% Benefit from proposed web-scale 3D-aware video dataset, \data, \ours enables both object and scene-level 3D creation, including (text-)image-to-3D,
% sparse-view-to-3D, and 3D editing. It can also be used for Gaussian Splatting to extract meshes or render images from arbitrary viewpoints.

==> sec/method_v1.tex <==
\section{Method}

% \begin{table*}[ht]
% \centering
% \resizebox{0.8\textwidth}{!}{
% \begin{tabular}{c|c|ccc|cc}
% \toprule
% Website   & Domain    & \# Source Videos         & \# Source Clips           & Total Time (hrs)         &\#Filtered Videos  & Filtered Time (hrs) \\ \midrule
% Pexels   & Open      & 1.27M        & 6.18M          & 101.77K          & 0.61M         & 9.96K             \\
% Artgrid  & Open      & 1.03M        &  3.94M        &  92.49K            &  0.54M        & 8.77K      \\
% Airvuz   & Drone    & 0.63M         &  5.10M        &  94.75K                &  0.54M        & 8.72K                    \\
% Skypixel & Landscape & 1.27M        &  10.27M       &   105.47K            & 0.61M           & 8.82K                 \\ \midrule
%   \textbf{Total}    & Open       & 4.20M       & 25.48M        & 394.48K              & \textbf{2.30M  }          & 36.27K  \\
% \bottomrule
% \end{tabular}
% }
% \begin{table}[ht]
% \centering
% \resizebox{0.5\textwidth}{!}{
% \begin{tabular}{c|c|cc|ccc}
% \toprule
% Website   & Domain    & \# Src. Vids     & Total Hrs.   &\#Fil. Vids   &\#Fil. Clips & Fil. Hrs. \\ \midrule
% Pexels   & Open      &  6.18M                & 101.77K          & 0.61M    & 2.65M        & 9.96K             \\
% Artgrid  & Open      & 3.94M               &  92.49K            &  0.54M     &  1.10M       & 8.77K      \\
% Airvuz   & Drone    &  5.10M                &  94.75K          &  0.54M      &  5.87M   & 8.72K                    \\
%     Skypixel & Landscape & 10.27M          &   105.47K            & 0.61M      & 6.37M     & 8.82K                 \\ \midrule
%   \textbf{Total}    & Open    & 25.48M         & 394.48K                & \textbf{2.30M  }    & \textbf{15.99M  }          & 36.27K  \\
% \bottomrule
% \end{tabular}
% }
% \caption{\textbf{\textit{WebVi3D} Dataset}. Sourced from four open websites and filtered through four steps, we curate approximately 2.30M videos, which are divided into 15.99M clips featuring  temporally static scenes with large-range viewpoint, supporting large-scale MVD model training.}
% \label{tab:data_stat}
% \end{table}

% \todo{The primary objective of this work is to build a robust 3D generation model through dataset scaling.}
The primary objective of this work is to build a robust 3D generative model from the perspective of dataset scaling-up.
Previous works \cite{deitke2023objaverse, tung2024megascenes,reizenstein2021common} laboriously collect 3D data from designed artists, stereo matching, or Structure from Motion (SfM), which are often costly, time-intensive,  and in some cases, infeasible.   In contrast, multi-view images offer a highly scalable alternative, as they can be automatically extracted from the vast and rapidly growing Internet videos. Using multi-view prediction as a pretext task, we show that learned 3D priors enable a range of 3D creation applications, such as single view generation, sparse views reconstruction, and 3D editing in open-world scenarios.

% \vspace{2pt}
In the following sections, we outline our approach. Section \ref{sec:data} details the data curation pipeline, which selects static scenes with sufficient multi-view observations from raw video footage. Section \ref{sec:model} introduces our visual-conditional multi-view diffusion model, which effectively learns general 3D priors from pose-free videos. Finally, Section \ref{sec:3DGen} demonstrates a new visual-conditional 3D generation framework utilizing  a warping-based pipeline.

\subsection{Video Data Curation} \label{sec:data}

% Pretraining on high-quality large-scale video data with 3D features is essential for our model to produce accurate and reliable 3D priors. A well-defined 3D video has two properties: \textbf{a) the contents in the scene remain static temporally}, and \textbf{b) the camera's ego-motion produces large multi-view baselines}. The first one ensures consistent scene geometry across different viewpoints in the video, which facilitate our model to learn accurate 3D priors. While the dynamic areas create biases in the model's comprehension of 3D, thus degrading the generation accuracy. The second provides sufficient 3D observations from multiple viewpoints, thereby providing our model with a more comprehensive understanding of the 3D world. Conversely, \todo{when training on multi-view videos with smaller baselines, the limited 3D observations in the data provide insufficient visual hints for the model to actually learn adequate 3D priors imposed by the camera movement. This limitation causes the model training to bias towards fitting the adjacent input views, resulting in “lower” training loss.}
% \begin{table*}[ht]
% \centering
% \resizebox{0.8\textwidth}{!}{
% \begin{tabular}{c|cccc|cc}
% \toprule
% Source   & Domain    & \#Videos         & \#Clips           & Total Time (hrs)         &\#Filtered Clips  & Filtered Time (hrs) \\ \midrule
% Pexels   & Open      & 1,274,649      & 6,181,091          &   101,765.49          & 606,566         & 9,961.70              \\
% Artgrid  & Open      & 1,030,430        &  3,936,872        &  92,487.55            &  541,327        & 8,767.93      \\
% Airvuz   & Drone & 633,310         &  5,101,363     &  94,749.20                &  538,894        & 8,721.73                     \\
% Skypixel & Landscape & 1,268,614       &  10,265,262     &   105,468.26            & 605,554           & 8,821.93                 \\ \midrule
% Total    & Open         & 4,207,003       & 25,484,588     & 394,470.5              &\colorbox{pink!50} {2,292,341}            & 36,273.29  \\
% \bottomrule
% \end{tabular}
% }
% \caption{\textbf{Our WebVi3D Dataset}. Sourced from four open platforms and filtered through four steps, it contains approximately 2.3M video clips with temporally static scenes and large viewpoint variations, supporting large-scale MVD model training.}
% \label{tab:data_stat}
% \end{table*}

High-quality, large-scale video data rich in 3D knowledge is essential  for learning  accurate and reliable 3D priors. 
A well-defined 3D-aware video clip should exhibit two key properties: \textbf{a) temporally static scene content } and \textbf{ b) large viewpoint variation caused by the camera's ego-motion.} 
The first property ensures consistent 3D geometry across different viewpoints, while the dynamic content alters the scene’s geometry, introduces biases that may degrade generation performance (see \cref{fig:data}a-Row1). The second property ensures sufficient 3D observations from multiple viewpoints. If the model is trained on videos with limited viewpoint variation (see \cref{fig:data}a-Row2), it may focus primarily on views adjacent to the reference view, rather than developing a comprehensive 3D understanding.
 % enabling the model to learn reliable  3D priors

% the model \todo{will be prone to fall into a local minima, where it tends to generate images that are close to the reference viewpoint that achieves lower training loss}, without actually learning the 3D priors imposed by the camera movement.
% 其中第一个xxx，第二个会xxxx。
% 为了获取到大量的3D数据，我们收集了各种各样的视频数据用于我们的模型训练。但是挑出来是不trivial的。

% \vspace{4pt}
% Current open-source dataset that meets the definition, such as MVImgNet \cite{yu2023mvimgnet}, RealEstate10K \cite{real10k}, and DL3DV \cite{ling2024dl3dv}, contains \todo{a limited number of multi-view frames}, which hinders the training at scale. 

To obtain a massive volume of 3D data, we collect approximately  \textbf{25.48M} open-sourced raw videos, totaling \textbf{44.98 years} from the Internet, covering a wide range of categories, such as landscapes, drones, animals, plants, games, and actions. Specifically, our dataset is sourced from four websites: Pexels \cite{pexels}, Artgrid \cite{artgrid}, Airvuz \cite{airvuz}, and Skypixel \cite{skypixel}. We follow Emu3 \cite{wang2024emu3} to split the videos with PySceneDetect \cite{pyscene} to identify content changes and fade-in/out events. Additionally, we remove clips with excessive text using PaddleOCR \cite{paddle}. The detailed composition of our \textit{WebVi3D} dataset is presented in \cref{tab:data_stat}.

% \todo{whether add previous 3D dataset info or not?}
% \begin{table}[!ht]
% \centering
% \resizebox{0.48\textwidth}{!}{
% \begin{tabular}{ccccccc}
% \toprule
% Source   & Domain    & \#Videos         & \#Clips                   & Total Duration                                                &\# Filtered Clips           & Filtered Duration \\ \midrule
% Pexels   & Open      & 729,489 +545160      & 729,489 +5451602          &   10,905.46h,554.4d,1.24y+90860.03h,3785.84d,10.36y            & 86,995 + 519571         & 1300.52h, ratio 0.12+8661.18h              \\
% Artgrid  & Open      & 485,270 +545160        &  485,270 +5451602        &  1,627.52h,67.81h,0.19y+90860.03h,3785.84d,10.36             &  21,756  +519571      & 106.75h,4.45d.0.01y, ratio0.065+8661.18h      \\
% Airvuz   & Landscape & 88,150  +545160         &  1,649,761 +5451602     &  3,889.17h,162d,0.44y+90860.03h,3785.84d,10.36y              &  19,323  +519571        & 60.55h,ratio 0.012+8661.18h                     \\
% Skypixel & Landscape & 723,454 +545160        &  7,813,660 +5451602     &   14,608.23h,608d,1.67y+90860.03h,3785.84d,10.36y            & 85,983  +519571           & 160.75h,ratio 0.011+8661.18h                 \\ \midrule
% Total    & -         & xx                   & xx                         & xx              & xx                  &                \\
% \bottomrule
% \end{tabular}
% }
% \caption{Initial Dataset Statistic.}
% \label{tab:data_stat}
% \end{table}

\begin{table}[ht]
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{c|c|cc|ccc}
\toprule
Website   & Domain    & \# Src. Vids     & Total Hrs.   &\#Fil. Vids   &\#Fil. Clips & Fil. Hrs. \\ \midrule
Pexels   & Open      &  6.18M                & 101.77K          & 0.61M    & 2.65M        & 9.96K             \\
Artgrid  & Open      & 3.94M               &  92.49K            &  0.54M     &  1.10M       & 8.77K      \\
Airvuz   & Drone Shot    &  5.10M                &  94.75K          &  0.54M      &  5.87M   & 8.72K                    \\
    Skypixel & Landscape & 10.27M          &   105.47K            & 0.61M      & 6.37M     & 8.82K                 \\ \midrule
  \textbf{Total}    & Open    & 25.48M         & 394.48K                & \textbf{2.30M  }    & \textbf{15.99M  }          & 36.27K  \\
\bottomrule
\end{tabular}
}
\vspace{-6pt}
\caption{\textbf{\textit{WebVi3D} Dataset}. Sourced from four open websites, we curate  $\sim$2.30M videos, which are divided into 15.99M clips featuring temporally static scenes with large-range viewpoint.}
\vspace{-8pt}
\label{tab:data_stat}
\end{table}

% \vspace{2pt}
However, identifying 3D-aware videos presents a nontrivial challenge.
Since most videos are derived from real-world footage, such videos often contains dynamic scenes or  small camera movement. 
To address this, we propose a sophisticated pipeline to automatically select relevant, high-quality 3D data  by leveraging priors from instance segmentation \cite{maskrcnn}, optical flow \cite{raft}, and pixel tracking \cite{cotracker}. This pipeline consists of four core steps: 1) Temporal-Spatial Downsampling, 2) Semantic-Based Dynamic Recognition, 3) Non-Rigid Dynamic Filtering, and 4) Tracking-Based Small Viewpoint Filtering. The detailed curation pipeline can be found at Appendix.
% \paragraph{a. Temporal-Spatial Downsampling.}
% We downsample each video in time and space thereby increasing the efficiency. We use the final resolution of 480p and the temporal downsample rate is factor of two. It is worth noting that our downsampling here is only for more efficient data filtering, and we use additional data processing during pretraining. 
% \vspace{-10pt}

% \textbf{1) Temporal-Spatial Downsampling.}
% To improve data filtering efficiency, we first downsample each video clip both temporally and spatially. The final resolution is set to 480p, and the temporal downsampling rate is set to 2. Note that this downsampling operation is applied  only during data curation, not during model training. \textbf{2) Semantic-Based Dynamic Recognition.} We employ instance segmentation model, Mask R-CNN \cite{maskrcnn}, to generate motion masks for potential dynamic objects, such as humans, animals, sports. A threshold is applied to filter videos based on the proportion of frames containing such objects, as these are more likely dynamic scenes.  \textbf{3) Non-Rigid Dynamic Filtering.} To filter out videos with dynamic regions precisely, we use offline optical flow estimation \cite{raft} to obtain dense matching, which enables us to identify non-rigid motion masks in video frames. These masks are then analyzed depending on their location and extent to further determine whether the video is a dynamic one. \textbf{4) Tracking-Based Small Viewpoint Filtering.} We focus on videos with large viewpoint variations. We propose to track the motion trajectory of key points across different frames, and calculate  the radius of the minimum outer tangent circle of the trajectory, filtering out videos with small trajectory radius. More detailed data curation processes are provided in the Appendix.

Finally, we curate approximately 320M multi-view images from 15.99M video clips with static content and sufficient multi-view observations (see Fig.\ref{fig:data}b). To better validate the effectiveness of our data acquisition method, we randomly select 10,000 video clips for human annotation, of which 8,859 were labeled as 3D-aware, representing 88.6\% of the total. This indicates that our pipeline effectively filtered 3D videos from massive video data. As the volume of Internet videos continues to grow, we can continually use this pipeline to acquire more 3D data, thereby expanding our data support over time.

%We randomly selected 10,000 video clips for users to annotate after data screening, and found that the number of 3D video annotations was 88,59 videos with a ratio of 88.6\%, indicating that our proposed method effectively preserves 3D videos.
% \subsubsection{Step 1: Temporal-Spatial Downsampling}
% We downsample each video in time and space thereby increasing the efficiency. Temporally, we downsample by a factor of two, retaining an image every two frames for subsequent identification. Spatially, for each segmented image, it is different in aspect ratio between images in different videos. To ensure that the original content is as reliable as possible after downsampling, we downsample a different multiplier according to the size of the original resolution to achieve comparable resolution. In this paper, we use the final resolution of 480p. It is worth noting that our downsampling here is only for more efficient data filtering, and we use additional data processing during pretraining.
% \subsubsection{Step 2: Semantic-Based Dynamic Filter}
% We process the content recognition on each image frame. We follow \cite{liu2023robust} to utilize the off-the-shelf instant segmentation model Mask R-CNN \cite{maskrcnn} to generate coarse motion masks $\mathcal{M}_m$ of humans, animals, sports, etc. If the number of frames with motion mask is more than half of the total number of frames in the current video, we consider that there is a higher probability of dynamic regions in this video, and we remove this in the subsequent processing.

\begin{figure}[tb]
\centering
\includegraphics[width=0.48\textwidth]{images/data3.pdf}
\vspace{-24pt}
\caption{\small(a-Row1): Internet videos  often contain dynamic content that alters scene geometry across views; (a-Row2): Source videos with limited camera movement provide insufficient multi-view priors; (b) Our \textit{\data} comprises 3D-aware Videos with static scenes and diverse camera trajectories.}
\vspace{-14pt}
\label{fig:data}
\end{figure}

% \subsubsection{Step 3: Non-Rigidity Dynamic Recognition}
% After coarse filtering out videos with common dynamic objects, we apply a more precise strategy to filter out videos with non-rigidity dynamic regions, such as drifting water or swaying trees \cite{rodynrf}. Following \cite{rodynrf}, we first apply pretrained RAFT \cite{raft} to generate optical flow between every two extracted frames, we then calculate and threshold the Sampson distance to obtain a non-rigid motion mask $\mathcal{M}_s$, where the Sampson distance is the distance of each pixel to the estimated epipolar line \cite{}. A higher number of these mask pixels represents a higher probability of motion occurring in the current frame. However, it is unreliable to rely solely on this condition to determine whether there is a motion, because most of our data are collected from real shots, where people usually place the dynamic object of interest in the center of the imaging plane, and these moving regions may not very large. Therefore, based on this assumption, we additionally consider the location of the dynamic mask appears. Therefore, we propose a dynamic score $\mathcal{S}$ to evaluate the dynamic probability of the current frame. Denote $H, W$ is the height and weight of an image, $W'=0.25\times W, H'=0.25\times H$ is the central start of an image, the proportion $\Theta_i$ of the entire image occupied by the mask, and the central proportion $\Theta_c$ of the central area can be calculated as:
% \begin{equation}
% \Theta_i = \frac{\Sigma_{u,v=0}^{W,H}\mathcal{M}_s(u,v)}{H\times W}, \\
% \Theta_c = \frac{\Sigma_{u,v=W', H'}^{W-W',H-H'}\mathcal{M}_s(u,v)}{H/2\times W/2}.
% \end{equation}
% The dynamic score can be formulated as:
% \begin{equation}
% \mathcal{S}_i =\begin{cases}
%      2, & \Theta_i \geq 0.12 \And \Theta_c \geq 0.35 \\
%       1.5, &\Theta_i \geq 0.12 \And 0.2 \leq \Theta_c < 0.35 \\
%       1, &\Theta_i < 0.12 \And 0.2 \leq \Theta_c < 0.35 \\
%       0.5, &\Theta_i < 0.12 \And \Theta_c < 0.2 
% \end{cases}.
% \end{equation}
% % After that, we determine whether a dynamic region appears in the current frame based on the number of pixels and the overall position of the mask. We notice that most of the dynamic regions in casually captured videos are distributed in the central area of the image. 
% % \sigma_s(\mathcal{M}_s)=\Sigma_{u,v=0}^{W,H}\mathcal{M}_s(u,v), \\
% % \sigma_c(\mathcal{M}_s)=\Sigma_{u,v=W', H'}^{W-W',H-H'}\mathcal{M}_s(u,v)
% This strategy enhances the focus of the dynamic region in the center of the image, which increases the accuracy of filtering. We then calculate the final dynamic score $\mathcal{S}$ of the whole sequence as:
% \begin{equation}
%     \mathcal{S} = \Sigma_{i=0}^N \mathcal{S}_i,
% \end{equation}
% where $N$ represents the number of extracted frames. When $\mathcal{S} >= 0.25 \times N$, we filter out this sequence as dynamic video.

% \subsubsection{Step 4: Tracking-Based Small Baseline Filter}
% We obtained videos where the scene contents remained static in previous steps. As we mentioned above, we still need to obtain videos consisting of multi-view images with a large camera baseline. Our core idea is to track the motion trajectory of key points in an image by tracking them in different frames and determining the radius of the minimum outer tangent circle of the trajectory. If a large number of circle radii are smaller than the threshold, it indicates that the camera trajectory of this video is small, and it is not possible to extract a multi-view image with a larger baseline. The procedure combines keypoint extraction, trajectory tracking, and circle fitting using RANSAC (Random Sample Consensus).

% We further downsample the previously extracted video frames by taking every fourth frame to reduce computational complexity. Then, we leverage SuperPoint \cite{superpoint} to extract keypoints $\mathbf{K} \in \mathbb{R}^{N \times 2}$ on the first frame, where $N=100$ is the number of detected keypoints, are used to initialize tracking. Keypoints are tracked through all frames using pretrained CoTracker \cite{cotracker}. It generates trajectories and the keypoints' visibility over time as:
% \begin{equation}
% \mathbf{T}_{\text{pred}}, \mathbf{V}_{\text{pred}} = \text{CoTracker}(\mathbf{I}, \text{queries}=\mathbf{K}),
% \end{equation}
% where $\mathbf{I}$ is the input frames, $\mathbf{T}_{\text{pred}} \in \mathbb{R}^{1 \times T \times N \times 2}$ represents the tracked positions of each keypoint across time steps, and $\mathbf{V}_{\text{pred}} \in \mathbb{R}^{1 \times T \times N \times 1}$ indicates the visibility of each point. For each tracked keypoint, a circle fitting method is applied to its trajectory. We select only those frames where the keypoint is visible $(\mathbf{V}_{\text{pred}} = 1)$. Let $\mathbf{T}_{\text{visible}} \in \mathbb{R}^{M \times 2}$ be the filtered points, where $M$ is the number of visible points, we apply the RANSAC-based circle fitting algorithm to $\mathbf{T}_{\text{visible}}$ to find the circle’s center $\mathbf{c} = (c_x, c_y)$ and radius  $r$:
% \begin{equation}
% \mathbf{c}, r = \text{RANSAC}(\mathbf{T}_{\text{visible}}),
% \end{equation}
% the RANSAC algorithm selects random subsets of three points to define candidate circles, computes inliers, and optimizes for the circle with the highest inlier count and smallest radius. Finally, we count the number of circles with a radius smaller than a threshold  $r \leq 20$:
% \begin{equation}
% \text{count} = \sum_{i=1}^{N} \mathbb{I}(r_i \leq 20),
% \end{equation}
% where $\mathbb{I}$ is the indicator function. The mean radius is also computed to provide an overall measurement of the circular motion. If the number of small radius circle is more than 40 and the average circular motion is less than 5, we filter this video with small camera trajectory.

% \subsubsection{User Study}
% To verify the effectiveness of our data filtering pipeline, we randomly selected 10,000 video clips as user study before filtering, of which the number of videos that satisfy our definition of 3D video is 1,163, and the percentage of 3D data is 11.6\%. We also randomly selected 10,000 video clips for people to annotate after data screening, and found that the number of 3D video annotations was 88,59 videos with a ratio of 88.6\%, which is 77\% higher compared to the previous one, indicating that our proposed method effectively preserves 3D data.

\subsection{Visual-conditional Multi-View Diffusion Model} \label{sec:model}
\paragraph{Preliminary.}
Diffusion models \cite{sohl2015deep,song2020denoising,ho2020denoising} operate by perturbing the training data $X_0 \sim  q(X_0)$ through a forward diffusion process and learning to reverse it. The forward diffusion process $X_t \sim q_{t|0}(X_t | X_0)$ can be formally represented by $X_{t} = \sqrt{\bar{\alpha}_{t}} \mathbf{X}_0 + \sqrt{1 - \bar{\alpha}_{t}} \boldsymbol{\epsilon}, \quad \boldsymbol{\epsilon} \sim \mathcal{N}(0, \mathbf{I})$, where $\bar{\alpha}_{t}$ is variance schedule used in noise scheduler. In theory, $X_t$ approximates an isotropic Gaussian distribution for sufficiently large timesteps $t$. The training objective is to learn the reverse process. 
% Thus, a trained diffusion model can generate a sample from the target distribution $q(X_0)$ by converting back-sampling noise from the Gaussian distribution through a reverse process. 

% \paragraph{Objective.}
\noindent\textbf{Objective.} We aim for multi-view prediction: generating novel views along specified camera trajectories from a single or sparse input, while ensuring consistency with the input appearance. 
MVD model inherits the generalizability of 2D diffusion model while capturing cross-view consistency, which naturally aligns with our goal.  Following this line, we present \textit{\ours}, a pose-free, visual-conditional MVD model trained on Internet videos to enable robust 3D generation (see Fig.\ref{fig:trainpipe}).

% \paragraph{Challenge.}
\noindent\textbf{Challenge.} The main technical challenge lies in learning precise camera control from pose-free videos. 
Previous works commonly incorporate camera parameters for both input and target views into diffusion models to guide multi-view generation from specified viewpoints. However, training these models generally requires expensive 3D data with precise camera pose annotations, which limits scalability. 
To address this,  we explore an alternative approach that conditions on 2D-inductive visual hints to implicitly control camera movement during training, thereby avoiding the need for hard-to-obtain camera trajectories. 
% \paragraph{Formulation.}

\noindent\textbf{Formulation.} Formally, we propose training the MVD model conditioned on 2D-inductive visual signals, referred to as \textit{visual-condition}, without incorporating  camera parameters. This task can be formulated as designing a conditional distribution, achieved by a conditional diffusion model that minimizes:
\begin{equation}
\label{eq:loss}
\mathbb{E}_{X_0, Y_0, \epsilon, t} \left[ \left\lVert \epsilon_{\theta}(X_t, Y_0, V, t) - \epsilon \right\rVert_2^2 \right],
\end{equation}
where $X_t$ denotes the noisy latent as mentioned in \cref{sec:model}. Here  $X_0=\left \{ x_{0}^{i}  \right \} _{i=1}^{N}$ represents a multi-view observation of 3D content, formed by sampling one clip from  \textit{\data}  as described in Section \ref{sec:data}, with $N=S+L$ being the number of frames in each clip.  
From $X_0$, $S$ frames are randomly selected as reference view(s), denoted  $Y_0=\left \{ y_{0}^{i}  \right \} _{i=1}^{S}$,  while the remaining $L$ frames are treated as target images, denoted  $G=\left \{ g^{i}  \right \} _{i=1}^{L}$. Our approach focuses on constructing the \textit{visual-condition} $V$, which guides the diffusion model to generate plausible 3D content estimates from target viewpoints consistent with the appearance of $Y_0$. 

\subsubsection{ Time-dependent Visual Condition} 
% \paragraph{\todo{Principle of Visual-condition.}}
\noindent\textbf{Principle of Visual-condition.}
A robust \textit{visual-condition} should satisfy  the following criteria: a) it can be constructed without the need for additional 3D annotations, b) it is independent of specific downstream tasks, and c) it offers sufficient generalization to support various task-specific visual conditions, enabling precise control of camera movements.

\vspace{2pt}
Ideally, this \textit{visual-Condition} can be derived  from  pixel-space hints within the original videos, implicitly guiding the model to learn camera position control from diverse, large-scale multi-view images.
Moreover, it should be robust enough to handle domain gaps between task-specific visual cues and pixels extracted from video data.
For example, in warping-based generation, warped images often suffer from issues like self-occlusions, artifacts, and distortions, creating a significant gap compared to real video data as shown in Fig. \ref{fig:single-3d} and Fig. \ref{fig:Vt-ablation}. Based on this, we propose constructing the \textit{visual-condition} by applying masks and noise to the input video data. Our design principles are: 
\begin{itemize}
\item \textbf{Masking}: Corrupting video data through random masking reduces reliance on direct pixel-space visual signals, helping the model partially mitigate the domain gap between task-specific visual cues and video data. 
\item \textbf{Noise Addition}: Adding noise to video data to approximate a Gaussian distribution. When applied to different downstream tasks, task-specific visual inputs are similarly noised, aligning their distribution with a Gaussian profile, and further bridging  the gap between video data and task-specific input.
\end{itemize}
% \uncer{Warping the given view(s) onto the camera plane defined by the target camera parameters provides an effective visual hint, as warp images inherently capture camera movement information through the rearrangement of pixels from the input images, replacing the camera parameters. However, it is indeed not trivial to construct warp images as conditioning in the use of such large-scale video data, especially in cases where the camera trajectories and 3D geometric structures of a large volume of video data are unknown. To address this dilemma, we first analyze the properties of warp images and then propose a solution.As shown in Fig. 4, warp images generally exhibit four distinct characteristics compared to regular images: 1) missing regions, 2) occlusions, 3) artifacts, and 4) geometric distortions. The first two characteristics arise the movement of the camera, which causes some points in the point cloud to be unable to project onto the target camera plane, or self-occlusion occurring within the camera plane. The latter two characteristics are caused by the imperfections in the estimated point cloud due to insufficient observation. Based on the above analysis, the specific content of warp images is formed by various complex factors, including point cloud quality, camera poses, and self-occlusion relationships in the 3D scene, making it challenging to simulate such warp images using video data. Therefore, we propose a novel solution. We abandon the highly impractical approach of simulating warp images from video data as visual hints. Instead, we attempt to explore whether it is feasible to use video data as visual hints during the training phase, while using warp images as visual hints during the inference phase. Our insight is to minimize the model's dependence on visual cues from video data as much as possible, thereby enabling the model to disregard the differences between visual cues from video data during training and warped images during inference.}

% In our preliminary attempts, a natural approach is to perturb and randomly mask video data, then use this corrupted video data as visual hints to condition the diffusion model.


% \paragraph{Time-dependent Noise.}
% \todo{To enhance the robustness of the \textit{visual-condition}, }
\noindent\textbf{Time-dependent Noise.} In our preliminary attempts, we initially  add  noise and random irregular masks to the video data, creating what we call `corrupted' video data $C_t$, as defined in Eq.\ref{eq:ct}. This corrupted data is then used as the \textit{visual-condition} for MVD model training.
A critical challenge of this strategy lies in determining an appropriate level of perturbation. If too much noise is added, the conditional signals become ineffective, resulting in poor visual quality and inaccurate camera control. Conversely, if insufficient noise is added, the corrupted data retains substantial details from the target images, causing the model to overly rely on visual hints from video data.
% To explain further, compared to using warped images as visual hints during inference, minimally corrupted video data retains significant information about the target views during training. This information leakage during training exacerbates the training-inference discrepancy, leading to a significant drop in test performance.

To overcome this, we further introduce a \textit{time-dependent noise} distribution applied to the video data. The core idea is to apply higher noise levels at larger time steps, effectively disrupting the video data to prevent over-reliance on it.
As the time step decreases, the noise level is reduced, providing  cleaner conditional signals to facilitate content generation.
However, as the noise level decreases, the risk of information leakage increases, causing the distribution to deviate from a Gaussian distribution.
To mitigate this, we propose gradually replacing the corrupted video data $C_t$ with the noisy latent $X_t$ as the \textit{visual-condition} 
 (see Eq.\ref{eq:mix}) , encouraging the model to  primarily rely on $X_t$ for generation while minimizing dependence on pixel-space signals from video data as timestep decreases. Additionally, $X_t$ is predicted by model and thus exhibits task-agnosticity, as formalized by:
\begin{equation} \label{eq:ct}
C_{t} = \sqrt{\bar{\alpha}_{t'}} (1-M)\mathbf{X}_0 + \sqrt{1 - \bar{\alpha}_{t'}} \boldsymbol{\epsilon}, \quad \boldsymbol{\epsilon} \sim \mathcal{N}(0, \mathbf{I})
\end{equation}
\begin{equation} \label{eq:mix}
V_t=[W_t\ast C_t+  \left ( 1-W_t \right ) \ast X_t;M]
\end{equation}
% \begin{equation}
% t'=f(t), 
% \end{equation}
% where $M=\left \{ m^{i}  \right \} _{i=1}^{N}$ denotes random irregular mask operations, \todo{ in which $m^{0:S}$ are the zero matrix to ensure the given reference images are clean without masking, 
where $M = \left\{  m^{0:S} \cup m^{S+1:N} \right \}$, with $m^{0:S}$ as the zero matrix, keeping the reference images $Y_0$ unmasked, and $m^{S+1:N}$ as random irregular masks applied to the target images $G$. $t'=f(t)$, function $f$ is strictly monotonically increasing and requires $t' < t$, which guarantees that $C_t$ contains at least as much information as $X_t$ at earlier timesteps. Here, $\bar{\alpha}_{t'}$ are variances used in DDIM \cite{song2020denoising},  and $V_t=\left \{ v_{t}^{i}  \right \} _{i=1}^{N}$ represents our final \textit{ visual-condition}, which is a mixture of $C_t$ and $X_t$, concatenated with masks $M$ along the channel dimension.  Consequently, Eq.\ref{eq:loss} can be reformulated as $\mathbb{E}_{X_0, Y_0, \epsilon, t} \left[ \left\lVert \epsilon_{\theta}(X_t, Y_0, V_t, t) - \epsilon \right\rVert_2^2 \right]$. 
In practice, an additional processing step assigns $v_{t}^{0:S}$ to the reference images $Y_0$ directly, in order to inject the clean information of $Y_0$ into the model, facilitating alignment between the predicted images and the reference images.
The term $W_t$ represents a balancing weight that decreases monotonically with timestep $t$, ranging from 1 to 0. 
% Function $f$ is strictly monotonically increasing and requires $t' < t$, which guarantees that $C_t$ contains at least as much information as $X_t$ at earlier timesteps. 
% Otherwise, when $t$ becomes sufficiently large, $C_t$ will approach Gaussian noise, which would result in a loss of control over camera movement.

\subsubsection{Visual-conditional Model Architecture.}
Our model architecture is based on video diffusion model \cite{svd}. However, we removed the time embedding, as we aim for the model to control the camera movement purely through visual conditions, rather than inferring movement trends based on temporal cues. To further minimize the effect of temporality, we shuffle the frames in each video clip, treating the data as unordered $X_0$. 
Specifically,  we randomly select a subset of frames from a video clip as reference images, with the remaining frames as target images. The number of reference images is randomly selected to accommodate different downstream tasks.  The multi-view diffusion model is optimized by calculating the loss only on the target images, as described in Eq.\ref{eq:loss}. For more details on the model architecture, such as design of self-attention layers, Zero-Initialize, trainable parameters, noise schedule and cross-attention, please refer to Appendix.

% The main backbone of our model follows the structure of 2D diffusion model but incorporates 3D self-attention to connect the latents of multiple images, as demonstrated in prior work \cite{shi2023mvdream}. Specifically, we adapt the existing 2D self-attention layers of the original 2D diffusion model into 3D self-attention by inflating different views within the self-attention layers. To inject visual conditions, we add the necessary convolutional kernels and biases via the Zero-Initialize \cite{singer2022make}. The model is initialized from a 2D diffusion model \cite{sd} and fine-tuned with all parameters, leveraging FlashAttention for acceleration. In line with prior work \cite{shi2023zero123++}, we found it crucial to switch from a scaled-linear noise schedule to a linear schedule to achieve better global consistency across multiple views. We perform cross-attention between the latents of multiple views and per-token CLIP embeddings of reference images via a linear guidance mechanism \cite{song2022diffusion}. 

% $V_t=\left \{ v_{t}^{i}  \right \} _{i=1}^{N}$ are the visual hints, which are used as condition injected into the diffusion model to guide the generation of multiple views in Eq.\ref{eq:loss}. $\bar{\alpha}_{t'}$ are variances used in DDIM. $W_t$ is the balance weight, which is designed to decrease monotonically with timestep $t$, ranging from 1 to 0. $X_t=\left \{ x_{t}^{i}  \right \} _{i=1}^{N}$ is the noise latent at timestep $t$, which introduces noise to $X_0$ by employing diffusion model’s inversion process. During the training phase, $R_0$ denotes corrupted video data formed by irregular masks. In the testing phase, $R_0$ denotes the warp images corresponding to a predefined camera trajectory. Function $f$ is designed to be strictly monotonically increasing and requires that $t' < t$, thus ensuring that $C_t$ does not contain less information than $X_t$. Otherwise, when timestep $t$ is large enough, $C_t$ will converge to Gaussian noise, resulting in no ability to control the camera movement at all. Here, $N = S + M$, where $S$ is the number of given images, and $M$ is the number of target images. 

\subsection{Visual-conditional  3D Generation} \label{sec:3DGen}
\begin{figure*}[tb]
\centering
\includegraphics[width=0.9\linewidth]{images/infer.pdf}
\caption{\small \textbf{\ours for Multi-View Generation}: From $n$ iteratively generated views (brown camera), we randomly select a few anchor views (yellow stars) to guide  the generation of  $m$ target views along the gray camera trajectory. 
We first perform keypoint matching to establish correspondences between anchor views.  
Then, monocular depth estimation is applied to the latest anchor view, followed by our 
 \textit{Iterative Sparse Pixel-Wise Depth Alignment} to refine the depth and recover a dense depth map. This dense depth is then used to project and  obtain  warped images from the gray camera viewpoints. The warped and anchor images are fed into \ours to produce  3D-consistent target views. Finally, the gray camera resets to brown, and the generated views  are added to $n$, guiding multi-view generation in the next iteration.
} 
\label{fig:infer}
\end{figure*}

% 假设我们的生成轨迹沿着左边所指的方向，棕色的相机为当前已经生成的视角，我们的目标是通过已有的生成图像生成灰色的指定视角。我们在已生成视角中选取若干个anchor views作为后续生成的视觉提示，并选定最后一个anchor view进行深度估计构建后续的视觉提示。我们利用离线的关键点匹配在不同的anchor views中寻找匹配关系，并使用单目深度估计算法估计深度。接着，我们提出使用Iterative Sparse Pixel-Wise Depth Alignment来修复最后一帧的深度的错误估计并恢复真实尺度。我们利用metric dense depth进行后续帧投影得到warped images. 这些images被送入SEED最后得到新的多视角生成结果。此时，这些灰色相机将会被置成棕色，进行后续生成。

%In this section, we leverage the 3D priors of \ours for domain-free 3D generation. We utilize monocular depth estimation \cite{fu2025geowizard} to provide preliminary 3D structure, and generate visual guidance with depth-based warping iteratively for multi-view generation. Recent efforts \cite{chung2023luciddreamer, fridman2024scenescape, lei2023rgbd2} typically require monocular depth or point cloud of the reference view, using 3D constraints to aid in multi-view consistency for subsequent generation. However, since the reference view typically has a limited observation of the scene, using offline methods often leads to scale ambiguity and geometric estimation errors. Previous methods usually conduct global alignment to recover depth scale but overlook the correction of geometric estimation errors, resulting in distortions and stretching artifacts. These errors will continue to accumulate in subsequent iterative generation, severely impacting the quality of the output.

%\todo{We use monocular depth estimation \cite{fu2025geowizard} to obtain an initial 3D structure and iteratively generate visual guidance through depth-based warping for multi-view generation. As illustrated in Fig.\ref{fig:infer} }
In this section, we apply the proposed \textit{\ours} for domain-free 3D generation. Given a single or a few input views, we iteratively generate warped images with predefined camera poses and estimated global depth \cite{bhat2023zoedepth} as the visual condition, then \ours is applied to generate frames corresponding to the target poses. This iterative pipeline is shown in Fig.\ref{fig:infer}, where the brown cameras represent the already generated views, and our objective is to generate the target views marked as gray cameras.

% We first apply monocular depth estimation \cite{bhat2023zoedepth} to obtain an initial 3D structure, then generate visual condition through a depth-based warping operation for multi-view generation.
% \vspace{2pt}
Recent efforts \cite{chung2023luciddreamer, fridman2024scenescape, lei2023rgbd2} rely on monocular depth or point clouds, and perform global point-cloud alignment to recover the actual geometry for subsequent generations. However, since the reference view often provides a limited scene observation, using offline methods tends to suffer from \textit{scale ambiguity} and \textit{geometric estimation errors}, while previous methods overlook the correction of geometric estimation errors, resulting in distortions and stretching artifacts. These errors accumulate during iterative generation, severely degrading the generation quality.
% and apply 3D constraints to ensure multi-view consistency in subsequent generations.

% However, since the reference view often provides a limited scene observation, using offline methods tends to suffer from \textit{scale ambiguity} and \textit{geometric estimation errors}. 
% Previous approaches typically perform global alignment to recover depth scale, but overlook the correction of geometric estimation errors, resulting in distortions and stretching artifacts. These errors accumulate during iterative generation, severely degrading  output quality.

% Recent efforts \cite{chung2023luciddreamer, fridman2024scenescape, lei2023rgbd2} typically aligned the affine invariant depth with the preceding estimated 3D structure with a one-step global scale and shift recovery, which can not monocular depth estimation lead to geometry ambiguity due to limited observation.
% global align 不能解决xxx 具体解释。
% However, monocular depth estimation leads to geometry ambiguous due to limited observation, which cannot be corrected simply by aligning the global scales from the preceding frames. 
% Therefore, visual hints generated through previous methods are prone to distortions and stretching artifacts that affect subsequent generation.\todo{viewcrafter?}
% To address this limitation, we propose a learning based sparse-to-global depth alignment. starting by sparse pixel-level depth restoration via matching prior on multi-view generation, which restores the depth scale locally and corrects geometric estimation errors point-by-point. Then, these sparse and accurate depth are transformed by Locally Weighted Linear Regression \cite{frozenrecon} to recover the global metric of the entire depth map. 

To further correct local geometry errors, we propose pixel-wise depth scale alignment using sparse keypoints. we perform high-degree-of-freedom independent optimization for all keypoints by leveraging multi-view matching priors from anchor views. 
Each keypoint independently identifies its multi-view matches,  enabling the recovery of both depth scale and surrounding geometry.
Finally, we propagate the corrected  scale to the entire depth map using the 2D distances between keypoints and their neighbors.

% Previous works \cite{chung2023luciddreamer,yu2024viewcrafter} usually maintain a global 

% point cloud for next-frame rendering, however, the depth estimation and MVD are tightly coupled, using global point cloud to produce visual guidance may easily introduce error accumulation. Therefore, we cut the correlation with the early-stage estimation, and use only the latest generated view for next-frame visual guidance. 
% pre-define a camera trajectory for synthesizing novel viewpoints, 

% Following \cite{luciddreamer, wonderworld}, we utilize a monocular depth estimation \cite{geowizard} to provide preliminary geometry, pre-define a camera trajectory for synthesizing novel viewpoints, and generate partial visual hints as novel view guidance with homography warping. We further introduce a 3D Gaussian Splatting \cite{3dgs} with camera refinement for 3D representation.
% Benefiting from the robust visual conditioning strategy, our MVD model demonstrates resilience to artifacts and distortions from the monocular depth estimation for warping. However, significant viewpoint shifts and depth estimation errors still remain challenging in certain regions. To address these issues, we propose learning-based monocular geometric alignment, which leverage the robust matching prior \cite{lightglue} to recover the actual scale of depths and corrects erroneous where needed.
Specifically, let $\{T_i\}_{i=0}^{N}$ denote  the predefined camera trajectory. Suppose we have generated $n$ images $\{I_i\}_{i=0}^n$, we now proceed to generate the next $m$ views using warped image from the last anchor views $I_n$,  which referred to as source view. We first utilize the pre-trained MoGe \cite{wang2024moge} to estimate affine-invariant depth $\boldsymbol{\hat{D}}_n$ of $I_n$. Inspired by \cite{xu2023frozenrecon}, we perform sparse alignment with $1024$ pairs of matching keypoints $\{\mathbf{m}_n, \mathbf{m}_i\}_k$, obtained by the pre-trianed extractor SuperPoint \cite{detone2018superpoint} and feature matcher LightGlue \cite{lindenberger2023lightglue}. For each matched point, we optimize the corresponding scale $\alpha^k$ and shift $\beta^k$ parameters, where $k \in [0, 1024]$, Our core idea is to recover the depth scaling by minimizing the $L_2$ distance of re-projection between matching points. For each iteration, the warping operation $\Pi_{n\rightarrow i}$ transforms pixels from the source image’s coordinate frame to the target image’s coordinate frame, formulated as: $\Pi_{n \rightarrow i}(\hat{d}_n) =  \hat{d}_n K_{i} T_{i} T_{n}^{-1} K_{n}^{-1}$, where $K_i,  K_n,T_i, T_n$ represent the intrinsic and extrinsic parameters of the source and target frames, respectively. The alignment for each pair is performed using normalized coordinates, ensuring that the warping aligns with the matching prior:
\begin{equation}
\begin{gathered}
    \alpha^{k*},\beta^{k*} = \mathop{argmin} \limits_{\alpha^{k},\beta^{k}} \sum_{i=0}^n || \hat{d}_n^{k*} K_i T_i T_n^{-1} K_n^{-1} m_n^t - m_i^t||_2^2 \\
    \hat{d}_n^{k*} = \alpha^{k} \odot \hat{d}_n^k + \beta^{k},
\end{gathered}
\end{equation}
where $\hat{d}_n^{k*}$ is the recovered depth of $k$th pixel and $\odot$ is the pixel-wise Hadamard Product, we minimize the matching loss via gradient descent to obtain best scale $ \alpha^{k*}$ and shift parameters $\beta^{k*}$ for each pixel. By performing individual scale recovery and geometry correction, we decouple the depth correlation among different points, achieving accurate single-view reconstruction.

After that, we set these recovered positions as sparse guidance $\hat{d}_n^*$, and introduce Locally Weighted Linear Regression \cite{xu2023frozenrecon} (marked as LWLR in Fig.\ref{fig:infer}) to recover the whole depth map based on the locations between guided points and the other target points. Let the global scale and shift parameters be $\boldsymbol{\beta_{u,v}} = [\boldsymbol{S}_{scale},\boldsymbol{S}_{shift}]_{u,v} ^ \mathsf{T}$, the metric depth recovery can be formulated as: 
\begin{equation}
\min_{\boldsymbol{\beta}_{u, v}} (\hat{d}_n^* -\boldsymbol{X}\boldsymbol{\beta}_{u,v})^\mathsf{T}\boldsymbol{W}_{u,v}(\hat{d}_n^* -\boldsymbol{X}\boldsymbol{\beta}_{u,v})+\lambda\boldsymbol{S}_{shift}^2.
\end{equation}

% appendix 
% Denote $(u,v)$ represent the 2D positions of the remaining target points, their depth $\boldsymbol{\hat{D}}_n$ can be fitted to the sparse guided points by minimizing the squared locally weighted distance, which is reweighted by the diagonal weight matrix as:
% \begin{equation}
%     \boldsymbol{W}_{u,v}=diag(w_1,w_2,...,w_m), w_i=\frac1{\sqrt{2\pi}}\exp(-\frac{\mathrm{dist}_i^2}{2b^2}),
% \end{equation}
% where $b$ is the bandwidth of Gaussian kernel, and $\mathrm{dist}$ is the Euclidean distance between the guided point and the underestimate target point. Denote $\boldsymbol{X}$ the homogeneous representation of $\boldsymbol{\hat{D}}_n$, the scale map $\boldsymbol{S}_{scale}$ and shift map $\boldsymbol{S}_{shift}$ of target points can be calculated by iterating every location on the whole image, which can be formulated as:
% \begin{equation}
%     \begin{gathered}
%         \min_{\boldsymbol{\beta}_{u, v}} (\hat{d}_n^* -\boldsymbol{X}\boldsymbol{\beta}_{u,v})^\mathsf{T}\boldsymbol{W}_{u,v}(\hat{d}_n^* -\boldsymbol{X}\boldsymbol{\beta}_{u,v})+\lambda\boldsymbol{S}_{shift}^2, \\
%     \boldsymbol{\hat{\beta}}_{u,v}=(\boldsymbol{X}^\mathsf{T}\boldsymbol{W}_{u,v}\boldsymbol{X}+\lambda)^{-1}\boldsymbol{X}^\mathsf{T}\boldsymbol{W}_{u,v}\hat{d}_n^*, \\
%     \boldsymbol{\beta_{u,v}} = [\boldsymbol{S}_{scale},\boldsymbol{S}_{shift}]_{u,v} ^ \mathsf{T}, \\
%     \boldsymbol{D}_n = \hat{d}_n^* \oplus  \boldsymbol{S}_{scale} \odot \boldsymbol{\hat{D}}_n + \boldsymbol{S}_{shift},
% \end{gathered}
% \end{equation}
% where $\boldsymbol{D}_n$ is the scaled whole depth map, $\oplus$ is the concatenation operator, $\lambda$ is a $l_2$ regularization hyperparameter used for restricting the solution to be simple. Besides, the explicit constraint of the source frame with the target frames allows each novel view to maintain contextual consistency from preceding generations.

After obtaining the aligned depth $\boldsymbol{D}_n$, we generate the target visual hint through warping $\hat{I}_j = \Pi_{n \rightarrow j}(\boldsymbol{D}_n)$. The warped image $\{\hat{I}_j\}_{j=n}^{n+m}$ carries unfilled regions as the binary warping mask $\{M_j\}_{j=n}^{n+m}$, which serves as a strong visual hint for \ours to perform generation. To ensure multi-view consistency between the newly generated sequence and the previous content, we randomly select $k$ anchor views $\{I_k\},k \in [1,N]$ from the earlier  generated frames to guide subsequent generation. The generation process  can be formulated as: $I_j = \ours (\hat{I}_j, M_{j}, \{I_0,I_k\})$. We iteratively perform depth estimation, alignment, warping, and generation  until all target images are acquired. More details can be found at Appendix.

\noindent\textbf{3D Reoncstruction.} \label{sec: 3dgs} We reconstruct the 3D scene using 3D Gaussian Splatting (3DGS) \cite{3dgs}. Following \cite{fan2024instantsplat}, we additionally introduce joint pose-Gaussian optimization, where camera parameters are treated as learnable variables alongside Gaussian attributes, thus reducing gaps between generated viewpoints and their corresponding camera poses.

% appendix
% Our training minimizes the sum of photometric loss and SSIM loss as the original 3DGS. We additionally introduce a perceptual loss (LPIPS \cite{lpips}) to mitigate the impact of subtle \textbf{inter-frame} discrepancies in multi-view generated images on 3D geometric structure (3DGS) reconstruction. LPIPS emphasizes higher-level semantic consistency between the Gaussian-rendered and generated multi-view images, rather than focusing on minor high-frequency differences.
% Besides, the potential \textbf{inner-frame} diversity may cause inconsistency with the corresponding camera poses. Following \cite{fan2024instantsplat}, we introduce joint pose-Gaussian optimization, where camera parameters are treated as learnable variables alongside Gaussian attributes, thus reducing gaps between generated viewpoints and their corresponding camera poses.





% The intrinsic and extrinsic of the reference frame and the warped target visual hints $\{\hat{I}_j\}_{j=n}^{n+m}$ are denoted as $K_n, \{K_j\}_{j=n}^{n+m}$ and $T_n, \{T_j\}_{j=n}^{n+m}$. The warping operation between reference and on of the target view $\Pi_{n \rightarrow j}$ can be defined as: $\Pi_{n \rightarrow j}(\cdot) =  d_n K_{j} T_{j} T_{n}^{-1} K_{n}^{-1}$, where 


% Previous works \cite{chung2023luciddreamer,yu2024viewcrafter} usually maintain a global point cloud for next-frame rendering, however, the depth estimation and MVD are tightly coupled, using global point cloud to produce visual guidance may easily introduce error accumulation. Therefore, we cut the correlation with the early-stage estimation, and use only the latest generated view for next-frame visual guidance. However, to maintain geometric consistency within the 3D scene, It is required to restore the actual depth scale so that the next frame will be aligned to the expected camera trajectory. 


% This exploits multi-view consistency for point-by-point geometric restoration and global scale recovery for multi-view generation, providing higher quality visual guidance for multi-view generation.


% Additionally, we explicitly constrain the alignment of the point cloud in the current frame with the previous frame, allowing each new view to incorporate contextual information from preceding frames.


% Inspired by \cite{frozenrecon}, we present a learning-based monocular geometric alignment, which leverages the robust matching prior to \cite{lightglue} to obtain precise metric depth. Instead of directly recovering the actual scale at once, we conduct geometric alignment from a few reliable matching points. For each matched point, we predict a scale and offset, which not only restores the depth scale locally but also corrects potential geometric estimation errors. We then diffuse these local metric to obtain global metric depth. Specifically, for the $i^{th}$ step, denote the reference image $I_i$, and the corresponding mono-depth map $d_i$, the corresponding intrinsic and extrinsic are $K_i, T_i$, we detect feature correspondences between the target image and each reference image $I_j, j \in (0, i-1)$ by applying the LightGlue \cite{lightglue}, obtaining $k$ groups of matching pairs $\{\mathbf{m}_i, \mathbf{m}_j\}$, where $k=1024$ in our experiment.

% Next, we scale the matched monocular depths $d_i$ of the target image with learnable scale $\alpha$ map and shift  $\beta$ map, to yield the sparse metric depth $\hat{d}_i$:
% \begin{equation}
%     \hat{d}_i =  \alpha \cdot (\alpha \cdot d_i + \beta)  + \beta,
% \label{eq: scale shift}
% \end{equation}
% where we set $\alpha = 4.0 $ and $\beta = 0.25$ for faster convergence. For each iteration, the optimized metric depth is then used in the warping operation $\Pi_{i\rightarrow j}$ to transform pixels from the reference image’s coordinate frame to the target image’s coordinate frame, yielding warped coordinates $\mathbf{C}_{\text{sample}}^j = \Pi_{i\rightarrow j}(m_i)$. The matching loss is computed for each image pair using normalized coordinates, ensuring the warping aligns with detected match points:
% \begin{equation}
%     \mathcal{L}_{\text{match}} = \frac{1}{|\mathbf{m}_j|} \sum{\mathbf{m}_j} \| \mathbf{C}_{\text{sample}}^j - \mathbf{m}_j \|_2^2,
% \end{equation}
% where we minimize $\mathcal{L}_{\text{match}}$ via gradient descent over the scale and shift parameters. Finally, we utilize the Locally Weighted Liner Regression \cite{frozenrecon} to diffuse the sparse points to global scale-consistent depth. We conducted depth estimation, learning-based alignment, warping, and generation repeatedly until we had acquired all predefined multi-view images.

% \noindent\textbf{3D Reconstruction.}  After acquiring the multi-view images through the above process, we reconstruct the 3D scene using 3D Gaussian Splatting (3DGS) \cite{3dgs}. 3DGS represents scenes with a set of explicit anisotropic 3D Gaussians. Each Gaussian distribution is defined by a 3D covariance matrix $\bm{\Sigma}$ and a center position at point (mean) $\mathcal{X}$. A 3D Gaussian distribution $G(\mathcal{X})$ is formulated as follows:
% \begin{equation}
%     G(\mathcal{X}) = e ^{- \frac{1}{2} \mathcal{X}^{T} \bm{\Sigma}^{-1} \mathcal{X}},
% \end{equation}
% the rendering color $\boldsymbol{C}$ of each pixel is accumulated by blending the overlapping Gaussians as $\boldsymbol{C} = \bm{\Sigma}_{i \in N} \alpha_i c_i \Pi_{j=1}^{i-1} (1 - \alpha_j)$, where $\alpha_i$ is $\sigma_i$ multiplied by $\bm{\Sigma}'$. The tile-based rasterizer is utilized for efficient forward and backward passes. We concatenate the monocular depth estimates for each viewpoint from the previous stage into an initial point cloud, and optimize Gaussians with generated multi-view images. 

% However, the multi-view images are obtained from generation, the potential diversity may cause problems of inconsistency in the the generated views with their corresponding camera poses. Following \cite{instantsplat}, we further introduce a joint pose-Gaussian optimization to remove gaps between generated viewpoints and camera poses. Specifically, we turn camera parameters $\boldsymbol{T}$ into learnable variables with Gaussians attributes $G$. The detailed optimization is as follows:
% \begin{equation}
%     \boldsymbol{G}^*,\boldsymbol{T}^*=\arg\min_{\boldsymbol{G},\boldsymbol{T}}\sum_{v\in N}\sum_{i=1}^{HW}\left\|\tilde{\boldsymbol{C}}_v^i(\boldsymbol{G},\boldsymbol{T})-\boldsymbol{C}_v^i(\boldsymbol{G},\boldsymbol{T})\right\|,
% \end{equation}
% where $N$ is the number of generated views. This joint-optimization reduces the effects of inconsistencies between the generated observation and the camera poses, and promotes more robust 3D reconstruction.

% For more effectively optimized by gradient decent, the 3D covariance matrix  $\Sigma$  can be decomposed into a rotation matrix $\textbf{R}$ and a scaling matrix $\textbf{S}$ via $\bm{\Sigma} = \textbf{R}\textbf{S}\textbf{S}^{T}\textbf{R}^{T}$, where $\textbf{J}$ is the Jacobian of the affine approximation of the projection transformation. Finally, the color $C$ of each pixel is accumulated by blending the overlapping Gaussians as $C = \bm{\Sigma}_{i \in N} \alpha_i c_i \Pi_{j=1}^{i-1} (1 - \alpha_j)$, where $\alpha_i$ is $\sigma_i$ multiplied by $\bm{\Sigma}'$. The tile-based rasterizer is utilized for efficient forward and backward pass.





% For each iteration, the optimized metric depth is then used in a point cloud warping operation to transform pixels from the reference image’s coordinate frame to the target image’s coordinate frame based on the relative pose \mathbf{P}{\text{rel}}^i, yielding warped coordinates \mathbf{C}{\text{sample}}^i and a validity index set \mathbf{V}_{\text{idx}}.
